Spatial and Statistical Modeling of Multi-Panel Millimeter Wave Self-Interference

Characterizing self-interference is essential to the design and evaluation of in-band full-duplex communication systems. Until now, little has been understood about this coupling in full-duplex systems operating at millimeter wave (mmWave) frequencies, and it has been shown that the highly-idealized models proposed for such do not align with practice. This work presents the first spatial and statistical model of mmWave self-interference backed by measurements, enabling engineers to draw realizations that exhibit the large-scale and small-scale spatial characteristics observed in our nearly 6.5 million measurements taken at 28 GHz. Core to our model is its use of system and model parameters having real-world meaning, which facilitates its extension to systems beyond our own phased array platform through proper parameterization. We demonstrate this by collecting nearly 13 million additional measurements to show that our model can generalize to two other system configurations. We assess our model by comparing it against actual measurements to confirm its ability to align spatially and in distribution with real-world self-interference. In addition, using both measurements and our model of self-interference, we evaluate an existing beamforming-based full-duplex mmWave solution to illustrate that our model can be reliably used to design new solutions and validate the performance improvements they may offer.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> sec-contribution-i.tex <==
\section{Analog Beamforming Codebook Design for Full-Duplex mmWave Systems}
% \section{Analog Beamforming Codebook Design} 
\label{sec:contribution}


Practical \mmwave systems---which have operated in a half-duplex fashion thus far---rely on beam alignment to identify beams that deliver high beamforming gain when serving a particular user.
This is typically done by sweeping a set of candidate beams called a \textit{codebook} and measuring the \gls{rsrp} for each beam candidate in order to select which is used to close a link. % for a given \mmwave link.
This beam alignment procedure allows a \mmwave system to reliably deliver high beamforming gain without the need for downlink/uplink \mimo channel knowledge (i.e., $\vhtx$ and $\vhrx$).
% A conventional beam codebook is often constructed by discretizing a service region based on the number of beams in the codebook or their beamwidth.
A conventional beam codebook can be constructed by distributing a number of beams spatially across some desired service region, typically based on their beamwidth.
% In this work, 

As mentioned in the introduction, plenty of existing work has designed particular transmit and receive beams $\vf$ and $\vw$ to use at the \bs to reduce self-interference when full-duplexing downlink and uplink users, but these existing designs have a number of practical shortcomings.
% These existing designs have a number of practical shortcomings, however.
In this work, we instead design transmit and receive beam codebooks $\precbbar$ and $\comcbbar$, from which the \bs can draw for $\vf$ and $\vw$ via conventional beam alignment.
% Put simply, $\vf \in \precbbar \subset \precb$ and $\vw \in \comcbbar \subset \comcb$.
% \begin{align}
% \vf \in \precbbar \subset \precb, \quad \vw \in \comcbbar \subset \comcb.
% \end{align}
% If successful, our beam codebooks will have effects twofold.
The goal of our design---which we call \lonestar---is to create codebooks that a full-duplex \mmwave \bs can use to deliver high beamforming gain to users while simultaneously mitigating self-interference.
% A full-duplex \mmwave \bs with our codebooks will be able to deliver high beamforming gain to users via beam alignment while simultaneously mitigating self-interference.
This will be achieved by strategically designing $\precbbar$ and $\comcbbar$ such that their transmit and receive beams couple low self-interference, regardless of which $\vf \in \precbbar$ and $\vw \in \comcbbar$ are selected following beam alignment.
In contrast, off-the-shelf codebooks created for conventional \mmwave systems can deliver high beamforming gain but are not necessarily robust to self-interference if used in full-duplex systems \cite{roberts_wcm}. % ; we demonstrate this in our numerical results in \secref{sec:simulation-results} and also highlighted this through measurements in \cite{roberts_att_angular,roberts_steer}.
In fact, this was confirmed in our recent measurement campaign \cite{roberts_att_angular} and in our recent work \cite{roberts_steer}, both of which showed that conventional beams typically couple prohibitively high amounts of self-interference if used in a practical full-duplex \mmwave system.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth,height=\textheight,keepaspectratio]{fig/lonestar_timeline_type_05}
    \caption{\lonestar is executed following estimation of the self-interference channel $\mH$. Over the coherence time of $\mH$, transmit and receive beam codebooks designed with \lonestar can be used for beam alignment and subsequently to serve downlink and uplink users in a full-duplex fashion.}
    \label{fig:timeline}
\end{figure*}


Our envisioned use of \lonestar is depicted in \figref{fig:timeline}, which illustrates that our design need only be executed once per coherence time of $\mH$, allowing the same codebook design to be used over many downlink-uplink user pairs (i.e., data transmissions).
This is a key advantage of \lonestar versus most existing \mmwave full-duplex solutions, which tailor their beams for each downlink-uplink user pair and often require real-time downlink/uplink \mimo channel knowledge.
Naturally, the coherence time of \mmwave self-interference, which is not currently well understood, will be an important factor in justifying the use of \lonestar since it dictates how frequently \lonestar needs to be re-executed.
Nonetheless, if our design sufficiently mitigates self-interference between all beam pairs, a \mmwave \bs employing our codebooks can seamlessly operate in a full-duplex fashion without any additional self-interference cancellation---any transmit and receive beams from our codebooks selected via beam alignment will couple sufficiently low self-interference.
As such, we name the design methodology herein \lonestar, since it has the potential to be a standalone solution enabling simultaneous transmission and reception in full-duplex \mmwave systems.
% \lonestar could also enhance existing \mmwave full-duplex work that accounts for codebook-based analog beamforming.
% Hybrid beamforming full-duplex systems could leverage our codebooks to weaken the effective self-interference channel post beam alignment.
% Furthermore, codebooks designed by \lonestar could also enhance existing \mmwave full-duplex solutions, including those for hybrid beamforming systems.

\subsection{Quantifying Our Codebook Design Criteria}
In pursuit of transmit and receive beam codebooks that reliably offer high sum spectral efficiency $\setx + \serx$, we desire sets of transmit and receive beams that can deliver high $\snrtx$ and $\snrrx$ while coupling low self-interference $\inrrx$.
As mentioned, cross-link interference $\inrtx$ is fixed for a given downlink-uplink user pair since it does not depend on the choice of $\vf$ nor $\vw$.
%The goal of \lonestar is to produce a codebook of transmit beams $\precbbar$ and a codebook of receive beams $\comcbbar$ with objectives twofold:
%\begin{enumerate}
%    \item The codebooks contain transmit and receive beams that deliver high beamforming gain and collectively provide coverage over some defined spatial regions.
%    \item Each transmit-receive beam pair couples low self-interference.
%\end{enumerate}
In the remainder of this section, we first quantify our codebook design criteria and then assemble a design problem that tackles both objectives jointly.
As we proceed with outlining our design, please refer to \figref{fig:block} for an illustration of the inputs and outputs of \lonestar.
% We outline our methodology by first quantifying our design criteria and then assembling our codebook design problem.
% In the next section, we present an algorithm for solving our codebook design problem.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth,height=0.24\textheight,keepaspectratio]{fig/lonestar_block_type_02}
    \caption{Using an estimate of the self-interference channel and knowledge of the estimation error variance, \lonestar produces transmit and receive beamforming codebooks that serve some coverage regions with quality based on tolerated coverage variances.}
    \label{fig:block}
\end{figure}

\begin{definition}[Transmit and receive coverage regions]
% Let $\dirtxset$ be a set of $\Mtx$ directions---or a \textit{transmit coverage region}---that our transmit codebook $\precbbar$ aims to serve, and let $\dirtxset$ be a set of $\Mrx$ receive directions---or a \textit{receive coverage region}---that our receive codebook $\comcbbar$ aims to serve.
Let $\dirtxset$ be a set of $\Mtx$ directions---or a \textit{transmit coverage region}---that our transmit codebook $\precbbar$ aims to serve, and let $\dirrxset$ be a \textit{receive coverage region} defined analogously.
\begin{align}
\dirtxset = \braces{\dirtx\idx{i} : i = 1, \dots, \Mtx}, \qquad \dirrxset = \braces{\dirrx\idx{j} : j = 1, \dots, \Mrx}
% \dirtxset = \braces{\dirtx\idx{i} : i = 1, \dots, \Mtx} \\
% \dirrxset = \braces{\dirrx\idx{j} : j = 1, \dots, \Mrx}
\end{align}
Note that $\dirtx\idx{i}$ and $\dirrx\idx{j}$ each may capture both azimuthal and elevational components of a given steering direction.
$\dirtxset$ and $\dirrxset$, for example, may be comprised of $\Mtx = \Mrx$ directions uniformly distributed over the region from $-60^\circ$ to $60^\circ$ in azimuth and $-30^\circ$ to $30^\circ$ in elevation. % , each with $10^\circ$ steps.
\end{definition}

%Let $\Atx \in \setmatrixcomplex{\Nt}{\Mtx}$ be the matrix of transmit array response vectors evaluated at the directions in $\dirtxset$, and let $\Arx \in \setmatrixcomplex{\Nr}{\Mrx}$ be the matrix of receive array response vectors evaluated at the directions in $\dirrxset$.
%\begin{align}
%\Atx &= 
%\begin{bmatrix}
%\atx{\dirtx\idx{1}} & \atx{\dirtx\idx{2}} & \cdots & \atx{\dirtx\idx{\Mtx}}
%\end{bmatrix}  \\
%\Arx &= 
%\begin{bmatrix}
%\arx{\dirrx\idx{1}} & \arx{\dirrx\idx{2}} & \cdots & \arx{\dirrx\idx{\Mrx}}
%\end{bmatrix}
%\end{align}

\begin{definition}[Transmit and receive beamforming codebooks]
We index the $\Mtx$ beams in $\precbbar$ and the $\Mrx$ beams in $\comcbbar$ according to $\dirtxset$ and $\dirrxset$, respectively, as % $\precbbar = \braces{\vf_1, \dots, \vf_{\Mtx}}$ and $\comcbbar = \braces{\vw_1, \dots, \vw_{\Mrx}}$, 
\begin{align}
\precbbar = \braces{\vf_1, \dots, \vf_{\Mtx}} \label{eq:unpack-1}, \qquad \comcbbar = \braces{\vw_1, \dots, \vw_{\Mrx}}
% \precbbar = \braces{\vf_1, \dots, \vf_{\Mtx}} \label{eq:unpack-1} \\
% \comcbbar = \braces{\vw_1, \dots, \vw_{\Mrx}}
\end{align}
where $\vf_i \in \precb$ is responsible for transmitting toward $\dirtx\idx{i}$ and $\vw_j \in \comcb$ is responsible for receiving from $\dirrx\idx{j}$. % \footnote{Recall, physically realizable $\vf$ and $\vw$ are fundamentally required to come from $\precb$ and $\comcb$, capturing digitally controlled phase shifters and attenuators.}
Using this notation, we build the transmit codebook matrix $\precbmat$ by stacking transmit beams $\vf_i$ as follows and the receive codebook matrix $\comcbmat$ analogously.
\begin{align}
\precbmat = 
\begin{bmatrix}
\vf_1 & \vf_2 & \cdots & \vf_{\Mtx}
\end{bmatrix} \in \setmatrixcomplex{\Nt}{\Mtx}, \qquad
\comcbmat = 
\begin{bmatrix}
\vw_1 & \vw_2 & \cdots & \vw_{\Mrx}
\end{bmatrix} \in \setmatrixcomplex{\Nr}{\Mrx} \label{eq:unpack-2}
%\precbmat = 
%\begin{bmatrix}
%\vf_1 & \vf_2 & \cdots & \vf_{\Mtx}
%\end{bmatrix} \in \setmatrixcomplex{\Nt}{\Mtx} \\
%\comcbmat = 
%\begin{bmatrix}
%\vw_1 & \vw_2 & \cdots & \vw_{\Mrx}
%\end{bmatrix} \in \setmatrixcomplex{\Nr}{\Mrx} \label{eq:unpack-2}
\end{align}
\end{definition}

\begin{definition}[Transmit and receive beamforming gains]
    Let $\Gtx^2\parens{\dirtx\idx{i}}$ be the transmit beamforming gain afforded by $\vf_i$ in the direction $\dirtx\idx{i}$ and $\Grx^2\parens{\dirrx\idx{j}}$ be the receive beamforming gain afforded by $\vw_j$ in the direction $\dirrx\idx{j}$, expressed as
    \begin{align}
    \Gtx^2\parens{\dirtx\idx{i}} &= \bars{\atx{\dirtx\idx{i}}\ctrans  \vf_i}^2 \leq \Nt^2 \label{eq:Gtx}, \qquad 
    \Grx^2\parens{\dirrx\idx{j}} = \bars{\arx{\dirrx\idx{j}}\ctrans  \vw_j}^2 \leq \Nr^2. % \label{eq:Grx}.
    \end{align}
    The transmit and receive beamforming gains are upper-bounded by $\Nt^2$ and $\Nr^2$, respectively, by virtue of normalizations presented in our system model. 
    Maximum beamforming gains can be achieved toward any direction $\dir$ with beams $\vf = \atx{\dir}$ and $\vw = \arx{\dir}$, respectively, often referred to as \textit{conjugate beamforming} or \textit{matched filter beamforming} \cite{heath_lozano}.
\end{definition}

\begin{definition}[Average self-interference coupled]
The coupling between the $i$-th transmit beam $\vf_i$ and the $j$-th receive beam $\vw_j$ can be captured by the product $\vw_j\ctrans \mH \vf_i$, which can be extended to all transmit-receive beam pairs as $\comcbmat\ctrans \mH \precbmat \in \setmatrixcomplex{\Mrx}{\Mtx}$.
\lonestar will aim to minimize the coupling across all beam pairs and does so by minimizing the average $\inrrx$ coupled between beam pairs, which can be written as
\begin{align}
\inrrxavg 
&= \frac{1}{\Mtx \cdot \Mrx} \cdot \sum_{i=1}^{\Mtx} \sum_{j=1}^{\Mrx}  \frac{\powertxbs \cdot G^2 \cdot \bars{\vw_j\ctrans \mH \vf_i}^2}{\powernoisebs} = \frac{\powertxbs \cdot G^2}{\powernoisebs} \cdot \frac{\normfro{\mW\ctrans \mH \mF}^2}{\Mtx \cdot \Mrx}. \label{eq:inr-rx-avg}
\end{align}
Minimizing $\inrrxavg$ reduces to minimizing $\normfro{\mW\ctrans \mH \mF}^2$ through the design of $\mF$ and $\mW$ for a given $\mH$ since all other terms are constants.
In \lonestar's attempt to minimize $\inrrxavg$, it must also ensure that the beams in $\precbmat$ and $\comcbmat$ remain useful in serving users; of course, $\precbmat$ and $\comcbmat$ minimize $\inrrxavg$ when driven to $\zeromat$ if unconstrained.
We now quantify a means to constrain \lonestar to ensure adequate service is maintained in its aim to minimize $\inrrxavg$.
\end{definition}

\begin{definition}[Transmit and receive coverage variances]
To offer flexibility in minimizing $\inrrxavg$, \lonestar tolerates some loss in beamforming gain over the transmit and receive coverage regions.
In other words, we allow for some transmit and receive beamforming gain less than $\Nt^2$ and $\Nr^2$ over $\txdirsetcb$ and $\rxdirsetcb$ in pursuit of reduced self-interference. % , as we will see.
Let $\sigmatx^2 \geq 0$ be the maximum variance tolerated in delivering maximum transmit gain across $\txdirsetcb$, normalized to $\Nt^2$.
Defining $\sigmarx^2 \geq 0$ analogously, we express these tolerated coverage variances as %\footnote{We use magnitude here, which is simply the square root of power gain in \eqref{eq:Gtx}.}
\begin{align}
\frac{1}{\Mtx} \cdot \sum_{i=1}^{\Mtx} \frac{\bars{\Nt - \Gtx\parens{\dirtx\idx{i}}}^2}{\Nt^2} &\leq \sigmatx^2 \label{eq:sigma-tx}, \qquad 
\frac{1}{\Mrx} \cdot \sum_{j=1}^{\Mrx} \frac{\bars{\Nr - \Grx\parens{\dirrx\idx{j}}}^2}{\Nr^2} \leq \sigmarx^2. % \label{eq:sigma-rx}.
% \frac{1}{\Mtx} \cdot \sum_{i=1}^{\Mtx} \frac{\bars{\Nt - \Gtx\parens{\dirtx\idx{i}}}^2}{\Nt^2} &\leq \sigmatx^2 \label{eq:sigma-tx} \\ %, \quad 
% \frac{1}{\Mrx} \cdot \sum_{j=1}^{\Mrx} \frac{\bars{\Nr - \Grx\parens{\dirrx\idx{j}}}^2}{\Nr^2} &\leq \sigmarx^2 \label{eq:sigma-rx}.
\end{align}
% Note that we used magnitude here, which is simply the square root of power gain in \eqref{eq:Gtx}.
Here, $\sigmatx^2$ and $\sigmarx^2$ are design parameters that can be tuned by system engineers; increasing them will offer \lonestar greater flexibility in reducing $\inrrxavg$ but may degrade coverage since it permits more variability in beamforming gain over the service regions.
% More variance across transmit and receive gain provided by our beams may increase the disparity of service seen across users but would also allow our design more flexibility in its attempt to reduce self-interference.
\end{definition}


\subsection{Assembling Our Codebook Design Problem}
In the previous subsection, we outlined that \lonestar will attempt to minimize the average self-interference coupled by transmit and receive beams while constraining the variance of beamforming gain delivered to specified transmit and receive coverage regions.
With expressions for our codebook design criteria in hand, we now turn our attention to assembling a formal design problem.
% Let $\gtxtgt = \Gtxtgt \cdot \onevec{\Mtx}$ and $\grxtgt = \Grxtgt \cdot \onevec{\Mrx}$ be vectors containing the target transmit and receive gains at each entry.
%\begin{align}
%\gtxtgt = \Gtxtgt \cdot \onevec{\Mtx} \label{eq:gtx} \\
%\grxtgt = \Grxtgt \cdot \onevec{\Mrx} \label{eq:grx}
%\end{align}
Let $\Atx \in \setmatrixcomplex{\Nt}{\Mtx}$ be the matrix of transmit array response vectors evaluated at the directions in $\dirtxset$, and let $\Arx \in \setmatrixcomplex{\Nr}{\Mrx}$ be defined analogously. %  evaluated at the directions in $\dirrxset$.
\begin{align}
\Atx &= 
\begin{bmatrix}
\atx{\dirtx\idx{1}} & \atx{\dirtx\idx{2}} & \cdots & \atx{\dirtx\idx{\Mtx}}
\end{bmatrix} \\
\Arx &= 
\begin{bmatrix}
\arx{\dirrx\idx{1}} & \arx{\dirrx\idx{2}} & \cdots & \arx{\dirrx\idx{\Mrx}}
\end{bmatrix}
\end{align}
Recall, these can be computed directly based on the transmit and receive array geometries \cite{heath_lozano,balanis}.
Using these, the expressions of \eqref{eq:sigma-tx} can be written equivalently (up to arbitrary phase shifts of $\vf_i$ and $\vw_j$) as follows, which we refer to as \textit{coverage constraints}.
\begin{align}
\normtwo{\Nt\cdot \vone - \diag{\Atx\ctrans \precbmat}}^2 &\leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \label{eq:coverage-constraint-tx} \\
\normtwo{\Nr\cdot \vone - \diag{\Arx\ctrans \comcbmat}}^2 &\leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \label{eq:coverage-constraint-rx}
\end{align}
Note that the $(i,i)$-th entry of $\Atx\ctrans \precbmat$ has magnitude $\Gtx\parens{\dirtx\idx{i}}$ and the $(j,j)$-th entry of $\Arx\ctrans \comcbmat$ has magnitude $\Grx\parens{\dirrx\idx{j}}$.
By satisfying \eqref{eq:coverage-constraint-tx} and \eqref{eq:coverage-constraint-rx}, engineers can ensure that \lonestar codebooks adequately serve their coverage regions for appropriately chosen $\sigmatx^2$ and $\sigmarx^2$.
% By satisfying \eqref{eq:coverage-constraint-tx} and \eqref{eq:coverage-constraint-rx}, engineers can ensure that codebooks produced by \lonestar adequately serve their coverage regions for appropriately chosen $\sigmatx^2$ and $\sigmarx^2$.
% Note that these two constraints capture the gain and coverage constraints of our two codebooks $\prerfcbbar$ and $\comrfcbbar$.

%\begin{definition}[Target self-interference level]
%Suppose the system aims to satisfy a target average receive link \ginr denoted $\inrrxthresh$.
%In other words, we desire $\inrrxavg \leq \inrrxthresh$.
%This target may be based on BLANK.
%Our design does not guarantee that this target is met but does not incentivize the design to reduce self-interference below this threshold.
%Nonetheless, engineers can choose $\inrrxthresh = -\infty$ dB if they wish for the design to truly minimize $\inrrxavg$.
%\end{definition}

With coverage constraints \eqref{eq:coverage-constraint-tx} and \eqref{eq:coverage-constraint-rx}, we now formulate an analog beamforming codebook design in problem \eqref{eq:problem-desired-i}.
The goal of \lonestar is to design transmit and receive codebooks that minimize the self-interference coupled between each transmit and receive beam pair while ensuring the codebooks remain useful in delivering service to users.
% In problem \eqref{eq:problem-desired-i} below, we formulate an optimization problem that designs transmit and receive codebooks to achieve this.
% minimize the average self-interference coupled across all transmit-receive beam pairs while 
% We begin by formulating problem \eqref{eq:problem-desired-i}, which aims to minimize the average self-interference coupled across all transmit-receive beam pairs.
\begin{subequations} \label{eq:problem-desired-i}
\begin{align}
\min_{\mF,\mW} \ & \ \normfro{\mW\ctrans \mH \mF}^2 \\
\st 
& \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \label{eq:constraint-cov-tx} \\
& \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \label{eq:constraint-cov-rx} \\
& \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:constraint-tx-limited} \\
& \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:constraint-rx-limited}
\end{align}
\end{subequations}
% \begin{subequations} \label{eq:problem-desired-i}
% \begin{align}
% \min_{\mF,\mW} \ & \ \normfro{\mW\ctrans \parens{\mHbar + \mDelta} \mF}^2 \\
% \st \ 
% & \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
% & \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
% & \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:constraint-tx-limited} \\
% & \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:constraint-rx-limited}
% \end{align}
% \end{subequations}
By minimizing the Frobenius norm in the objective, our designed codebooks aim to minimize the average self-interference coupled across all transmit-receive beam pairs as evident in \eqref{eq:inr-rx-avg}.
While doing so, our codebooks must satisfy the coverage constraints \eqref{eq:constraint-cov-tx} and \eqref{eq:constraint-cov-rx} that were established in \eqref{eq:coverage-constraint-tx} and \eqref{eq:coverage-constraint-rx}.
Constraints \eqref{eq:constraint-tx-limited} and \eqref{eq:constraint-rx-limited} require our design to create codebooks whose beams are physically realizable with digitally controlled phase shifters and attenuators. %  present in our analog beamforming networks.

Practical systems cannot solve problem \eqref{eq:problem-desired-i} since they do not have knowledge of the true self-interference channel $\mH$ but rather the estimate $\mHbar$.
% naturally do not have knowledge of the error matrix $\mDelta$.
% Without knowledge of the error $\mDelta$, solving problem \eqref{eq:problem-desired-i} is impossible.
% With some estimate $\mHbar$, the true channel $\mH$ is distributed based on \eqref{eq:channel}. %  and \eqref{eq:channel-error}.
This motivates us to modify problem \eqref{eq:problem-desired-i} to incorporate robustness to channel estimation error.
It is common in robust communication system optimization to minimize the worst-case error inflicted by some uncertainty \cite{cvx_boyd,convex_beamforming_2010,palomar_robust_2006,palomar_robust_2008,palomar_robust_2009}.
In our case, $\mDelta$ has \iid Gaussian entries, meaning the worst-case error inflicted on the objective of problem \eqref{eq:problem-desired-i} is unbounded.
In light of this, we instead minimize the expectation of our objective over the distribution of $\mH$.
% To account for this channel uncertainty, 
% We adjust our design as follows to minimize the expected average self-interference coupled between beam pairs in the face of channel estimation error $\mDelta$.
Forming problem \eqref{eq:problem-desired-ii}, \lonestar aims to minimize the \textit{expected} average self-interference coupled between beam pairs, given some estimate $\mHbar$. %  and distribution of its estimation error.
% We desire a solution that aims to minimize the expected coupling for a given channel estimate $\mHbar$ and distribution of its estimation error.
\begin{subequations} \label{eq:problem-desired-ii}
\begin{align}
% \min_{\mF,\mW} \ & \ \expect_{\mH,\mDelta} \brackets{\normfro{\mW\ctrans \parens{\mH + \mDelta} \mF}^2 \ \vert \ \mHbar} \\
\min_{\mF,\mW} \ & \ \expect_{\mH} \brackets{\normfro{\mW\ctrans \mH \mF}^2 \ \vert \ \mHbar} \label{eq:problem-desired-ii-obj} \\
\st 
& \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
& \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
& \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \\
& \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx
\end{align}
\end{subequations}
To transform problem \eqref{eq:problem-desired-ii} into one we can more readily solve, we derive a closed-form expression of the objective \eqref{eq:problem-desired-ii-obj}, courtesy of the fact that $\mDelta$ is Gaussian.
%Thus, we can transform the objective of \eqref{eq:problem-desired-ii} as the expectation over $\mDelta$ as follows.
%\begin{subequations} \label{eq:problem-desired-iii}
%    \begin{align}
%    % \min_{\mF,\mW} \ & \ \expect_{\mH,\mDelta} \brackets{\normfro{\mW\ctrans \parens{\mH + \mDelta} \mF}^2 \ \vert \ \mHbar} \\
%    \min_{\mF,\mW} \ & \ \expect_{\mDelta} \brackets{\normfro{\mW\ctrans \parens{\mHbar + \mDelta} \mF}^2} \\
%    \st \ 
%    & \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
%    & \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
%    & \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \\
%    & \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx
%    \end{align}
%\end{subequations}


%\begin{theorem} \label{thm:objective-expectation}
%    % For a matrix $\mDelta$ whose entries are \iid Gaussian with zero-mean and variance $\epsilon^2$,
%    The objective of problem \eqref{eq:problem-desired-ii} is equivalent to
%    \begin{align}
%    \expect_{\mH,\mDelta} \brackets{\normfro{\mW\ctrans \parens{\mH + \mDelta} \mF}^2 \ \vert \ \mHbar} 
%    = 
%    \normfro{\mW\ctrans \mHbar \mF}^2 + 2 \cdot \epsilon^2 \cdot \normfro{\mW}^2 \cdot \normfro{\mF}^2.
%    \end{align}
%    \begin{proof}
%        Recall, $\mH = \mHbar + \mDelta$ where $\mDelta$ has entries \iid Gaussian with mean zero and variance $\eps^2$.
%        As such, taking expectation over the true channel $\mH$ conditioning on its estimate $\mHbar$ is equivalent to taking expectation over the estimation error $\mDelta$.
%        This allows us to write
%        \begin{align}
%        \expect_{\mH,\mDelta} \brackets{\normfro{\mW\ctrans \parens{\mH + \mDelta} \mF}^2 \ \vert \ \mHbar}
%        =& \expect_{\mDelta_1,\mDelta_2} \brackets{\normfro{\mW\ctrans \parens{\mHbar + \mDelta_1 + \mDelta_2} \mF}^2}
%        \end{align}
%        where $\mDelta_1$ captures the error in $\mHbar$ from $\mH$ and $\mDelta_2$ captures 
%        We leverage the linearity of trace and expectation, the cyclic property of trace, the unitary (rotational) invariance of \iid zero-mean Gaussian matrices, the fact that $\ev{\mDelta} = \mZero$, and the fact that $\normfro{\mX}^2 = \trace{\mX\mX\ctrans}$.
%        \begin{align}
%        & \expect_{\mH,\mDelta} \brackets{\normfro{\mW\ctrans \parens{\mH + \mDelta} \mF}^2 \ \vert \ \mHbar} \\
%        =& \expect_{\mDelta_1,\mDelta_2} \brackets{\normfro{\mW\ctrans \parens{\mHbar + \mDelta_1 + \mDelta_2} \mF}^2} \\
%        =& \expect_{\hat\mDelta} \brackets{\normfro{\mW\ctrans \parens{\mHbar + \hat\mDelta} \mF}^2} \\
%        =& \expect_{\hat\mDelta} \brackets{\normfro{\mW\ctrans \mHbar \mF + \mW\ctrans \hat\mDelta \mF}^2} \\
%        =& \expect_{\hat\mDelta} \brackets{\trace{\parens{\mW\ctrans \mHbar \mF + \mW\ctrans \hat\mDelta \mF} \parens{\mW\ctrans \mHbar \mF + \mW\ctrans \hat\mDelta \mF}\ctrans}} \\
%        % =& \expect_{\mDelta} \brackets{\trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} + \trace{\mW\ctrans \mDelta \mF \mF\ctrans \mDelta\ctrans \mW} + \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mDelta\ctrans \mW} + \trace{\mW\ctrans \mDelta \mF \mF\ctrans \mHbar\ctrans \mW}} \\
%        % =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} + \expect_{\mDelta} \brackets{\trace{\mW\ctrans \mDelta \mF \mF\ctrans \mDelta\ctrans \mW} + \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mDelta\ctrans \mW} + \trace{\mW\ctrans \mDelta \mF \mF\ctrans \mHbar\ctrans \mW}} \\
%        % =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} + \expect_{\mDelta} \brackets{\trace{\mW\ctrans \mDelta \mF \mF\ctrans \mDelta\ctrans \mW}} + \expect_{\mDelta} \brackets{\trace{\mW\ctrans \mHbar \mF \mF\ctrans \mDelta\ctrans \mW}} + \expect_{\mDelta} \brackets{\trace{\mW\ctrans \mDelta \mF \mF\ctrans \mHbar\ctrans \mW}} \\
%        % =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} + \expect_{\mDelta} \brackets{\trace{\mF\ctrans \mDelta\ctrans \mW \mW\ctrans \mDelta \mF}} + \expect_{\mDelta} \brackets{\trace{\mF\ctrans \mDelta\ctrans \mW \mW\ctrans \mHbar \mF}} + \expect_{\mDelta} \brackets{\trace{\mF\ctrans \mHbar\ctrans \mW \mW\ctrans \mDelta \mF}} \\
%        % =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%        % + \trace{\expect_{\mDelta} \brackets{\mF\ctrans \mDelta\ctrans \mW \mW\ctrans \mDelta \mF}} 
%        % + \trace{\expect_{\mDelta} \brackets{\mF\ctrans \mDelta\ctrans \mW \mW\ctrans \mHbar \mF}}
%        % + \trace{\expect_{\mDelta} \brackets{\mF\ctrans \mHbar\ctrans \mW \mW\ctrans \mDelta \mF}} \\
%        =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%        + \trace{\mF\ctrans \expect_{\hat\mDelta} \brackets{\hat\mDelta\ctrans \mW \mW\ctrans \hat\mDelta} \mF} \nonumber \\
%        &+ \trace{\mF\ctrans \expect_{\hat\mDelta} \brackets{\hat\mDelta\ctrans} \mW \mW\ctrans \mHbar \mF}
%        + \trace{\mF\ctrans \mHbar\ctrans \mW \mW\ctrans \expect_{\hat\mDelta} \brackets{\hat\mDelta} \mF} \\
%        =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%        + \trace{\mF\ctrans \expect_{\hat\mDelta} \brackets{\hat\mDelta\ctrans \mW \mW\ctrans \hat\mDelta} \mF} \\
%        =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%        + \trace{\mF\ctrans \expect_{\hat\mDelta} \brackets{\hat\mDelta\ctrans \mU_{\mW} \mLambda_{\mW} \mU_{\mW}\ctrans \hat\mDelta} \mF} \\
%        =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%        + \trace{\mF\ctrans \expect_{\tilde\mDelta = \hat\mDelta\ctrans \mU_{\mW}} \brackets{\tilde\mDelta \mLambda_{\mW} \tilde\mDelta\ctrans} \mF} \\
%        % =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%        % + \trace{\mF\ctrans \trace{\epsilon^2 \cdot \mLambda_{\mW}} \mI \mF} \\
%        =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%        + 2 \cdot \epsilon^2 \cdot \trace{\mF\ctrans \mF} \cdot \trace{\mLambda_{\mW}} \\
%        =& \ \normfro{\mW\ctrans \mHbar \mF}^2 + 2 \cdot \epsilon^2 \cdot \normfro{\mF}^2 \cdot \normfro{\mW}^2
%        \end{align}
%        using the linearity of trace and expectation, cyclic property of trace, unitary (rotational) invariance of \iid zero-mean Gaussian matrices \cite{heath_lozano}, the fact that $\ev{\mDelta} = \mZero$, and \cite{gupta_matrix}
%        \begin{align}
%        \expect_{\mX} \brackets{\mX \mA \mX\ctrans} = \alpha^2 \cdot \trace{\mA\ctrans} \cdot \mI
%        \end{align}
%        where $\mX$ has entries \iid Gaussian with mean $0$ and variance $\alpha^2$.
%    \end{proof}
%\end{theorem}

\begin{theorem} \label{thm:objective-expectation}
    % For a matrix $\mDelta$ whose entries are \iid Gaussian with zero-mean and variance $\epsilon^2$, the objective of problem \eqref{eq:problem-desired-ii} 
    The objective of problem \eqref{eq:problem-desired-ii}
    % \begin{align}
    % \expect_{\mH} \brackets{\normfro{\mW\ctrans \mH \mF}^2 \ \vert \ \mHbar}
    % \end{align}
    is equivalent to
    \begin{align}
    % \expect_{\mDelta} \brackets{\normfro{\mW\ctrans \parens{\mHbar + \mDelta} \mF}^2} 
    % = 
    \expect_{\mH} \brackets{\normfro{\mW\ctrans \mH \mF}^2 \ \vert \ \mHbar} =
    \normfro{\mW\ctrans \mHbar \mF}^2 + \epsilon^2 \cdot \normfro{\mF}^2 \cdot \normfro{\mW}^2.
    \end{align}
    \begin{proof}
        % Recalling \eqref{eq:channel}, we begin by rewriting the objective as
        % \begin{align}
        % \expect_{\mH} \brackets{\normfro{\mW\ctrans \mH \mF}^2 \ \vert \ \mHbar}
        % =
        % \expect_{\mDelta} \brackets{\normfro{\mW\ctrans \parens{\mHbar + \mDelta} \mF}^2}.
        % \end{align}
        % Then, we can write
        We begin by recalling \eqref{eq:channel} to write
        \begin{align}
        \expect_{\mH} \brackets{\normfro{\mW\ctrans \mH \mF}^2 \ \vert \ \mHbar}
        =& \
        \expect_{\mDelta} \brackets{\normfro{\mW\ctrans \parens{\mHbar + \mDelta} \mF}^2} \\
        % =& \expect_{\mDelta} \brackets{\normfro{\mW\ctrans \mHbar \mF + \mW\ctrans \mDelta \mF}^2} \\
        \overset{\textrm{(a)}}{=}& \ \expect_{\mDelta} \brackets{\trace{\parens{\mW\ctrans \parens{\mHbar + \mDelta} \mF} \parens{\mW\ctrans \parens{\mHbar + \mDelta} \mF}\ctrans}} \\
        % =& \expect_{\mDelta} \brackets{\trace{\parens{\mW\ctrans \mHbar \mF + \mW\ctrans \mDelta \mF} \parens{\mW\ctrans \mHbar \mF + \mW\ctrans \mDelta \mF}\ctrans}} \\
        \overset{\textrm{(b)}}{=}& \ \normfro{\mW\ctrans \mHbar \mF}^2 + \trace{\mF\ctrans \expect_{\mDelta} \brackets{\mDelta\ctrans \mW \mW\ctrans \mDelta} \mF} \\
        % \overset{\mathrm{(b)}}{=}& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} + \trace{\mF\ctrans \expect_{\mDelta} \brackets{\mDelta\ctrans \mW \mW\ctrans \mDelta} \mF} \\
        % &+ \trace{\mF\ctrans \expect_{\mDelta} \brackets{\mDelta\ctrans} \mW \mW\ctrans \mHbar \mF} \nonumber \\
        % &+ \trace{\mF\ctrans \mHbar\ctrans \mW \mW\ctrans \expect_{\mDelta} \brackets{\mDelta} \mF} \\
        % \overset{\mathrm{(c)}}{=}& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
        % + \trace{\mF\ctrans \expect_{\mDelta} \brackets{\mDelta\ctrans \mW \mW\ctrans \mDelta} \mF} \\
        \overset{\textrm{(c)}}{=}& \ \normfro{\mW\ctrans \mHbar \mF}^2 + \trace{\mF\ctrans \expect_{\mDelta} \brackets{\mDelta\ctrans \mU_{\mW} \mLambda_{\mW} \mU_{\mW}\ctrans \mDelta} \mF} \\
        \overset{\textrm{(d)}}{=}& \ \normfro{\mW\ctrans \mHbar \mF}^2 + \trace{\mF\ctrans \expect_{\tilde\mDelta} \brackets{\tilde\mDelta \mLambda_{\mW} \tilde\mDelta\ctrans} \mF} \\
        \overset{\textrm{(e)}}{=}& \ \normfro{\mW\ctrans \mHbar \mF}^2 + \trace{\mF\ctrans \mF} \cdot \epsilon^2 \cdot \trace{\mLambda_{\mW}} \\
        \overset{\textrm{(f)}}{=}& \ \normfro{\mW\ctrans \mHbar \mF}^2 + \epsilon^2 \cdot \normfro{\mF}^2 \cdot \normfro{\mW}^2
        \end{align}
        where (a) follows from $\normfro{\mA}^2 = \trace{\mA\mA\ctrans}$; (b) is by the linearity of expectation and trace and the fact that $\ev{\mDelta} = \zeromat$; (c) is by taking the  eigenvalue decomposition $\mW\mW\ctrans = \mU_{\mW} \mLambda_{\mW} \mU_{\mW}\ctrans$; (d) is by defining $\tilde\mDelta = \mDelta\ctrans \mU_{\mW}$, which has the same distribution as $\mDelta$ by unitary invariance of \iid zero-mean Gaussian matrices \cite{heath_lozano}; (e) is via the property \cite{gupta_matrix}
        \begin{align}
        \expect_{\mX} \brackets{\mX \mA \mX\ctrans} = \epsilon^2 \cdot \trace{\mA\ctrans} \cdot \mI
        \end{align}
        where $\mX$ has entries \iid Gaussian with mean $0$ and variance $\epsilon^2$; and (f) follows from the definition of Frobenius norm.
    \end{proof}
\end{theorem}

%\begin{proof}
%    We begin by leveraging the fact that $\normfro{\mA}^2 = \trace{\mA\mA\ctrans}$, along with the linearity of trace and expectation and the cyclic property of trace. We can write
%    \begin{align}
%    \expect_{\mDelta} \brackets{\normfro{\mW\ctrans \parens{\mHbar + \mDelta} \mF}^2}
%    % =& \expect_{\mDelta} \brackets{\normfro{\mW\ctrans \mHbar \mF + \mW\ctrans \mDelta \mF}^2} \\
%    =& \expect_{\mDelta} \brackets{\trace{\parens{\mW\ctrans \mHbar \mF + \mW\ctrans \mDelta \mF} \parens{\mW\ctrans \mHbar \mF + \mW\ctrans \mDelta \mF}\ctrans}} \\
%    =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%    + \trace{\mF\ctrans \expect_{\mDelta} \brackets{\mDelta\ctrans \mW \mW\ctrans \mDelta} \mF} \nonumber \\
%    &+ \trace{\mF\ctrans \expect_{\mDelta} \brackets{\mDelta\ctrans} \mW \mW\ctrans \mHbar \mF}
%    + \trace{\mF\ctrans \mHbar\ctrans \mW \mW\ctrans \expect_{\mDelta} \brackets{\mDelta} \mF} \\
%    =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%    + \trace{\mF\ctrans \expect_{\mDelta} \brackets{\mDelta\ctrans \mW \mW\ctrans \mDelta} \mF}
%    \end{align}
%    where $\ev{\mDelta} = \zeromat$.
%    We take the eigenvalue decomposition $\mW\mW\ctrans = \mU_{\mW} \mLambda_{\mW} \mU_{\mW}\ctrans$
%    % \begin{align}
%    % \mW\mW\ctrans = \mU_{\mW} \mLambda_{\mW} \mU_{\mW}\ctrans
%    % \end{align}
%    to write
%    \begin{align}
%    \expect_{\mDelta} \brackets{\normfro{\mW\ctrans \parens{\mHbar + \mDelta} \mF}^2}
%    =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%    + \trace{\mF\ctrans \expect_{\mDelta} \brackets{\mDelta\ctrans \mU_{\mW} \mLambda_{\mW} \mU_{\mW}\ctrans \mDelta} \mF} \\
%    =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%    + \trace{\mF\ctrans \expect_{\tilde\mDelta} \brackets{\tilde\mDelta \mLambda_{\mW} \tilde\mDelta\ctrans} \mF}
%    \end{align}
%    where $\tilde\mDelta = \mDelta\ctrans \mU_{\mW}$, which has the same distribution as $\mDelta$ by unitary invariance of \iid zero-mean Gaussian matrices \cite{heath_lozano}.
%    Then, we use the property \cite{gupta_matrix}
%    \begin{align}
%    \expect_{\mX} \brackets{\mX \mA \mX\ctrans} = \epsilon^2 \cdot \trace{\mA\ctrans} \cdot \mI
%    \end{align}
%    where $\mX$ has entries \iid Gaussian with mean $0$ and variance $\epsilon^2$.
%    This leads to
%    \begin{align}
%    \expect_{\mDelta} \brackets{\normfro{\mW\ctrans \parens{\mHbar + \mDelta} \mF}^2}
%    =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%    + \trace{\mF\ctrans \mF} \cdot \epsilon^2 \cdot \trace{\mLambda_{\mW}} \\
%    =& \ \normfro{\mW\ctrans \mHbar \mF}^2 + \epsilon^2 \cdot \normfro{\mF}^2 \cdot \normfro{\mW}^2.
%    \end{align}
%\end{proof}

Using \thmref{thm:objective-expectation}, problem \eqref{eq:problem-desired-ii} can be rewritten equivalently as follows in problem \eqref{eq:problem-desired-final}.
% Problem \eqref{eq:problem-desired-final} is parameterized by the estimate $\mHbar$ and the error variance $\eps^2$, abstracting out the error matrix $\mDelta$.
For some channel estimate $\mHbar$ and knowledge of the estimation error variance $\eps^2$, engineers can aim to solve problem \eqref{eq:problem-desired-final} for the codebooks $\mF$ and $\mW$ that minimize the expected average self-interference coupled between transmit and receive beams while ensuring coverage is delivered with some quality parameterized by $\sigmatx^2$ and $\sigmarx^2$.
\begin{subequations} \label{eq:problem-desired-final}
\begin{align}
\min_{\mF,\mW} \ & \ \normfro{\mW\ctrans \mHbar \mF}^2 + \epsilon^2 \cdot \normfro{\mF}^2 \cdot \normfro{\mW}^2 \\
\st  
& \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
& \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
& \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \\
& \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx
\end{align}
\end{subequations}
This concludes the formulation of our codebook design problem.
In the next section, we present a means to solve problem \eqref{eq:problem-desired-final}, along with a summary of and commentary on \lonestar.
% This is non-convex due to limited phase and amplitude control of the analog beamforming networks.
% It is also difficult to solve this jointly in $\mF$ and $\mW$. We take advantage of the fact that the objective is separably convex in $\mF$ and $\mW$.


%\begin{subequations} \label{eq:problem-desired-i}
%    \begin{align}
%    \min_{\mF,\mW} \ & \ \normfro{\mW\ctrans \mH \mF}^2 \\
%    \st \ 
%    & \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
%    & \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
%    & \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \\
%    & \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx
%    \end{align}
%\end{subequations}

%With $\mDelta$ Gaussian, we can rewrite the objective in a closed form that depends only on its variance.
%\begin{theorem}
%    For a matrix $\mDelta$ with entries Gaussian with zero-mean and variance $\epsilon^2$, the objective of BLANK is equivalent to
%    \begin{align}
%    \expect_{\mDelta} \brackets{\normfro{\mW\ctrans \parens{\mHbar + \mDelta} \mF}^2} 
%    = 
%    \normfro{\mW\ctrans \mHbar \mF}^2 + \epsilon^2 \cdot \normfro{\mW}^2 \cdot \normfro{\mF}^2
%    \end{align}
%    \begin{proof}
%        \footnotesize
%        \begin{align}
%        & \expect_{\mDelta} \brackets{\normfro{\mW\ctrans \parens{\mHbar + \mDelta} \mF}^2} \\
%        =& \expect_{\mDelta} \brackets{\normfro{\mW\ctrans \mHbar \mF + \mW\ctrans \mDelta \mF}^2} \\
%        =& \expect_{\mDelta} \brackets{\trace{\parens{\mW\ctrans \mHbar \mF + \mW\ctrans \mDelta \mF} \parens{\mW\ctrans \mHbar \mF + \mW\ctrans \mDelta \mF}\ctrans}} \\
%        =& \expect_{\mDelta} \brackets{\trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} + \trace{\mW\ctrans \mDelta \mF \mF\ctrans \mDelta\ctrans \mW} + \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mDelta\ctrans \mW} + \trace{\mW\ctrans \mDelta \mF \mF\ctrans \mHbar\ctrans \mW}} \\
%        =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} + \expect_{\mDelta} \brackets{\trace{\mW\ctrans \mDelta \mF \mF\ctrans \mDelta\ctrans \mW} + \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mDelta\ctrans \mW} + \trace{\mW\ctrans \mDelta \mF \mF\ctrans \mHbar\ctrans \mW}} \\
%        =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} + \expect_{\mDelta} \brackets{\trace{\mW\ctrans \mDelta \mF \mF\ctrans \mDelta\ctrans \mW}} + \expect_{\mDelta} \brackets{\trace{\mW\ctrans \mHbar \mF \mF\ctrans \mDelta\ctrans \mW}} + \expect_{\mDelta} \brackets{\trace{\mW\ctrans \mDelta \mF \mF\ctrans \mHbar\ctrans \mW}} \\
%        =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} + \expect_{\mDelta} \brackets{\trace{\mF\ctrans \mDelta\ctrans \mW \mW\ctrans \mDelta \mF}} + \expect_{\mDelta} \brackets{\trace{\mF\ctrans \mDelta\ctrans \mW \mW\ctrans \mHbar \mF}} + \expect_{\mDelta} \brackets{\trace{\mF\ctrans \mHbar\ctrans \mW \mW\ctrans \mDelta \mF}} \\
%        =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%        + \trace{\expect_{\mDelta} \brackets{\mF\ctrans \mDelta\ctrans \mW \mW\ctrans \mDelta \mF}} 
%        + \trace{\expect_{\mDelta} \brackets{\mF\ctrans \mDelta\ctrans \mW \mW\ctrans \mHbar \mF}}
%        + \trace{\expect_{\mDelta} \brackets{\mF\ctrans \mHbar\ctrans \mW \mW\ctrans \mDelta \mF}} \\
%        =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%        + \trace{\mF\ctrans \expect_{\mDelta} \brackets{\mDelta\ctrans \mW \mW\ctrans \mDelta} \mF} 
%        + \trace{\mF\ctrans \expect_{\mDelta} \brackets{\mDelta\ctrans} \mW \mW\ctrans \mHbar \mF}
%        + \trace{\mF\ctrans \mHbar\ctrans \mW \mW\ctrans \expect_{\mDelta} \brackets{\mDelta} \mF} \\
%        =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%        + \trace{\mF\ctrans \expect_{\mDelta} \brackets{\mDelta\ctrans \mW \mW\ctrans \mDelta} \mF} \\
%        =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%        + \trace{\mF\ctrans \expect_{\mDelta} \brackets{\mDelta\ctrans \mU_{\mW} \mLambda_{\mW} \mU_{\mW}\ctrans \mDelta} \mF} \\
%        =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%        + \trace{\mF\ctrans \expect_{\tilde\mDelta = \mDelta\ctrans \mU_{\mW}} \brackets{\tilde\mDelta \mLambda_{\mW} \tilde\mDelta\ctrans} \mF} \\
%        =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%        + \trace{\mF\ctrans \trace{\epsilon^2 \cdot \mLambda_{\mW}} \mF} \\
%        =& \ \trace{\mW\ctrans \mHbar \mF \mF\ctrans \mHbar\ctrans \mW} 
%        + \trace{\mF\ctrans \mF} \cdot \epsilon^2 \cdot \trace{\mLambda_{\mW}} \\
%        =& \ \normfro{\mW\ctrans \mHbar \mF}^2 + \epsilon^2 \cdot \normfro{\mF}^2 \cdot \normfro{\mW}^2
%        \end{align}
%        using the linearity of trace and expectation, cyclic property of trace, unitary (rotational) invariance of \iid zero-mean Gaussian matrices, the fact that $\ev{\mDelta} = \mZero$ and \cite{gupta_matrix,heath_lozano}
%        \begin{align}
%        \expect_{\mX} \brackets{\mX \mA \mX\ctrans} = \epsilon^2 \cdot \trace{\mA\ctrans}
%        \end{align}
%        where $\mX$ has Gaussian entries with mean $0$ and variance $\epsilon^2$.
%    \end{proof}
%\end{theorem}


==> sec-contribution-ii.tex <==
\section{Solving for Our Design and Summarizing Remarks} \label{sec:contribution-ii}

We concluded the previous section with problem \eqref{eq:problem-desired-final}, a codebook design problem that accounts for self-interference channel estimation error and digitally controlled phase shifters and attenuators.
In this section, we present an approach for (approximately) solving this design problem using a projected alternating minimization approach.
We conclude this section with a summary of our design and remarks regarding design decisions and future research directions.  

\subsection{Solving for Our Design}
Problem \eqref{eq:problem-desired-final} cannot be efficiently solved directly due to the non-convexity posed by digitally controlled phase shifters and attenuators (i.e., $\precb$ and $\comcb$ are non-convex).
The joint optimization of $\mF$ and $\mW$ introduces further complexity, especially given their dimensionality.
In order to approximately but efficiently solve problem \eqref{eq:problem-desired-final}, we take a projected alternating minimization approach, which is summarized in \algref{alg:algorithm-ii}.
Let $\project{\entry{\mF}{:,i}}{\precb}$ be the projection of the $i$-th beam (column) of $\mF$ onto the set of physically realizable beamforming vectors $\precb$.
We extend this projection onto each beam in $\mF$ as $\project{\mF}{\precb}$ by applying it column-wise on $\mF$; the projection of $\mW$ onto $\comcb$ is defined analogously.
With digitally controlled phase shifters and attenuators, each element of $\mF$ must be quantized in both phase and amplitude.
Since the set of physically realizable beamforming weights is the same for each element in a beamforming vector, the projection of that vector reduces to projecting each of its elements.
The $(m,n)$-th element following the projection of $\mF$ onto $\precb$ can be expressed as
\begin{align} \label{eq:project}
\entry{\project{\mF}{\precb}}{m,n} = A\opt \cdot \exp\parens{\j \cdot \theta\opt}
\end{align}
where $A\opt$ and $\theta\opt$ are the quantized amplitude and phase of $\entry{\mF}{m,n}$.
These can be expressed as
\begin{align}
A\opt &= \argmin_{A_i \in \set{A}} \ \bars{A_i - A}, \qquad
\theta\opt = \argmin_{\theta_i \in \set{P}} \ \bars{\exp\parens{\j \cdot \theta_i} - \exp\parens{\j \cdot \theta}}
\end{align}
where $A = \bars{\entry{\mF}{m,n}}$ and $\theta = \angleop{\entry{\mF}{m,n}}$ are the magnitude and phase of $\entry{\mF}{m,n}$.
%where $A$ and $\theta$ are the magnitude and phase of $\entry{\mF}{m,n}$.
%\begin{align}
%A &= \bars{\entry{\mF}{m,n}}, \qquad
%\theta = \angleop{\entry{\mF}{m,n}}
%% \theta = \tan\inv\parens{\frac{\realpart{\entry{\mF}{m,n}}}{\imagpart{\entry{\mF}{m,n}}}}
%\end{align}
Here, $\set{A}$ and $\set{P}$ are the sets of physically realizable amplitudes (attenuator settings) and phases (phase shifter settings), respectively.
For instance, with attenuators having a fixed step size of $\delta$ dB per \gls{lsb} (which is common in practice \cite{ibm_array_2017}) and phase shifters having phase control uniformly distributed over $[0,2\pi)$, these sets can be expressed as
\begin{align}
\set{A} &= \braces{A_i = 10^{-\delta \cdot (i-1) / 20} : i = 1, \dots, 2^\bitsamp} \\
\set{P} &= \braces{\theta_i = \frac{(i-1) \cdot 2 \pi}{2^\bitsphase} - \pi : i = 1, \dots, 2^\bitsphase}
\end{align}
where $\bitsamp$ and $\bitsphase$ are the resolutions (in bits) of each attenuator and phase shifter, respectively.

%
%---
%
%When using phase shifters with phase control uniformly distributed with over $[0,2\pi)$ with $\bitsphase$ bits of resolution, we can write $\theta\opt$ as
%\begin{align}
%\theta\opt 
%&= \argmin_{\theta_i \in \set{P}} \ \bars{\exp\parens{\j \cdot \theta_i} - \exp\parens{\j \cdot \theta}}
%\end{align}
%where $\theta = \angleop{\entry{\mF}{i,j}}$ and
%\begin{align}
%\set{P} 
%&= \braces{\theta_i = \frac{(i-1) \cdot 2 \pi}{2^\bitsphase} - \pi : i = 1, \dots, 2^\bitsphase} .
%\end{align}
%With attenuators with a fixed step size of $\delta$ dB per \gls{lsb} (starting at $0$ dB), the quantized amplitude can be expressed similarly as
%\begin{align}
%A\opt &= \argmin_{A_i \in \set{A}} \ \bars{A_i - A}
%\end{align}
%where $A = \bars{\entry{\mF}{i,j}}$ and the set of all realizable amplitudes $\set{A}$ is
%\begin{align}
%\set{A} 
%&= \braces{A_i = 10^{-\delta \cdot (i-1) / 20} : i = 1, \dots, 2^\bitsamp}.
%\end{align}

To approximately solve problem \eqref{eq:problem-desired-final}, we begin with $\precbmat \leftarrow \project{\Atx}{\precb}$ and $\comcbmat \leftarrow \project{\Arx}{\comcb}$, % , quantizing their entries to have phase and amplitude resolutions $\bitsphase$ and $\bitsamp$.
% To approximately solve problem \eqref{eq:problem-desired-final}, our algorithm begins by initializing $\precbmat$ and $\comcbmat$ as the projections of $\Atx$ and $\Arx$ onto $\precb$ and $\comcb$ using \eqref{eq:project}. % , quantizing their entries to have phase and amplitude resolutions $\bitsphase$ and $\bitsamp$.
% That is, $\precbmat \leftarrow \project{\Atx}{\precb}$ and $\comcbmat \leftarrow \project{\Arx}{\comcb}$, 
%\begin{gather}
%\precbmat \leftarrow \project{\Atx}{\precb} \label{eq:init-F}, \qquad 
%\comcbmat \leftarrow \project{\Arx}{\comcb} % \label{eq:init-W}
%\end{gather}
which initializes our beams as matched filters to achieve (near) maximum gains across $\dirtxset$ and $\dirrxset$, respectively.
Then, we fix the receive codebook $\comcbmat$ and solve problem \eqref{eq:problem-am-F} below.
\begin{subequations} \label{eq:problem-am-F}
    \begin{align}
    \min_{\mF} \ & \ \normfro{\mW\ctrans \mHbar \mF}^2 + \epsilon^2 \cdot \normfro{\mF}^2 \cdot \normfro{\mW}^2 \\
    \st 
    & \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
    & \ \bars{\entry{\mF}{i,j}} \leq 1, \ i = 1, \dots, \Nt, \ j = 1, \dots, \Mtx \label{eq:problem-unit-entry-F}
    \end{align}
\end{subequations}
As a temporary convex relaxation, we have introduced constraint \eqref{eq:problem-unit-entry-F} instead of requiring strict quantized phase and amplitude control.
This enforces that each beamforming weight not exceed unit magnitude, understood by the fact that attenuators are used for amplitude control as outlined in \eqref{eq:unit-f-w}.
% This enforces that each beamforming weight must not exceed unit magnitude, understood by the fact that attenuators are used for amplitude control (as opposed to amplifiers).
Problem \eqref{eq:problem-am-F} is convex and can be readily solved using convex optimization solvers (e.g., we used \cite{cvx}).
Dedicated algorithms more efficient than general solvers can likely be developed for \lonestar, but that is beyond the scope of this work, making it a good topic for future work.
%\begin{gather}
%\bars{\entry{\vf}{m}} \leq 1 \ \forall \ m = 1, \dots, \Nt \\
%\bars{\entry{\vw}{n}} \leq 1 \ \forall \ n = 1, \dots, \Nr
%\end{gather}
%understood by the fact that attenuators are used for amplitude control.
% s that to ensure our beamforming weights can be implemented using attenuators (as opposed to amplifiers).
% In other words, each beamforming weight must not exceed unit magnitude, 
After solving problem \eqref{eq:problem-am-F}, the solution $\mF\opt$ is projected onto the set $\precb$ before setting it as $\precbmat$ to ensure it is physically realizable.
\begin{align}
\precbmat \leftarrow \project{\mF\opt}{\precb}
\end{align}
The projected $\precbmat$ is then used when solving for the receive codebook in problem \eqref{eq:problem-am-W} below.
\begin{subequations} \label{eq:problem-am-W}
\begin{align}
\min_{\mW} \ & \ \normfro{\mW\ctrans \mHbar \mF}^2 + \epsilon^2 \cdot \normfro{\mF}^2 \cdot \normfro{\mW}^2 \\
\st 
& \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
& \ \bars{\entry{\mW}{i,j}} \leq 1, \ i = 1, \dots, \Nr, \ j = 1, \dots, \Mrx
\end{align}
\end{subequations}
Problem \eqref{eq:problem-am-W} has a form identical to problem \eqref{eq:problem-am-F} and is thus convex and can be solved using the same approach used for problem \eqref{eq:problem-am-F}.
Upon solving problem \eqref{eq:problem-am-W}, we ensure the solution $\mW\opt$ is physically realizable by projecting it onto $\comcb$. %  before updating $\comcbmat$.
\begin{align}
\comcbmat \leftarrow \project{\mW\opt}{\comcb}
\end{align}
This concludes our design of \lonestar, which has produced physically realizable transmit and receive codebook matrices $\precbmat$ and $\comcbmat$.
These can then be unpacked via \eqref{eq:unpack-1} and \eqref{eq:unpack-2} to form the sets $\precbbar$ and $\comcbbar$ that can be used for beam alignment and subsequent full-duplexing of downlink and uplink. % with reduced self-interference.
In the next section, we evaluate \lonestar extensively through simulation.


%In our approach, we use alternating minimization to approximately solve problem \eqref{eq:problem-desired-final} by solving for the transmit codebook then the receive codebook. 
%We separate problem problem \eqref{eq:problem-desired-final} into problems \eqref{eq:problem-am-F} and \eqref{eq:problem-am-W} below, which solve for the transmit codebook and receive codebook, respectively.
%Problems \eqref{eq:problem-am-F} and \eqref{eq:problem-am-W} are convex since they remove the hardware constraints and can be readily solved using a convex solver (e.g., we used \cite{cvx}).
%% We solve for the $i$-th transmit beam $\vf_i$ in problem \eqref{eq:problem-full-4a}, starting with $i=1$ and the initialized $\comcbmat$.
%Note that we have introduced the constraint \eqref{eq:problem-entry-tx-4a} to ensure our beamforming weights can be implemented using attenuators.

%Define projection operator, for example, when phase shifters are quantized uniformly and attenuators are quantized log-uniformly, we have
%\begin{align}
%\entry{\project{\mF}{\precb}}{i,j} = A\opt \cdot \exp\parens{\j \cdot \theta\opt}
%\end{align}
%where $\vartheta = \angleop{\entry{\mF}{i,j}} \in [0,2\pi)$.
%\begin{align}
%A &=  \frac{1}{2^\bitsphase - 1} \cdot \floor{\frac{\vartheta \cdot 2^\bitsphase}{2\pi} + \frac{1}{2}} \\
%\theta &= \frac{2\pi}{2^\bitsphase} \cdot \floor{\frac{\vartheta \cdot 2^\bitsphase}{2\pi} + \frac{1}{2}}
%\end{align}

%\begin{align}
%\set{P} 
%&= \braces{\theta_i = \frac{(i-1) \cdot 2 \pi}{2^\bitsphase} - \pi : i = 1, \dots, 2^\bitsphase} \\
%\set{A}_{\mathrm{dB}} 
%&= \braces{-\delta/2 \cdot (i-1): i = 1, \dots, 2^\bitsamp} \\
%\set{A} 
%&= \braces{A_i = 10^{-\delta \cdot (i-1) / 20} : i = 1, \dots, 2^\bitsamp}
%\end{align}

%\begin{align}
%\theta\opt 
%&= \argmin_{\theta_i \in \set{P}} \ \bars{\exp\parens{\j \cdot \theta_i} - \exp\parens{\j \cdot \theta}} \\
%A\opt 
%&= \argmin_{A_i \in \set{A}} \ \bars{A_i - A}
%\end{align}

\input{alg/algorithm-ii.tex}

\begin{remark}[Complexity]
    It is difficult to comment on the complexity of our design for a few reasons.
    First and foremost, its complexity depends heavily on the solver used for solving problems \eqref{eq:problem-am-F} and \eqref{eq:problem-am-W}.
    As mentioned, more efficient solving algorithms may be tailored for \lonestar, but that is out of the scope of this work.
    Additionally, total computational costs will depend on the initialization of $\mF$ and $\mW$.
    We have initialized them both as conjugate beamforming codebooks; in practice, it would likely be efficient to use previous solutions of $\mF$ and $\mW$ when rerunning \lonestar to account for drift in the self-interference channel.
    Note that our design takes place at the full-duplex \bs, which presumably has sufficient compute resources to execute \lonestar.
    Practically, it may be preferred to conduct a thorough estimation of $\mH$ and execution of \lonestar during initial setup of the \bs and then perform updates to the estimate of $\mH$ and possibly to our design over time; this would be interesting future work.
    % Complexity depends on what $\precb$ and $\comcb$ are initialized to.
    % Why use projection alternating minimization.
    % Difficult to address the joint optimization of $\mF$ and $\mW$.
    % Also difficult to optimize over the non-convex set, due to number of antennas and resolutions. Even for low resolution phase shifters and attenuators, the size of the set is very large.
    % Also many beams.
    Most existing beamforming-based full-duplex solutions need to be executed for each downlink-uplink user pair, whereas the same \lonestar design can be used across many user pairs, meaning it may offer significant computational savings in comparison. % , meaning its complexity/overhead scales with the coherence time of the self-interference channel.
\end{remark}

\subsection{Design Summary and Remarks}

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth,height=0.5\textheight,keepaspectratio]{fig/lonestar_block_type_01}
%    \caption{A block diagram describing \lonestar.}
%    \label{fig:block}
%\end{figure}

% Block diagram of how design works.
% Algorithm of entire design.
% Solving algorithm.

A summary of \lonestar is outlined in \algref{alg:algorithm-i}.
\lonestar begins by obtaining an estimate $\mHbar$ of the self-interference \mimo channel and knowledge of the channel estimation error variance $\eps^2$.
Then, the transmit and receive coverage regions $\txdirsetcb$ and $\rxdirsetcb$ are defined by system engineers, and the array response matrices $\Atx$ and $\Arx$ are assembled based on the transmit and receive array geometries.
Engineers specify the tolerated transmit and receive coverage variances $\sigmatx^2$ and $\sigmarx^2$, and \lonestar codebook matrices $\mF$ and $\mW$ are designed by solving problem \eqref{eq:problem-desired-final} using \algref{alg:algorithm-ii}.
The codebooks $\precbbar$ and $\comcbbar$ are formed by unpacking $\mF$ and $\mW$.
The \bs then uses $\precbbar$ and $\comcbbar$ for beam alignment and full-duplexing of downlink and uplink over several time slots before rerunning \lonestar to account for drift in the self-interference channel.

\begin{remark}[Design decisions]
    We now present a few remarks on our approach and communicate our motivations and design decisions.
    The objective of \lonestar is to create transmit and receive codebooks that minimize the average $\inrrx$ while still delivering high transmit and receive beamforming gain.
    It may seem preferred to maximize the average $\sinrrx$ or the sum spectral efficiency, but this requires knowledge of the transmit and receive \gpsnr, which the system only has \textit{after} conducting beam alignment, or real-time knowledge of $\vhtx$ and $\vhrx$, which is currently impractical.
    \lonestar only relies on knowledge of the self-interference \mimo channel and not that of the transmit and receive channels.
    By minimizing $\inrrx$ while constraining transmit and receive coverage quality (i.e., maintaining high $\snrtx$ and $\snrrx$), \lonestar can consequently achieve high $\sinrrx$ and $\sinrtx$.
    % Why minimize INR, not include SNR.
    % Why not minimize the maximum INR instead of minimzing the average.
    One may also suggest we instead minimize the maximum $\inrrx$ (to minimize worst-case self-interference) rather than minimize the average $\inrrx$.
    We chose to minimize the average $\inrrx$ because this prevents \lonestar from being significantly hindered if there are select transmit-receive beam pairs that simply cannot offer low self-interference while delivering high beamforming gain.
    It is important to note that the Frobenius norm objective used by \lonestar will be more incentivized to reduce high self-interference but does not exclusively prioritize these worst-case beam pairs \cite{cvx_boyd}.
    Individual beam pairs that do not yield sufficiently low $\inrrx$ when minimizing the average $\inrrx$ with \lonestar could potentially be avoided via scheduling or half-duplexed as a last resort.
\end{remark}

\input{alg/algorithm-i.tex}

\begin{remark}[Future directions]
We now outline future research directions particularly relevant to \lonestar.
Extensive study and modeling of \mmwave self-interference channels and their coherence time will be important to understanding the potentials of \lonestar---and full-duplex \mmwave systems in general---along with developing efficient means for self-interference channel estimation.
Also, methods to dynamically update \lonestar as the self-interference channel changes would be valuable future work, along with implementations of \lonestar using real \mmwave platforms.
Naturally, there are some ways to improve upon this work, such as by better handling limited phase and amplitude control and by creating efficient, dedicated solvers for \lonestar.
Beyond \lonestar, measurement-driven beamforming-based full-duplex solutions (potentially using machine learning) that do not require self-interference \mimo channel knowledge (e.g., \steer \cite{roberts_steer}) would be excellent contributions to the research community.
% Studying self-interference channel, modeling, coherence time of self-interference channel, ways to tackle this problem with no self-interference channel knowledge (measurement-based), self-interference channel estimation. Efficient algorithms for solving this problem, along with updating it with changes in the self-interference channel. Prototyping and implementation of \lonestar and other full-duplex solutions.
% Potential to create a joint codebook instead of two independent transmit-receive codebooks (optimization would take longer and would require more memory but would naturally yield better performance; similar to STEER).
% Can improve with better handling of quantization (e.g., could quantize row-by-row in F, W and iterate through each row so that each iteration accounts for quantization, or use soft quantization via penalty).
\end{remark}


\comment{
---

\begin{align}
\min_{\mF,\mW} \ & \ \maxop{\frac{\powertxbs \cdot G^2}{\powernoisebs} \cdot \frac{\normfro{\mW\ctrans \mH \mF}^2}{\Mtx \cdot \Mrx},\inrrxthresh} \\
\st \ 
& \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
& \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
& \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \\
& \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx
\end{align}


\begin{align}
\gamma = \sqrt{\frac{\inrrxthresh \cdot \Mtx \cdot \Mrx \cdot \powernoisebs}{\powertxbs \cdot G^2}}
\end{align}

\begin{subequations} \label{eq:problem-iii}
    \begin{align}
    \min_{\mF,\mW} \ & \ \maxop{\normfro{\mW\ctrans \mH \mF},\gamma} \\
    \st \ 
    & \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
    & \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
    & \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-1} \\
    & \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-1}
    \end{align}
\end{subequations}


\begin{subequations} \label{eq:problem-iii}
    \begin{align}
    \min_{\mF,\mW} \ & \ \maxop{\normfro{\mW\ctrans \parens{\mHbar + \mDelta} \mF},\gamma} \\
    \st \ 
    & \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
    & \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
    & \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-1} \\
    & \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-1}
    \end{align}
\end{subequations}


\begin{subequations} \label{eq:problem-iii}
    \begin{align}
    \min_{\mF,\mW} \ & \ \maxop{\max_{\mDelta} \ \normfro{\mW\ctrans \parens{\mHbar + \mDelta} \mF},\gamma} \\
    \st \ 
    & \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
    & \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
    & \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-1} \\
    & \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-1} \\
    & \ \normfro{\mDelta}^2 \leq \eps^2 \cdot \Nt \cdot \Nr
    \end{align}
\end{subequations}


\begin{subequations} \label{eq:problem-iii}
    \begin{align}
    % \min_{\mF,\mW} \ & \ \maxop{\normfro{\mW\ctrans \mHbar \mF} + \eps \cdot \sqrt{\Nt \cdot \Nr} \cdot \svmax{\mW} \cdot \svmax{\mF},\gamma} \\
    \min_{\mF,\mW} \ & \ \maxop{\normfro{\mW\ctrans \mHbar \mF} + \eps \cdot \svmax{\mW} \cdot \svmax{\mF},\gamma} \\
    \st \ 
    & \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
    & \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
    & \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-1} \\
    & \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-1}
    \end{align}
\end{subequations}

---

\begin{align}
\Nt^2 \cdot \Nr^2 = \max_{\vf,\vw,\mH} \ & \ \bars{\vw\ctrans \mH \vf}^2 \\
\st \ 
& \ \normfro{\mH}^2 = \Nt \cdot \Nr \\
& \ \normtwo{\vf}^2 = \Nt \\
& \ \normtwo{\vw}^2 = \Nr
\end{align}

\begin{align}
\svmaxsq{\mH} \cdot \Nt \cdot \Nr = \max_{\vf,\vw} \ & \ \bars{\vw\ctrans \mH \vf}^2 \\
\st \ 
& \ \normtwo{\vf}^2 = \Nt \\
& \ \normtwo{\vw}^2 = \Nr
\end{align}

So max \ginr is 
\begin{align}
\inrrxbar = \frac{\powertxbs \cdot G^2 \cdot \Nt^2 \cdot \Nr^2}{\powernoisebs} \geq \inrrx
\end{align}

INR target $\inrrxthresh$
\begin{align}
\inrrxthresh = \frac{\powertxbs \cdot G^2 \cdot \gamma}{\powernoisebs}
\end{align}

The average \ginr coupled across all beam pairs is
\begin{align}
\frac{\powertxbs \cdot G^2}{\powernoisebs} \cdot \frac{\normfro{\mW\ctrans \mH \mF}^2}{\Mtx \cdot \Mrx}
\end{align}

We aim to minimize the average \ginr coupled across all beam pairs but do not incentivize it to reduce such below some target $\inrrxthresh$.
\begin{subequations} \label{eq:problem-i}
    \begin{align}
    \min_{\mF,\mW} \ & \ \maxop{\frac{\powertxbs \cdot G^2}{\powernoisebs} \cdot \frac{\normfro{\mW\ctrans \mH \mF}^2}{\Mtx \cdot \Mrx},\inrrxthresh} \\
    \st \ 
    & \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
    & \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
    & \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-1} \\
    & \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-1}
    \end{align}
\end{subequations}

\begin{subequations} \label{eq:problem-ii}
\begin{align}
\min_{\mF,\mW} \ & \ \maxop{\frac{\powertxbs \cdot G^2}{\powernoisebs} \cdot \frac{\normfro{\mW\ctrans \parens{\mHbar + \mDelta} \mF}^2}{\Mtx \cdot \Mrx},\inrrxthresh} \\
\st \ 
& \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
& \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
& \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-1} \\
& \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-1}
\end{align}
\end{subequations}


Minimize the worst-case average \ginr caused by channel estimation error.
\begin{subequations} \label{eq:problem-ii}
    \begin{align}
    \min_{\mF,\mW} \ & \ \maxop{\max_{\mDelta} \frac{\powertxbs \cdot G^2}{\powernoisebs} \cdot \frac{\normfro{\mW\ctrans \parens{\mHbar + \mDelta} \mF}^2}{\Mtx \cdot \Mrx},\inrrxthresh} \\
    \st \ 
    & \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
    & \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
    & \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-1} \\
    & \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-1} \\
    & \ \normfro{\mDelta}^2 \leq \eps^2 \cdot \Nt \cdot \Nr
    \end{align}
\end{subequations}

\begin{align}
\max_{\normfro{\mDelta}^2 \leq \eps^2} \ \normfro{\mW\ctrans \parens{\mHbar + \sqrt{\Nt \cdot \Nr} \cdot \mDelta} \mF}
&= \max_{\normfro{\mDelta}^2 \leq \eps^2} \ \normfro{\mW\ctrans \mHbar \mF + \sqrt{\Nt \cdot \Nr} \cdot \mW\ctrans \mDelta \mF} \\
&= \normfro{\mW\ctrans \mHbar \mF} + \sqrt{\Nt \cdot \Nr} \cdot \eps \cdot \svmax{\mW} \cdot \svmax{\mF}
\end{align}




\begin{subequations} \label{eq:problem-iii}
    \begin{align}
    \min_{\mF,\mW} \ & \ \maxop{\normfro{\mW\ctrans \mHbar \mF} + \eps \cdot \sqrt{\Nt \cdot \Nr} \cdot \svmax{\mW} \cdot \svmax{\mF},\gamma} \\
    \st \ 
    & \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
    & \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
    & \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-1} \\
    & \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-1}
    \end{align}
\end{subequations}








\section{Extra}

\begin{align}
\min_{\mF,\mW} \ & \ \maxop{\normfro{\mW\ctrans \mH \mF}^2,\gamma} \\
\st \ 
& \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
& \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
& \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \\
& \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx
\end{align}
}



==> sec-contribution.tex <==
\section{Analog Beamforming Codebook Design} \label{sec:contribution}

The goal of our design is to produce a codebook of transmit beams $\precbbar$ and a codebook of receive beams $\comcbbar$ with objectives twofold:
\begin{enumerate}
    \item The codebooks contain transmit and receive beams that deliver high beamforming gain and collectively provide broad coverage.
    \item Each transmit-receive beam pair couples low self-interference.
\end{enumerate}
We outline our methodology by first quantifying our design criteria and then assembling our codebook design problem.
In the next section, we present an algorithm for solving our codebook design problem.

\subsection{Quantifying Our Codebook Design Criteria}

\begin{definition}[Transmit and receive coverage regions]
Let $\dirtxset$ be a set of $\Mtx$ directions---or a \textit{transmit coverage region}---that our transmit codebook $\precbbar$ aims to serve, and let $\dirtxset$ be a set of $\Mrx$ receive directions---or a \textit{receive coverage region}---that our receive codebook $\comcbbar$ aims to serve.
\begin{gather}
\dirtxset = \braces{\dirtx\idx{i} : i = 1, \dots, \Mtx} \\
\dirrxset = \braces{\dirrx\idx{j} : j = 1, \dots, \Mrx}
\end{gather}
For example, $\dirtxset$ and $\dirrxset$ may be comprised of $\Mtx = \Mrx$ beams uniformly distributed over $-60^\circ$ to $60^\circ$ in azimuth and $-30^\circ$ to $30^\circ$ in elevation. % , each with $10^\circ$ steps.
Note that $\dirtx$ and $\dirrx$ each may capture both azimuthal and elevational steering direction.
\end{definition}

%Let $\Atx \in \setmatrixcomplex{\Nt}{\Mtx}$ be the matrix of transmit array response vectors evaluated at the directions in $\dirtxset$, and let $\Arx \in \setmatrixcomplex{\Nr}{\Mrx}$ be the matrix of receive array response vectors evaluated at the directions in $\dirrxset$.
%\begin{align}
%\Atx &= 
%\begin{bmatrix}
%\atx{\dirtx\idx{1}} & \atx{\dirtx\idx{2}} & \cdots & \atx{\dirtx\idx{\Mtx}}
%\end{bmatrix}  \\
%\Arx &= 
%\begin{bmatrix}
%\arx{\dirrx\idx{1}} & \arx{\dirrx\idx{2}} & \cdots & \arx{\dirrx\idx{\Mrx}}
%\end{bmatrix}
%\end{align}
We index the $\Mtx$ beams in $\precbbar$ and the $\Mrx$ beams in $\comcbbar$ according to $\dirtxset$ and $\dirrxset$, respectively, as % $\precbbar = \braces{\vf_1, \dots, \vf_{\Mtx}}$ and $\comcbbar = \braces{\vw_1, \dots, \vw_{\Mrx}}$, 
\begin{gather}
\precbbar = \braces{\vf_1, \dots, \vf_{\Mtx}} \\
\comcbbar = \braces{\vw_1, \dots, \vw_{\Mrx}}
\end{gather}
where $\vf_i \in \precb$ is responsible for transmitting toward $\dirtx\idx{i}$ and $\vw_j \in \comcb$ is responsible for receiving from $\dirrx\idx{j}$.\footnote{Recall, physically realizable $\vf$ and $\vw$ are fundamentally required to come from $\precb$ and $\comcb$, capturing digitally controlled phase shifters and attenuators.}
Using this notation, we build the codebook matrix $\precbmat$ by stacking transmit beams $\vf_i$ as follows and the codebook matrix $\comcbmat$ analogously.
\begin{gather}
\precbmat = 
\begin{bmatrix}
\vf_1 & \vf_2 & \cdots & \vf_{\Mtx}
\end{bmatrix} \in \setmatrixcomplex{\Nt}{\Mtx} \\
\comcbmat = 
\begin{bmatrix}
\vw_1 & \vw_2 & \cdots & \vw_{\Mrx}
\end{bmatrix} \in \setmatrixcomplex{\Nr}{\Mrx}
\end{gather}

\begin{definition}[Average self-interference coupled]
The coupling between the $i$-th transmit beam $\vf_i$ and the $j$-th receive beam $\vw_j$ can be captured by the product $\vw_j\ctrans \mH \vf_i$, which can be extended to all beam pairs as $\comcbmat\ctrans \mH \precbmat \in \setmatrixcomplex{\Mrx}{\Mtx}$.
Our design aims to minimize the average \ginr coupled between beam pairs, which can be written as
\begin{align}
\inrrxavg 
&= \frac{1}{\Mtx \cdot \Mrx} \cdot \sum_{i=1}^{\Mtx} \sum_{j=1}^{\Mrx}  \frac{\powertxbs \cdot G^2 \cdot \bars{\vw_j\ctrans \mH \vf_i}^2}{\powernoisebs} \\
&= \frac{\powertxbs \cdot G^2}{\powernoisebs} \cdot \frac{\normfro{\mW\ctrans \mH \mF}^2}{\Mtx \cdot \Mrx}.
\end{align}
In our design's attempt to minimize $\inrrxavg$, we must also ensure that the beams in $\precbmat$ and $\comcbmat$ remain useful in serving users within the coverage region; of course, unconstrained, $\precbmat$ and $\comcbmat$ minimize $\inrrxavg$ when driven to $\zeromat$.
We now quantify a means to constrain our design to ensure it can maintain service in its minimization of $\inrrxavg$.
\end{definition}

\begin{definition}[Transmit and receive gain]
Let $\Gtx^2\parens{\dirtx\idx{i}}$ be the transmit power gain afforded by $\vf_i$ in the direction of $\dirtx\idx{i}$ and $\Grx^2\parens{\dirrx\idx{j}}$ be the receive power gain afforded by $\vw_j$ in the direction of $\dirrx\idx{j}$, expressed as
\begin{align}
\Gtx^2\parens{\dirtx\idx{i}} &= \bars{\atx{\dirtx\idx{i}}\ctrans  \vf_i}^2 \leq \Nt^2 \label{eq:Gtx} \\
\Grx^2\parens{\dirrx\idx{j}} &= \bars{\arx{\dirrx\idx{j}}\ctrans  \vw_j}^2 \leq \Nr^2 \label{eq:Grx}.
\end{align}
The transmit and receive gain are upper-bounded by $\Nt^2$ and $\Nr^2$, respectively, by virtue of normalizations presented in our system model. 
This gain can be achieved toward any $\dir$ with $\vf = \atx{\dir}$ and $\vw = \arx{\dir}$, respectively, often referred to as conjugate beamforming or matched filter beamforming.
\end{definition}

\begin{definition}[Transmit and receive gain variance]
To offer our design flexibility in reducing $\inrrxavg$, we tolerate some loss in beamforming gain toward our desired directions; in other words, we allow for some beamforming gain less than $\Nt^2$ and $\Nr^2$ in exchange for improved self-interference rejection, as we will see.
Let $\sigmatx^2 \geq 0$ be the maximum variance tolerated in achieving maximum transmit gain\footnote{We use magnitude here, which is simply the square root of power gain.} across beams in the transmit codebook $\precbbar$, normalized to $\Nt^2$.
Defining $\sigmarx^2 \geq 0$ analogously, we have
\begin{gather}
\frac{1}{\Mtx} \cdot \sum_{i=1}^{\Mtx} \frac{\bars{\Nt - \Gtx\parens{\dirtx\idx{i}}}^2}{\Nt^2} \leq \sigmatx^2 \label{eq:sigma-tx} \\
\frac{1}{\Mrx} \cdot \sum_{j=1}^{\Mrx} \frac{\bars{\Nr - \Grx\parens{\dirrx\idx{j}}}^2}{\Nr^2} \leq \sigmarx^2  \label{eq:sigma-rx}.
\end{gather}
Here, $\sigmatx^2$ and $\sigmarx^2$ are design parameters that can be chosen by system engineers; increasing them will offer our design greater flexibility in reducing $\inrrxavg$ but may degrade coverage.
% More variance across transmit and receive gain provided by our beams may increase the disparity of service seen across users but would also allow our design more flexibility in its attempt to reduce self-interference.
\end{definition}


\subsection{Assembling Our Codebook Design Problem}
With expressions for our codebook design criteria in hand, we now turn our attention to assembling a formal design problem.
% Let $\gtxtgt = \Gtxtgt \cdot \onevec{\Mtx}$ and $\grxtgt = \Grxtgt \cdot \onevec{\Mrx}$ be vectors containing the target transmit and receive gains at each entry.
%\begin{align}
%\gtxtgt = \Gtxtgt \cdot \onevec{\Mtx} \label{eq:gtx} \\
%\grxtgt = \Grxtgt \cdot \onevec{\Mrx} \label{eq:grx}
%\end{align}
Let $\Atx \in \setmatrixcomplex{\Nt}{\Mtx}$ be the matrix of transmit array response vectors evaluated at the directions in $\dirtxset$, and let $\Arx \in \setmatrixcomplex{\Nr}{\Mrx}$ be the matrix of receive array response vectors evaluated at the directions in $\dirrxset$.
\begin{align}
\Atx &= 
\begin{bmatrix}
\atx{\dirtx\idx{1}} & \atx{\dirtx\idx{2}} & \cdots & \atx{\dirtx\idx{\Mtx}}
\end{bmatrix}  \\
\Arx &= 
\begin{bmatrix}
\arx{\dirrx\idx{1}} & \arx{\dirrx\idx{2}} & \cdots & \arx{\dirrx\idx{\Mrx}}
\end{bmatrix}
\end{align}
Using this, the expressions of \eqref{eq:sigma-tx} and \eqref{eq:sigma-rx} can be written equivalently (up to an arbitrary phase shift of $\vf_i$ or $\vw_j$) as follows, which we refer to as our \textit{coverage constraints},
\begin{align}
\normtwo{\Nt\cdot \vone - \diag{\Atx\ctrans \precbmat}}^2 &\leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \label{eq:coverage-constraint-tx} \\
\normtwo{\Nr\cdot \vone - \diag{\Arx\ctrans \comcbmat}}^2 &\leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \label{eq:coverage-constraint-rx}.
\end{align}
Note that the $(i,i)$-th entry of $\Atx\ctrans \precbmat$ has magnitude $\Gtx\parens{\dirtx\idx{i}}$ and the $(j,j)$-th entry of $\Arx\ctrans \comcbmat$ has magnitude $\Grx\parens{\dirrx\idx{j}}$.
By satisfying \eqref{eq:coverage-constraint-tx} and \eqref{eq:coverage-constraint-rx}, we can ensure that our codebooks $\precbbar$ and $\comcbbar$ adequately serve our coverage regions for appropriately chosen $\sigmatx^2$ and $\sigmarx^2$.
% Note that these two constraints capture the gain and coverage constraints of our two codebooks $\prerfcbbar$ and $\comrfcbbar$.

\begin{definition}[Target self-interference level]
Suppose the system aims to satisfy a target average receive link \ginr denoted $\inrrxthresh$.
In other words, we desire $\inrrxavg \leq \inrrxthresh$.
This target may be based on BLANK.
Our design does not guarantee that this target is met but does not incentivize the design to reduce self-interference below this threshold.
Nonetheless, engineers can choose $\inrrxthresh = -\infty$ dB if they wish for the design to truly minimize $\inrrxavg$.
\end{definition}


We now formulate the follow analog beamforming codebook design problem.
\begin{align}
\min_{\mF,\mW} \ & \ \maxop{\frac{\powertxbs \cdot G^2}{\powernoisebs} \cdot \frac{\normfro{\mW\ctrans \mH \mF}^2}{\Mtx \cdot \Mrx},\inrrxthresh} \\
\st \ 
& \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
& \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
& \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \\
& \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx
\end{align}


\begin{align}
\gamma = \sqrt{\frac{\inrrxthresh \cdot \Mtx \cdot \Mrx \cdot \powernoisebs}{\powertxbs \cdot G^2}}
\end{align}

\begin{subequations} \label{eq:problem-iii}
    \begin{align}
    \min_{\mF,\mW} \ & \ \maxop{\normfro{\mW\ctrans \mH \mF},\gamma} \\
    \st \ 
    & \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
    & \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
    & \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-1} \\
    & \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-1}
    \end{align}
\end{subequations}


\begin{subequations} \label{eq:problem-iii}
    \begin{align}
    \min_{\mF,\mW} \ & \ \maxop{\normfro{\mW\ctrans \parens{\mHbar + \mDelta} \mF},\gamma} \\
    \st \ 
    & \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
    & \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
    & \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-1} \\
    & \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-1}
    \end{align}
\end{subequations}


\begin{subequations} \label{eq:problem-iii}
    \begin{align}
    \min_{\mF,\mW} \ & \ \maxop{\max_{\mDelta} \ \normfro{\mW\ctrans \parens{\mHbar + \mDelta} \mF},\gamma} \\
    \st \ 
    & \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
    & \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
    & \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-1} \\
    & \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-1} \\
    & \ \normfro{\mDelta}^2 \leq \eps^2 \cdot \Nt \cdot \Nr
    \end{align}
\end{subequations}


\begin{subequations} \label{eq:problem-iii}
    \begin{align}
    % \min_{\mF,\mW} \ & \ \maxop{\normfro{\mW\ctrans \mHbar \mF} + \eps \cdot \sqrt{\Nt \cdot \Nr} \cdot \svmax{\mW} \cdot \svmax{\mF},\gamma} \\
    \min_{\mF,\mW} \ & \ \maxop{\normfro{\mW\ctrans \mHbar \mF} + \eps \cdot \svmax{\mW} \cdot \svmax{\mF},\gamma} \\
    \st \ 
    & \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
    & \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
    & \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-1} \\
    & \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-1}
    \end{align}
\end{subequations}

---

\begin{align}
\Nt^2 \cdot \Nr^2 = \max_{\vf,\vw,\mH} \ & \ \bars{\vw\ctrans \mH \vf}^2 \\
\st \ 
& \ \normfro{\mH}^2 = \Nt \cdot \Nr \\
& \ \normtwo{\vf}^2 = \Nt \\
& \ \normtwo{\vw}^2 = \Nr
\end{align}

\begin{align}
\svmaxsq{\mH} \cdot \Nt \cdot \Nr = \max_{\vf,\vw} \ & \ \bars{\vw\ctrans \mH \vf}^2 \\
\st \ 
& \ \normtwo{\vf}^2 = \Nt \\
& \ \normtwo{\vw}^2 = \Nr
\end{align}

So max \ginr is 
\begin{align}
\inrrxbar = \frac{\powertxbs \cdot G^2 \cdot \Nt^2 \cdot \Nr^2}{\powernoisebs} \geq \inrrx
\end{align}

INR target $\inrrxthresh$
\begin{align}
\inrrxthresh = \frac{\powertxbs \cdot G^2 \cdot \gamma}{\powernoisebs}
\end{align}

The average \ginr coupled across all beam pairs is
\begin{align}
\frac{\powertxbs \cdot G^2}{\powernoisebs} \cdot \frac{\normfro{\mW\ctrans \mH \mF}^2}{\Mtx \cdot \Mrx}
\end{align}

We aim to minimize the average \ginr coupled across all beam pairs but do not incentivize it to reduce such below some target $\inrrxthresh$.
\begin{subequations} \label{eq:problem-i}
    \begin{align}
    \min_{\mF,\mW} \ & \ \maxop{\frac{\powertxbs \cdot G^2}{\powernoisebs} \cdot \frac{\normfro{\mW\ctrans \mH \mF}^2}{\Mtx \cdot \Mrx},\inrrxthresh} \\
    \st \ 
    & \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
    & \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
    & \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-1} \\
    & \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-1}
    \end{align}
\end{subequations}

\begin{subequations} \label{eq:problem-ii}
\begin{align}
\min_{\mF,\mW} \ & \ \maxop{\frac{\powertxbs \cdot G^2}{\powernoisebs} \cdot \frac{\normfro{\mW\ctrans \parens{\mHbar + \mDelta} \mF}^2}{\Mtx \cdot \Mrx},\inrrxthresh} \\
\st \ 
& \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
& \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
& \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-1} \\
& \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-1}
\end{align}
\end{subequations}


Minimize the worst-case average \ginr caused by channel estimation error.
\begin{subequations} \label{eq:problem-ii}
    \begin{align}
    \min_{\mF,\mW} \ & \ \maxop{\max_{\mDelta} \frac{\powertxbs \cdot G^2}{\powernoisebs} \cdot \frac{\normfro{\mW\ctrans \parens{\mHbar + \mDelta} \mF}^2}{\Mtx \cdot \Mrx},\inrrxthresh} \\
    \st \ 
    & \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
    & \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
    & \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-1} \\
    & \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-1} \\
    & \ \normfro{\mDelta}^2 \leq \eps^2 \cdot \Nt \cdot \Nr
    \end{align}
\end{subequations}

\begin{align}
\max_{\normfro{\mDelta}^2 \leq \eps^2} \ \normfro{\mW\ctrans \parens{\mHbar + \sqrt{\Nt \cdot \Nr} \cdot \mDelta} \mF}
&= \max_{\normfro{\mDelta}^2 \leq \eps^2} \ \normfro{\mW\ctrans \mHbar \mF + \sqrt{\Nt \cdot \Nr} \cdot \mW\ctrans \mDelta \mF} \\
&= \normfro{\mW\ctrans \mHbar \mF} + \sqrt{\Nt \cdot \Nr} \cdot \eps \cdot \svmax{\mW} \cdot \svmax{\mF}
\end{align}




\begin{subequations} \label{eq:problem-iii}
    \begin{align}
    \min_{\mF,\mW} \ & \ \maxop{\normfro{\mW\ctrans \mHbar \mF} + \eps \cdot \sqrt{\Nt \cdot \Nr} \cdot \svmax{\mW} \cdot \svmax{\mF},\gamma} \\
    \st \ 
    & \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
    & \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
    & \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-1} \\
    & \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-1}
    \end{align}
\end{subequations}



\subsection{Summary and Algorithm}

Block diagram of how design works.

Algorithm of entire design.

Solving algorithm.

\input{alg/algorithm-i.tex}




\section{Extra}

\begin{align}
\min_{\mF,\mW} \ & \ \maxop{\normfro{\mW\ctrans \mH \mF}^2,\gamma} \\
\st \ 
& \ \normtwo{\Nt\cdot\vone - \diag{\Atx\ctrans\mF}}^2 \leq \sigmatx^2 \cdot \Nt^2 \cdot \Mtx \\
& \ \normtwo{\Nr\cdot\vone - \diag{\Arx\ctrans\mW}}^2 \leq \sigmarx^2 \cdot \Nr^2 \cdot \Mrx \\
& \ \entry{\mF}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \\
& \ \entry{\mW}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx
\end{align}



==> sec-evaluation-i.tex <==
\section{Small-Scale Evaluation} \label{sec:evaluation-i}

Realized CDF of one (i,j) compared to measured CDF of its neighborhood.

Delta med, Delta mean, Delta var/std.

Let $\setinrijreal$ be a set of $\numreal$ realizations of $\inrijreal$, written as
\begin{align}
\setinrijreal = \braces{\inrijreal\idx{n} \sim \distgauss{\muijest}{\varijest} : n = 1,\dots,\numreal}
\end{align}
which represents an measured 

We can compare $\setinrijreal$ to its measured counterpart as 

\begin{align}
% \deltarange\parens{\LLij,\LLijest} &= \rangeop{\todB{\LLij}} - \rangeop{\todB{\LLijest}} \\
\deltamed\parens{\setinrij,\setinrijreal} &= \medop{\todB{\LLij}} - \medop{\todB{\LLijest}} \\
\deltamean\parens{\LLij,\LLijest} &= \meanop{\todB{\LLij}} - \meanop{\todB{\LLijest}} \\
% \deltamax\parens{\LLij,\LLijest} &= \maxop{\todB{\LLij}} - \maxop{\todB{\LLijest}} \\
% \deltamin\parens{\LLij,\LLijest} &= \minop{\todB{\LLij}} - \minop{\todB{\LLijest}} \\
\deltastd\parens{\LLij,\LLijest} &= \stdop{\todB{\LLij}} - \stdop{\todB{\LLijest}} % \\
% \deltavar\parens{\LLij,\LLijest} &= \varop{\todB{\LLij}} - \varop{\todB{\LLijest}}
\end{align}

==> sec-evaluation.tex <==
\section{Evaluating our Model of mmWave Self-Interference} \label{sec:evaluation}



==> sec-keywords.tex <==
\begin{IEEEkeywords}
Full-duplex, self-interference, phased arrays, channel modeling, measurements, millimeter wave.
\end{IEEEkeywords}

==> sec-modeling.tex <==
\section{Spatial and Statistical Modeling of mmWave Self-Interference} \label{sec:modeling}

In this section, we present our model of self-interference for multi-panel full-duplex \mmwave systems.
Our method is relatively simple, has theoretical foundations, and is built on system and model parameters having real-world meaning.
% captures the statistical and spatial characteristics of our measurements,
Naturally, we cannot guarantee that our model---nor the measurements it is based on---will perfectly translate to other systems. 
% Our hope is that it can be generalized to systems beyond our own, however, through appropriate parameterization. %  of our model.
We conjecture that it can be generalized to systems beyond our own, however, through appropriate parameterization, which we show in \secref{sec:remarks}.
% Together, the hope is that this will allow our model to better generalize to other multi-panel full-duplex \mmwave systems beyond our own through appropriate parameterization.
% Naturally, our model is constructed based on our measurements, meaning it is unclear how well it will extend to other systems. 
% We have, however, made multiple efforts to help facilitate such by creating a model built on system parameters such as \gls{eirp} and noise power, along with model parameters having physical meaning. %  and whose parameters are based on system values or can be attributed to underlying physical meaning.
% We have, however, made multiple efforts to help facilitate such by creating a model with sensible foundations built on physical meaning. %  and whose parameters are based on system values or can be attributed to underlying physical meaning.
% Using the approach described herein, engineers can fit our model to their own measurements or can vary model parameters to draw realizations from a variety of self-interference profiles.
% In addition, we have parameterized our model with values that can be adapted to fit other systems based on their \gls{eirp} and noise power and fitted to other measurements of self-interference.
% This allows the same model to be adapted to other systems.
% We present a model that is particular for our setup with the hope that it can extend to other systems/configurations, possibly with slight modifications.
% Naturally, we cannot guarantee that our model, nor the measurements it is based on, will extend to other systems perfectly. 
% Together, the hope is that this will allow our model to better generalize to other multi-panel full-duplex \mmwave systems beyond our own through appropriate parameterization.
At a high level, our model of \mmwave self-interference accomplishes two goals:
\begin{enumerate}
    % \item It captures the spatial and statistical properties of our measurements of self-interference.
    \item It is stochastic, allowing researchers to draw countless realizations of self-interference, rather than a single deterministic quantity.
    % This enables researchers to evaluate solutions broadly over many self-interference profiles and facilitates statistical evaluation of full-duplex systems and networks.
    \item Its realizations align spatially and in distribution with real-world self-interference.
    % This ensures that the levels of realized self-interference incurred by particular beams follow the trends observed in practice and that the variability observed over small spatial neighborhoods is also be captured by our model.
\end{enumerate}
As mentioned in the previous section, the foundation of our model is the seemingly random nature of self-interference across small spatial neighborhoods.
% As mentioned in the previous section, our model is rooted in leveraging the log-normally-distributed nature of self-interference across small spatial neighborhoods.
% This allows engineers to draw realizations of \ginr rather than compute a single deterministic value.
Having fit a log-normal distribution to the neighborhood surrounding each beam pair $(i,j)$, we have nearly 6.5 million fitted mean $\muij$ and variance $\varij$.
In this section, we reverse-engineer a methodology to estimate these fitted parameters $\parens{\muij,\varij}$ based on transmit beam $\vf\thphtxi$ and receive beam $\vw\thphrxj$.
Then, using this estimation methodology, a realization of self-interference for general transmit beam $\vf$ and receive beam $\vw$ can be drawn as
\begin{align}
\todB{\inrreal} \sim \distgauss{\muest}{\varest} \label{eq:realize-inr}
\end{align}
where $\muest$ and $\varest$ are an estimated mean and variance based on $\vf$ and $\vw$. %, along with other system and model parameters. % , the method for doing so we outline in this section.
% In this section, we describe our approach to computing $\muest$ and $\varest$. % for general transmit and receive beams $\vf$ and $\vw$. % , which can then be used to realize self-interference using \eqref{eq:realize-inr}.
% We leverage our nearly 6.5 million measurements to derive and validate such a method for estimating $\muest$ and $\varest$. 
% We will outline our method to compute $\muest$ and $\varest$ for any transmit beam $\vf$ and receive beam $\vw$---conditioned on our measurement platform and configuration---which can then be used to realize $\inr$ using \eqref{eq:realize-inr}.
%Desirably, our method is relatively simple, has theoretical foundations, captures the statistical and spatial characteristics of our measurements, and is parameterized in part by system values.
%Together, the hope is that this will allow our model to better generalize to other multi-panel full-duplex \mmwave systems beyond our own.
% In this section, we outline our methodology for computing the estimates $\muest$ and $\varest$.

% In this section, we outline our methodology for estimating $\muest$ and $\varest$, which is built on the nearly 6.5 million measurements collected in this campaign.

\subsection{Estimating Neighborhood Mean, $\muij$}
% Theoretically, the degree of self-interference experienced by the full-duplex system can be expressed in a closed-form as in \eqref{eq:power-si} and \eqref{eq:power-si-inr}.
% This is not possible, considering the self-interference \mimo channel $\mH$ is unknown.

With nearly 6.5 million true fitted $\muij$, we seek a means to reliably estimate each based on the known transmit and receive beams used during measurement.
% In this section, we will describe our approach to estimating $\muest$ for any transmit and receive beams $\vf$ and $\vw$.
If successful, the same approach can then be used to estimate the mean for general transmit and receive beams.
To estimate the mean $\muij$ for a given transmit-receive pair $(i,j)$, we found that a coarse approximation of the over-the-air self-interference channel between the transmit and receive arrays can be used.
As mentioned in the introduction, the spherical-wave \mimo channel model \cite{spherical_2005}---an idealized near-field model---has been widely used in research on full-duplex \mmwave systems.
However, as we pointed out in our prior work \cite{roberts_att_angular} and illustrate in \figref{fig:azimuth-meas-sim}, this spherical-wave channel model does not align with our measurements of self-interference. % , suggesting that this highly-idealized model is not suitable to describe self-interference in practical full-duplex \mmwave systems.
In light of this, we now propose a different channel model to coarsely describe the spatial composition of self-interference. % from within our measurements that can be used to coarsely describe spatial trends in self-interference.
% In light of this, we instead uncover a different channel model from within our measurements that can be used to coarsely describe spatial trends in self-interference.

\begin{figure*}[!t]
    \centering
    \subfloat[Measured \ginr.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{plots/main_apple_v20_03b.eps}
        \label{fig:azimuth}}
    \quad
    \subfloat[Simulated \ginr with spherical-wave channel \cite{spherical_2005}.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{plots/main_apple_v20_55b.eps}
        \label{fig:azimuth-sim}}
    \caption{(a) Measured \ginr as a function of azimuthal transmit and receive directions when $\phitx = \phirx = 0^\circ$. (b) The simulated counterpart of (a) when using a spherical-wave near-field self-interference channel model \cite{spherical_2005}, which clearly does not align well with what was measured. This motivates the need for a new, measurement-backed model of \mmwave self-interference.}
    \label{fig:azimuth-meas-sim}
\end{figure*}

\textbf{Coarse geometric modeling of the self-interference \mimo channel.} 
% Instead of using the spherical-wave \mimo channel model \cite{spherical_2005}---an idealized near-field model---we uncover a different channel model from within our measurements.
It is practically difficult to obtain precise over-the-air self-interference channel knowledge (i.e., the channel matrix $\mH~\in~\setmatrixcomplex{256}{256}$ shown in \eqref{eq:power-si}) due to its high dimensionality and the fact that it is observed through the lens of the analog beamforming networks in the transmit and receive phased arrays. %  and would require extremely involved electromagnetic propagation simulation of our measurement setup to precisely model.
Fortunately, we have uncovered from our measurements a coarse geometric model of the self-interference channel. %  that captures large-scale spatial trends.
% In other words, 
This model does not capture the significant variability observed {locally} but rather the large-scale spatial components of the self-interference channel.
We now outline this proposed geometric model, which we will use to estimate $\muij$.

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth,height=0.3\textheight,keepaspectratio]{plots/main_apple_v20_03b.eps}
%    \caption{Measured \ginr as a function of azimuthal transmit and receive directions when $\phitx = \phirx = 0^\circ$.}
%    \label{fig:azimuth}
%\end{figure}

%\begin{figure*}
%    \centering
%    \subfloat[Azimuth cut of measured self-interference.]{\includegraphics[width=0.475\linewidth,height=0.27\textheight,keepaspectratio]{plots/main_apple_v20_03b.eps}
%        \label{fig:azimuth}}
%    \qquad\qquad
%    \subfloat[Coupling clusters comprising $\mHbar$.]{\includegraphics[width=0.475\linewidth,height=0.27\textheight,keepaspectratio]{fig/si_model_geometry_type_04}
%        \label{fig:clusters}}
%    \caption{(a) Measured \ginr as a function of azimuthal transmit and receive directions when $\phitx = \phirx = 0^\circ$. (b) An illustration of two coupling clusters comprising the approximate self-interference channel $\mHbar$ between the transmit and receive arrays.}
%    \label{fig:subfigs}
%\end{figure*}




\begin{figure}
    \centering
    \includegraphics[width=\linewidth,height=0.3\textheight,keepaspectratio]{fig/si_model_geometry_type_04}
    \caption{An illustration of two coupling clusters comprising the coarse geometric model of the self-interference channel $\mHbar$ between the transmit and receive arrays.}
    \label{fig:clusters}
\end{figure}


Let us begin by inspecting the azimuth cut of our \ginr measurements (i.e., $\phitx = \phirx = 0^\circ$) plotted in \figref{fig:azimuth}.
% We observe an obvious grid-like structure in the measurements.
From the bright clouds in \figref{fig:azimuth}, we can readily see that there is high self-interference when $(\thetatx,\thetarx)$ is approximately $(0^\circ,-60^\circ)$, $(60^\circ,-60^\circ)$, $(60^\circ,60^\circ)$, and $(-60^\circ,-60^\circ)$.
This hints at which angular components couple high self-interference and paves the way for our proposed geometric model. %  of the self-interference channel.
Rather than model this coupling as single rays extending from the transmit array to the receive array, we instead model them as clouds of rays---or \textit{coupling clusters}---with some non-zero angular spread, as illustrated in \figref{fig:clusters}. 
Suppose $\numclust$ coupling clusters exist between the transmit and receive arrays, where each cluster contains $\numrays$ rays for simplicity.
The center of the $k$-th cluster is defined by some \gls{aod} from the transmit array $\parens{\varthetatx\idx{k},\varphitx\idx{k}}$ and some \gls{aoa} at the receive array $\parens{\varthetarx\idx{k},\varphirx\idx{k}}$.
These cluster centers correspond to the bright clouds identified by visual inspection of \figref{fig:azimuth}.

% Rather than modeling the coupling clusters as single paths We observe that the clusters have some angular spread in azimuth and elevation.
% We observe that the clusters have some angular spread in azimuth and elevation.
% The spread of each coupling cluster in azimuth and elevation 
We assume the angular spread of each cluster is quantified in azimuth and elevation by some $\Delta\vartheta$ and $\Delta\varphi$ and is common across clusters for simplicity.
We use $\set{D}_{\vartheta}$ and $\set{D}_{\varphi}$ defined as
\begin{align}
\set{D}_{\vartheta} &= \braces{-\Delta\vartheta,\dots,0,\dots,+\Delta\vartheta}, \qquad
\set{D}_{\varphi} = \braces{-\Delta\varphi,\dots,0,\dots,+\Delta\varphi}
% \set{D}_{\vartheta} &= \braces{-\Delta\vartheta,\dots,0,\dots,+\Delta\vartheta}, \\
% \set{D}_{\varphi} &= \braces{-\Delta\varphi,\dots,0,\dots,+\Delta\varphi}
\end{align}
to discretize this angular spread into individual rays with some resolution in azimuth and elevation, respectively. 
For instance, discretizing both $\set{D}_{\vartheta}$ and $\set{D}_{\varphi}$ with $1^\circ$ resolution has been sufficient for us.
% The \gls{aod}-\gls{aoa} pairs in $\set{R}$ can be thought of as the centers of the coupling clusters.
We model a coupling cluster as the collection of all \gls{aod}-\gls{aoa} combinations based on the angular spread $\nbrv$.
In this fashion, the \glspl{aod} and \glspl{aoa} of the rays comprising the $k$-th coupling cluster can be expressed as
\begin{align}
\sC_{k} = \bigcup_{\delta \in \set{D}_{\vartheta}} \bigcup_{\lambda \in \set{D}_{\varphi}} \parens{\varthetatx\idx{k} + \delta,\varphitx\idx{k} + \lambda,\varthetarx\idx{k} + \delta,\varphirx\idx{k} + \lambda},
\end{align}
which has cardinality $\card{\sC_k} = \card{\set{D}_{\vartheta}} \cdot \card{\set{D}_{\varphi}} = \numrays$.
% The number of rays per cluster is simply
%\begin{align}
%\card{\sC_i} = \numrays = \card{\set{D}_{\vartheta}} \cdot \card{\set{D}_{\varphi}}.
%\end{align}
The channel matrix produced by the $k$-th cluster can be written as
\begin{align}
%\mHestk &= \sum_{\parens{\varthetatx,\varphitx,\varthetarx,\varphirx} \in \set{C}_{k}} \arx{\varthetarx,\varphirx} \ \atx{\varthetatx,\varphitx}\ctrans, \\
%\mHestk &= \sum_{\varthetatx \in \set{D}_{\varthetatx}\idx{k}} \arx{\varthetarx,\varphirx} \ \atx{\varthetatx,\varphitx}\ctrans,\\
%\mHestk &= \sum_{\varthetatx \in \set{D}_{\varthetatx}\idx{k}}\sum_{\varthetatx \in \set{D}_{\varthetatx}\idx{k}}\sum_{\varthetatx \in \set{D}_{\varthetatx}\idx{k}}\sum_{\varthetatx \in \set{D}_{\varthetatx}\idx{k}} \arx{\varthetarx,\varphirx} \ \atx{\varthetatx,\varphitx}\ctrans, \\
%\mHestk &= \sum_{\parens{\varthetatx,\varphitx} \in \set{D}_{\labeltx}\idx{k}} \sum_{\parens{\varthetarx,\varphirx} \in \set{D}_{\labelrx}\idx{k}} \arx{\varthetarx,\varphirx} \ \atx{\varthetatx,\varphitx}\ctrans,\\
\mHestk &= \sum_{\substack{\parens{\varthetatx,\varphitx} \in \set{D}_{\labeltx}\idx{k}\\\parens{\varthetarx,\varphirx} \in \set{D}_{\labelrx}\idx{k}}} \arx{\varthetarx,\varphirx} \ \atx{\varthetatx,\varphitx}\ctrans,
\end{align}
which is simply the sum of rank-$1$ matrices produced by each of the rays in the cluster; recall, $\atx{\varthetatx,\varphitx}$ and $\arx{\varthetarx,\varphirx}$ are the array responses of the transmit array and receive array for some \gls{aod} and \gls{aoa}, respectively.
As implicitly done here, assuming all rays to have unit gain has proven sufficient for us but this could be generalized straightforwardly. 
The resulting channel matrix comprised of all $\numclust$ coupling clusters is then
\begin{align}
% \mHest = \gamma \cdot \sum_{i=1}^{\numclust} \mHesti
% \mHest = \gamma \cdot \sum_{i=1}^{\numclust} \sum_{\parens{\varthetatx,\varphitx,\varthetarx,\varphirx} \in \set{C}_{i}} \arx{\varthetarx,\varphirx} \ \atx{\varthetatx,\varphitx}\ctrans
% \mHest = \gamma \cdot \sum_{i=1}^{\numclust} \sum_{\delta \in \set{D}_{\vartheta}} \sum_{\nu \in \set{D}_{\varphi}} \arx{\varthetarx+\delta,\varphirx+\nu} \ \atx{\varthetatx+\delta,\varphitx+\nu}\ctrans
% \mHest = \gamma \cdot \sum_{i=1}^{\numclust} \sum_{\parens{\varthetatx,\varthetarx} \in \set{C}_{\vartheta}\idx{i}} \sum_{\parens{\varphitx,\varphirx} \in \set{C}_{\varphi}\idx{i}} \arx{\varthetarx,\varphirx} \ \atx{\varthetatx,\varphitx}\ctrans
\mHest = \sum_{k=1}^{\numclust} \mHestk \cdot \frac{\sqrt{\Nt\cdot\Nr}}{\normfro{\sum_{k=1}^{\numclust} \mHestk}} ,
% \mHest =  \sqrt{\Nt\cdot\Nr} \cdot \frac{\sum_{i=1}^{\numclust} \mHesti}{\normfro{\sum_{i=1}^{\numclust} \mHesti}}
\end{align}
where the scaling is simply to ensure the channel matrix has fixed energy $\normfro{\mHest}^2 = \Nt \cdot \Nr$.
%\begin{align}
%\gamma = \frac{\sqrt{\Nt\Nr}}{\normfro{\sum_{i=1}^{\numclust} \mHesti}}
%\end{align}

\input{tab/tab-fitting-results-clusters.tex}

% Geometric self-interference channel modeling based on 
Inspection of our measurements revealed the presence of $\numclust = 4$ clusters whose centers are listed in \tabref{tab:fitting-results-clusters} and were mentioned before based on \figref{fig:azimuth}.
Notice that the azimuthal components of the \glspl{aod} and \glspl{aoa} are beyond $\pm 90^\circ$ rather than within the $[-60^\circ,60^\circ]$ that was measured, as was illustrated in \figref{fig:clusters}.
This decision is an arbitrary one since the array response of a \upa is symmetric about $\pm 90^\circ$; in other words, an azimuth of $60^\circ$ induces the same array response as an azimuth of $120^\circ$.
We made this choice to follow the intuition that self-interference is presumably coupled \textit{behind} the arrays since measurements took place in an anechoic chamber free of any significant reflectors in front of the arrays.
We have observed that the dominant coupling exists in and around the azimuth plane, meaning $\varphitx\idx{k} = \varphirx\idx{k} = 0^\circ$ for all $k = 1, \dots, \numclust$.
This can likely be attributed to the fact that our transmit and receive arrays are aligned in elevation, though in other configurations, components beyond an elevation of $0^\circ$ may play a more significant role.
We empirically found a good angular spread to be $\Delta\vartheta = 4^\circ$ and $\Delta\varphi = 3^\circ$, meaning $\numrays = 9 \cdot 7 = 63$ rays per cluster when discretizing the clusters by $1^\circ$ in azimuth and elevation.
% We evaluate these modeling parameters shortly.
Note that other cluster parameters could be used for systems that see other self-interference profiles, potentially also to account for reflections off the environment.


\textbf{Using our geometric channel to estimate $\muij$.}
With our geometric channel model in hand, we now aim to estimate $\muij$ for particular transmit and receive beams.
To do so, we developed the estimator % expressed as
% found the following estimator to be particularly useful % expression
\begin{align}
\muijest = \todB{\frac{\eirp \cdot \Gsqest \cdot \bars{\vw\thphrxj\ctrans \mHest \vf\thphtxi}^{2\cdot\xi}}{\powernoise}}, \label{eq:compute-muij}
\end{align}
which is rooted in using $\mHest$ and the beamforming weights $\vf\thphtxi$ and $\vw\thphrxj$ to capture coupling trends as a function of transmit and receive beamforming.
The expression of \eqref{eq:compute-muij} is quite similar to and is inspired by that of \eqref{eq:power-si}--\eqref{eq:power-si-inr}. 
The scalars $\xi$ and $\Gsqest$ serve as model parameters that we will fit based on our measurements using the true $\braces{\muij}$.
Along with normalizing the energy of the channel matrix as $\normfro{\mHest}^2 = \Nt \cdot \Nr$, we also remind the reader that we normalize our beams as $\normtwo{\vf}^2 = \Nt$ and $\normtwo{\vw}^2 = \Nr$. 
These normalizations are crucial for proper scaling of $\muijest$.
% The parameters $\Gsq$ and $\xi$ are fitted using the true $\braces{\muij}$ as follows.
Recall that \eqref{eq:compute-muij} is used to estimate the mean $\muij$ of the $(i,j)$-th neighborhood and not the actual \ginr of the $(i,j)$-th beam pair.
For this reason, $\Gsqest$ and $\mHbar$ should not be thought of as equal to $\Gsq$ and $\mH$, though they may closely align. 

% Furthermore, the relationship defined by \eqref{eq:power-si} may not exactly hold in practice if self-interference is not linearly related to $\vf$ and $\vw$.

\textbf{Fitting model parameters $\xi$ and $\Gsqest$ to measurements.}
The model parameters $\xi$ and $\Gsqest$ introduced in \eqref{eq:compute-muij} provide us a means to account for distributional discrepancies in $\braces{\muij}$ and the \ginr one would theoretically expect based on our coarsely-approximated channel $\mHest$.
The role of these model parameters can be better observed by expressing \eqref{eq:compute-muij} in log-form as
\begin{align}
% \muijest &= \xi \cdot 10 \cdot \logten{\Gammaij} + \todB{G^2} + \todBm{\powertx} - \todBm{\powernoise} \\
% \muijest &= \underbrace{\xi}_{\mathsf{scale}} \cdot \underbrace{10 \cdot \logten{\Gammaij}}_{\mathsf{shape}} + \underbrace{\todB{\Gsqest}}_{\mathsf{location}} + \underbrace{\todBm{\eirp} - \todBm{\powernoise}}_{\mathsf{system~parameters}}
\muijest &= \underbrace{\xi}_{\mathsf{scale}} \cdot \underbrace{\todB{\Gammaij}}_{\mathsf{shape}} + \underbrace{\todB{\Gsqest}}_{\mathsf{location}} + \underbrace{\todBm{\eirp} - \todBm{\powernoise}}_{\mathsf{system~parameters}}, \label{eq:muijest-log}
\end{align}
where the coupling of the $i$-th transmit beam with the $j$-th receive beam over the channel $\mHest$ is
\begin{align}
\Gammaij = \bars{\vw\thphrxj\ctrans \mHest \vf\thphtxi}^2 \label{eq:gamma-ij}.
\end{align}
% captures the (theoretical) coupling of the $i$-th transmit beam with the $j$-th receive beam over the channel $\mHest$.
From \eqref{eq:muijest-log}, we see that the shape of the distribution of $\braces{\muijest}$ is dictated by the theoretical coupling factors $\braces{\Gammaij}$, while its scale and location are controlled by $\xi$ and $\Gsqest$, respectively. 

\begin{figure*}
    \centering
    \subfloat[True fitted mean $\muij$.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{plots/main_apple_v03_03}
        \label{fig:matrix-muij-a}}
    \quad
    \subfloat[Estimated mean $\muijest$.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{plots/main_apple_v03_04}
        \label{fig:matrix-muij-b}}
    \caption{(a) The true fitted mean $\muij$ for each of the nearly 6.5 million transmit-receive beam pairs $(i,j)$. (b) The estimated counterpart of (a), where $\muijest$ for each beam pair has been estimated using \eqref{eq:muijest-log} with fitted $\xi$ and $\Gsqest$. The strong structural similarity between the two confirms that $\mHest$ captures large-scale spatial trends observed in our measurements.}
    \label{fig:matrix-muij}
\end{figure*}


In order to ensure the distribution of our estimates $\braces{\muijest}$ matches that of the true $\braces{\muij}$ in terms of scale and location, we fit $\xi$ and $\Gsqest$ as follows.
We first fit $\xi$ as
\begin{align}
\xi = \sqrt{\frac{\varop{\braces{\muij}}}{\varop{\braces{\todB{\Gamma_{ij}}}}}}
\end{align}
to align the variance of our estimates $\braces{\muijest}$ with the variance of the true $\braces{\muij}$.
%\begin{align}
%\varop{\braces{\muijest}} = \varop{\braces{\muij}}
%\end{align}
Then, $\Gsqest$ is fitted to align their locations as
\begin{align}
\GsqestdB 
% = \frac{\meanop{\braces{\muij}}}{\meanop{\braces{\xi \cdot \todB{\Gamma_{ij}}}}}
% = \meanop{\braces{\muij}} - \meanop{\braces{\xi \cdot \todB{\Gamma_{ij}} + \todBm{\eirp} - \todBm{\powernoise}}} \\
= \meanop{\braces{\muij}} - \meanop{\braces{\xi \cdot \todB{\Gamma_{ij}}}} - \todBm{\eirp} + \todBm{\powernoise},
% = & \ \meanop{\braces{\muij}} - \meanop{\braces{\xi \cdot \todB{\Gamma_{ij}}}} \nonumber \\
% & - \todBm{\eirp} + \todBm{\powernoise},
\end{align}
which ensures that the mean of our estimates $\braces{\muijest}$ matches that of the true $\braces{\muij}$.
Following this fitting from our measurements and $\mHbar$, $\xi = 0.503$ and $\Gsqest = -130.19$ dB.







% In addition, $\xi$ and $\Gsq$ can account for distributional differences

% a means to correct for imperfections in our approximated channel $\mHest$ and the theoretical coupling power versus that of our measurements.


%\begin{figure*}
%    \centering
%    \subfloat[True fitted mean $\muij$ and estimated mean $\muijest$.]{\includegraphics[width=0.475\linewidth,height=0.265\textheight,keepaspectratio]{plots/main_apple_v03_02}
%        \label{fig:cdf-muij-a}}
%    \quad
%    \subfloat[Estimation error $\muij - \muijest$.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{plots/main_apple_v03_01}
%        \label{fig:cdf-muij-b}}
%    \caption{(a) The \gcdf of the true fitted mean $\muij$ and the estimated mean $\muijest$ for all nearly 6.5 million beam pairs $(i,j)$; in other words, the \gpcdf of \figref{fig:matrix-muij-a} and \figref{fig:matrix-muij-b}. (b) The empirical \gpdf of the error between $\muij$ and $\muijest$ for all nearly 6.5 million beam pairs $(i,j)$; in other words, the \gpdf of the difference between \figref{fig:matrix-muij-a} and \figref{fig:matrix-muij-b}.}
%    \label{fig:cdf-muij}
%\end{figure*}

\begin{figure*}
    \centering
    \subfloat[True fitted mean $\muij$ and estimated mean $\muijest$.]{\includegraphics[width=0.475\linewidth,height=0.265\textheight,keepaspectratio]{plots/main_apple_v03_02}
        \label{fig:cdf-muij-a}}
    \quad
    \subfloat[Estimation error $\muij - \muijest$.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{plots/main_apple_v03_01}
        \label{fig:cdf-muij-b}}
    \caption{(a) The \gcdf of the true fitted mean $\muij$ and the estimated mean $\muijest$ for all nearly 6.5 million beam pairs $(i,j)$; in other words, the \gpcdf of \figref{fig:matrix-muij-a} and \figref{fig:matrix-muij-b}. (b) The \gcdf of the error between $\muij$ and $\muijest$ for all nearly 6.5 million beam pairs $(i,j)$; in other words, the \gcdf of the difference between \figref{fig:matrix-muij-a} and \figref{fig:matrix-muij-b}.}
    \label{fig:cdf-muij}
\end{figure*}

We evaluate our estimation of $\muij$ in \figref{fig:matrix-muij} and \figref{fig:cdf-muij}.
First, consider \figref{fig:matrix-muij-a} and \figref{fig:matrix-muij-b}, which depict all nearly 6.5 million $\muij$ and the corresponding estimates $\braces{\muijest}$, respectively.
Clearly, our estimates $\braces{\muijest}$ align visually with the true $\braces{\muij}$.
% Our coarse approximation of the self-interference channel $\mHest$ produces estimates $\braces{\muijest}$ that align \textit{structurally} with the true $\braces{\muij}$. 
Our ability to closely reproduce the structure of $\braces{\muij}$ via $\mHbar$ suggests that the dominant source of self-interference stems from coupling clusters (implicitly a far-field model) as opposed to the aforementioned highly-idealized near-field model \cite{spherical_2005}.
The magnitude of these estimates $\braces{\muijest}$ follows that of the true $\braces{\muij}$, courtesy of appropriately fitted $\xi$ and $\Gsqest$.
This can be further observed in \figref{fig:cdf-muij-a}, which compares the \gpcdf of $\braces{\muij}$ and $\braces{\muijest}$ and illustrates that our estimates align closely in distribution with the ground truth.
Here, it can be thought that $\mHbar$ is responsible for aligning the \textit{shape} of the two distributions, while $\Gsqest$ and $\xi$ align the \textit{location} and \textit{scale}.
% Here, it can be thought that $\mHbar$ is responsible for producing estimates $\braces{\muijest}$ whose distributional \textit{shape} aligns with that of the true $\braces{\muij}$.
% This stark similarity suggests that 
% Our model parameters $\Gsqest$ and $\xi$ ensure that the \textit{location} and \textit{scale} of the distributions align, respectively.
% Finally, \figref{fig:cdf-muij-b} shows the empirical \acrfull{pdf} of the error associated with our estimation of $\muij$.
Finally, \figref{fig:cdf-muij-b} shows the empirical \gcdf of the error associated with our estimation of $\muij$.
As desired, this error is centered about $0$, and the vast majority of its density lay within $\bars{\muij-\muijest} \leq 10$.
Approximately $70$\% of our estimates are within $5$ dB and $90$\% are within $8$ dB.
% In other words, 
% The mean of any neighborhood $\muij$ can be estimated to within $5$--$10$ dB with high confidence.
% The tails of the error \gpdf decay quickly by around $\bars{\muij-\muijest} \geq 15$.
Altogether, this evaluation confirms that our approach accurately captures the spatial and distributional characteristics of $\muij$.
% This instills further confiden


\begin{figure*}
    \centering
    \subfloat[Linear estimation of $\varij$ based on $\muij$.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{plots/main_apple_v03_26}
        \label{fig:varij-a}}
    \quad
    \subfloat[Linear estimator error $\varij-\varijbar$.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{plots/main_apple_v03_28}
        \label{fig:varij-b}}
    \caption{(a) Pairs of true fitted $(\muij,\varij)$ and the linear estimator (dashed line) used to produce $\varijbar$. (b) The \gcdf of the linear estimator error $\varij - \varijbar$, along with the corresponding fitted normal distribution $\distgauss{0}{\nu^2}$.}
    \label{fig:varij}
    \vspace{-0.25cm}
\end{figure*}

It is natural to ask whether $\xi$ and $\Gsqest$ hold any physical meaning.
It is difficult to state precisely, but we can interpret $\xi$ and $\Gsqest$ as accomplishing a few things.
First, most naturally, $\Gsqest$ can largely be interpreted as capturing the inverse path loss and isolation between the transmit and receive arrays (e.g., due to enclosures, free space path loss), along with amplification therein. %  self-interference, with small-scale gain attributed to $\Gammaij$.
% In addition, $\Gsqest$ accounts for amplification within the transmit and receive phased array modules. 
The scale parameter $\xi$ plays an important role in correcting for deviations from the theoretical coupling between transmit and receive beams. 
It can account for small errors in our coarse geometric self-interference channel model $\mHest$, along with irregular beam patterns produced by practical arrays.
Practical beam patterns, for instance, typically do not exhibit the clean shapes and deep nulls we are accustomed to from array theory.
$\xi$ also may account for the fact that self-interference is potentially not linearly related to $\vf$ and $\vw$.
In addition, $\xi$ also importantly corrects for the fact that we are using $\Gammaij$ to estimate the \textit{mean} of the $(i,j)$-th neighborhood, rather than directly the \ginr of the $(i,j)$-th beam pair.
The parameters $\Gsqest$ and $\xi$---along with $\mHbar$---allow our statistical model to be extended to other systems by tailoring them appropriately, which presumably contain additional underlying physical meaning beyond what has already been mentioned, even if it is not yet fully fleshed out.
Note that the estimator in \eqref{eq:compute-muij} and \eqref{eq:muijest-log} is presented for measured beam pairs but can be naturally extended to more general $\vf$ and $\vw$ by dropping $(i,j)$ indexing, using fitted $\xi$ and $\Gsqest$.



% The structure of our estimates as a function of transmit-receive beam indices $(i,j)$ aligns with the measurements courtesy of our 


\subsection{Estimating Neighborhood Variance, $\varij$.}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth,height=0.27\textheight,keepaspectratio]{plots/main_apple_v03_06}
    \caption{The \gpcdf of the true fitted variance $\varij$ and the estimated variance $\varijest$.}
    \label{fig:cdf-varij}
    % \vspace{-0.5cm}
\end{figure}

Having estimated the mean $\muij$, we now focus on estimating the neighborhood variance $\varij$.
Estimating $\muij$ involved model and system parameters and fairly intuitive methods with sound connections to the physical world.
% Estimating the mean involved fairly intuitive principles and consisted of practical system parameters.
The estimation of the variance $\varij$, on the other hand, proved to be much more difficult, with less pronounced dependence on the transmit and receive beams. %  and the variance observed over the spatial neighborhood surrounding them. 
% Nonetheless, we did leverage a basic trends that were observed.
Consider \figref{fig:varij-a}, which shows scattered pairs of the true fitted $\parens{\muij,\varij}$. % ; only a fraction of the nearly 6.5 million pairs are shown for illustrative purposes.
We can observe that the variance $\varij$ varies significantly with the mean but that it tends to be smaller with higher $\muij$.
% This is in line with conclusions drawn in our prior work \cite{roberts_att_angular}.
Fitting a simple linear estimator to the true $\parens{\muij,\varij}$, shown as the dashed line, allows us to make the linear estimate $\varijbar$ of the variance $\varij$ using the mean $\muij$ via
\begin{align}
\varijbar = \muij \cdot \alpha + \beta \label{eq:varijbar}
\end{align}
where $\alpha = -0.733$ and $\beta = 42.53$ are the fitted slope and bias of our linear estimator based on our measurements.
% By first estimating $\muijest$ using our aforementioned approach, the linear estimate $\varijbar$ can be made. 
While this simple estimator captures the general trend in variance as a function of the mean, it does not capture its broad and seemingly random variability observed in \figref{fig:varij-a}.
To estimate $\varijest$, we therefore include randomness from a normal distribution in conjunction with the linear estimator to increase its variability. 
Following the linear estimator, the final estimate $\varijest$ is made via
\begin{align}
\varijest \sim \brackets{\varijbar + \distgauss{0}{\nu^2}}^{+} \label{eq:varijest}
\end{align}
where the variance of the normal distribution is fitted as $\nu^2 = 126.091$ based on the distribution of the error $\braces{\varij - \varijbar}$ illustrated in \figref{fig:varij-b}; here, $\brackets{x}^+ = \maxop{x,0}$ simply ensures $\varijest \geq 0$.
% $\nu^2$ could be a function of $\muij$.


By supplementing the linear estimate $\varijbar$ with normally-distributed noise, the distribution of $\braces{\varijest}$ closely aligns with that of the true fitted $\braces{\varij}$, as illustrated in \figref{fig:cdf-varij}.
Note that this approach aligns their \textit{distributions} rather than aiming to perfectly estimate $\varijest = \varij$.
This was done deliberately due to the simple fact that there was no reliable way to true estimate $\varij$; rather, it appeared to be extremely random.
% no relationships between $\varij$
However, by aligning the distributions of $\braces{\varijest}$ and $\braces{\varij}$, our model is able to produce realizations of self-interference with spatial richness comparable to the true measurements.
This importantly allows our model to capture the variability in self-interference over small spatial neighborhoods that was observed in our measurements.

%\begin{align}
%\varijest \sim \distgamma{\alpha}{\beta}
%\end{align}

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth,height=0.3\textheight,keepaspectratio]{plots/main_apple_v03_26}
%    \caption{Caption.}
%    \label{fig:}
%\end{figure}



\subsection{Summary}

\input{alg/algorithm-realization}
%An algorithmic summary of our statistical model of self-interference is shown in \algref{alg:algorithm-realization}.
%To summarize, engineers wishing to use our statistical model to realize self-interference would first generate $\mHest$. 
%There exists the potential to generate $\mHest$ based on different cluster parameters, array type/size, and array configuration than what we have presented based on our measurements; the methodology and validity of such is a good topic for future work.
%Likewise, the parameters $G^{-2}$, $\xi$, $\alpha$, and $\beta$ can be used directly as we presented or may be adapted for other setups and for experimentation---for instance, increasing $\Gsqest$ for configurations with greater inherent isolation between the arrays.
%For particular transmit and receive beamforming weights $\vf$ and $\vw$, the log-normal parameters $\muest$ and $\varest$ can be realized using the matrix $\hat\mH$ and model parameters.
%Then, isolation can be realized as $\todB{\inrreal} \sim \distgauss{\muest}{\varest}$, and optionally, bounding can be used to prevent undesired outliers as
%\begin{align}
%\todB{\inrreal} \leftarrow \minop{\maxop{\todB{\inrreal},\todB{\inrmin}},\todB{\inrmax}}
%\end{align}
%where $\todB{\inrmin}$ and $\todB{\inrmax}$ are lower and upper bounds on \ginr (in dB), respectively.
%The resulting self-interference power $\powersi$ and \gls{inr} $\inr$ can be computed based on a system's transmit power into the transmit array $\powertx$ and noise power $\powernoise$ of the receive array; note that $\powertx$ may be translated from our system's $\powertx = -15$ dBm based on a difference in \gls{eirp} (ours is $60$ dBm).
%Notice that our statistical model does not require beams to fall on our $1^\circ$ grid of measurements nor within our measurement region.

% \begin{remark}[Summary]
    \edit{A summary of our statistical model of self-interference is shown in \algref{alg:algorithm-realization}. % , and our system and fitted model parameters are listed in \tabref{tab:fitting-results}.
    For particular transmit and receive beamforming weights $\vf$ and $\vw$, the mean $\muest$ is computed using model parameters $\mHest$, $\Gsqest$, and $\xi$ and system parameters $\eirp$ and $\powernoise$.
    Then, the variance $\varest$ can be realized using $\muest$ and model parameters $\alpha$ and $\beta$, along with normally-distributed noise having variance $\nu^2$.
    Recall, these system and model parameters can be unique to a particular full-duplex \mmwave platform; they may be fitted directly from measurements or referenced from future wireless standards or the literature.
    A realization of self-interference can be drawn from the normal distribution $\distgauss{\muest}{\varest}$ and can be bounded if desired to prevent extreme outliers.}
    % If needed, self-interference power can be computed from the system noise power and the realized \ginr.
    
    % To summarize, engineers wishing to use our statistical model to realize self-interference would first generate the matrix $\mHest$.
    % One may wish to use the same cluster parameters we have presented in \tabref{tab:fitting-results-clusters} or there exists the potential use other cluster parameters, though the methodology and validity of such requires dedicated future work.
    
    % There exists the potential to generate $\mHest$ based on different cluster parameters, array type/size, and array configuration than what we have presented based on our measurements; the methodology and validity of such is a good topic for future work.
    % Likewise, the parameters $G^{-2}$, $\xi$, $\alpha$, and $\beta$ can be used directly as we presented or may be adapted for other setups and for experimentation---for instance, increasing $\Gsqest$ for configurations with greater inherent isolation between the arrays.
    % For particular transmit and receive beamforming weights $\vf$ and $\vw$, the log-normal parameters $\muest$ and $\varest$ can be realized using the matrix $\hat\mH$ and model parameters.
% \end{remark}


% \edit{We would like to remark that using $\mHbar$ to directly estimate self-interference based on \eqref{eq:power-si} is not reliable for a few reasons. First of all, the relatively simple geometric model we have uncovered does not capture the spatial richness of our measurements. Secondly, it will produce realiztions that align with our measurements on a large-scale but do not align in magnitude with our measurements without.}





==> sec-peer-review-title.tex <==
% For peer review papers, you can put extra information on the cover
% page as needed:
% \ifCLASSOPTIONpeerreview
% \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% \fi
%
% For peerreview papers, this IEEEtran command inserts a page break and
% creates the second title. It will be ignored for other modes.
\IEEEpeerreviewmaketitle

==> sec-problem-formulation-v2.tex <==
\section{Problem Formulation and Motivation} \label{sec:problem-formulation}

Using the established system model, we now further formulate and motivate this work.
Again taking the perspective of the full-duplex \bs, we refer to downlink as the \textit{transmit link} and to uplink as the \textit{receive link}.
For some transmit and receive beams $\vf$ and $\vw$, the \glspl{snr} of the transmit and receive links are respectively
\begin{align}
%\snrtx &= \frac{\powertxbs \cdot \Gtx^2 \cdot \bars{\vhtx\ctrans \vf}^2}{\Nt \cdot \powernoiseue} \quad \label{eq:snr-tx} \\
%\snrrx &= \frac{\powertxue \cdot \Grx^2 \cdot \bars{\vw\ctrans \vhrx}^2}{\normtwo{\vw}^2 \cdot \powernoisebs} \label{eq:snr-rx}
\snrtx &= \frac{\powertxbs \cdot \Gtx^2 \cdot \bars{\vhtx\ctrans \vf}^2}{\Nt \cdot \powernoiseue}, \qquad 
\snrrx = \frac{\powertxue \cdot \Grx^2 \cdot \bars{\vw\ctrans \vhrx}^2}{\normtwo{\vw}^2 \cdot \powernoisebs} \label{eq:snr-trx}
\end{align}
where dividing by $\Nt$ in $\snrtx$ handles power splitting within the transmit array and by $\normtwo{\vw}^{2}$ in $\snrrx$ handles noise combining at the receive array.
By virtue of the fact that % $\Na = \max_{\vx} \ \bars{\vh\ctrans \vx}^2 \ \st \normtwo{\vx}^2 \leq 1, \normtwo{\vh}^2 = \Na$,
\begin{align}
% \Na &= \max_{\vf} \ \bars{\vh\ctrans \vf}^2 \ \st \normtwo{\vf}^2 = 1, \normtwo{\vh}^2 = \Na \\
% \Na &= \max_{\vw} \ \bars{\vw\ctrans \vh}^2 \ \st \normtwo{\vw}^2 = 1, \normtwo{\vh}^2 = \Na
N^2 &= \normtwo{\vh}^2 \cdot \normtwo{\vx}^2 = \max_{\vx} \ \bars{\vh\ctrans \vx}^2 \ \st \normtwo{\vx}^2 \leq N, \normtwo{\vh}^2 = N
\end{align}
the maximum \gpsnr are denoted with an overline as
%\begin{align}
%\snrbhdlbar &= \frac{\powertxdonor \cdot \Gbh^2 \cdot \Na}{\powernoiseiab} \geq \snrbhdl \\
%\snracdlbar &= \frac{\powertxiab \cdot \Gac^2 \cdot \Na}{\powernoiseue} \geq \snracdl \\
%\snrbhulbar &= \frac{\powertxiab \cdot \Gbh^2 \cdot \Na}{\powernoisedonor} \geq \snrbhul \\
%\snraculbar &= \frac{\powertxue \cdot \Gac^2 \cdot \Na}{\powernoiseiab} \geq \snracul.
%\end{align}
\begin{align}
%\snrtxbar &= \frac{\powertxbs \cdot \Gtx^2 \cdot \Nt}{\powernoiseue} \geq \snrtx \quad \\
%\snrrxbar &= \frac{\powertxue \cdot \Grx^2 \cdot \Nr}{\powernoisebs} \geq \snrrx.
\snrtxbar &= \frac{\powertxbs \cdot \Gtx^2 \cdot \Nt}{\powernoiseue} \geq \snrtx, \qquad
\snrrxbar = \frac{\powertxue \cdot \Grx^2 \cdot \Nr}{\powernoisebs} \geq \snrrx.
\end{align}
In other words, these are achieved only when users are delivered maximum beamforming gain.

% \begin{align}
% \snrtx &= \snrtxbar \cdot \frac{\bars{\vhtx\ctrans \vf}^2}{\Nt^2} \\
% \snrrx &= \snrrxbar \cdot \frac{\bars{\vhrx\ctrans \vw}^2}{\Nr^2} 
% \end{align}

When juggling a transmit beam $\vf$ and receive beam $\vw$ in a full-duplex fashion, the \bs couples self-interference, leading to a receive link \ginr of
\begin{align}
\inrrx = \frac{\powertxbs \cdot G^2 \cdot \bars{\vw\ctrans \mH \vf}^2}{\Nt \cdot \normtwo{\vw}^2 \cdot \powernoisebs}
\end{align}
where $\bars{\vw\ctrans \mH \vf}^2$ captures the transmit and receive beam coupling over the self-interference channel.
Strategically steering $\vf$ and $\vw$ according to $\mH$ can therefore reduce self-interference.
% It can be readily seen that decreasing the large-scale gain $G$ (increasing isolation between the arrays) would reduce self-interference, as well as strategically steering $\vf$ and $\vw$ according to the channel $\mH$.
% It can be readily seen that strategically steering $\vf$ and $\vw$ according to the channel $\mH$ can reduce self-interference.
% By virtue of the fact that 
The worst-case coupling between transmit and receive beams at the full-duplex \bs is
\begin{align}
\Nt^2 \cdot \Nr^2 
% &= \normtwo{\vw}^2 \cdot \normfro{\mH}^2 \cdot \normtwo{\vf}^2 
&= \max_{\vf,\vw} \ \bars{\vw\ctrans \mH \vf}^2 \ \st \normtwo{\vf}^2 \leq \Nt, \normtwo{\vw}^2 \leq \Nr, \normfro{\mH}^2 = \Nt \cdot \Nr
\end{align}
leading to a maximum possible $\inrrx$ of
\begin{align}
\inrrxbar = \frac{\powertxbs \cdot G^2 \cdot \Nt \cdot \Nr}{\powernoisebs} \geq \inrrx
\end{align}
which we use as a metric in \secref{sec:simulation-results} to capture the inherent strength of self-interference at the \bs.
Note that $\inrrxbar$ depends solely on system parameters and artifacts at the \bs, chiefly the inverse path loss $G^2$ between its transmit and receive arrays. % at the \bs.
% $\inrrxbar$ increases 
Interestingly, we see that as $\powertxbs$ increases and/or $\powernoisebs$ decreases, which positively contribute to downlink and uplink, the inherent strength of self-interference $\inrrxbar$ increases, which negatively contributes to their full-duplexing.
% which is the worst-case coupling between the transmit and receive beam.

% Since the downlink and uplink users operate simultaneously and in-band in this full-duplex setting, 
We denote $\inrtx$ as the \ginr incurred at the downlink user due to cross-link interference.
\begin{align}
\inrtx = \frac{\powertxue \cdot \Gcl^2 \cdot \bars{\hcl}^2}{\powernoiseue}
\end{align}
Note that cross-link interference $\inrtx$ only depends on its inherent channel and path loss, not on $\vf$ nor $\vw$.
With all of this, the \gpsinr of the links are
\begin{align}
\sinrtx &= \frac{\snrtx}{1+\inrtx}, \qquad 
\sinrrx = \frac{\snrrx}{1+\inrrx}.
\end{align}
The achievable spectral efficiencies on each link, treating interference as noise, are
\begin{align}
\setx &= \logtwo{1 + \sinrtx}, \qquad
\serx = \logtwo{1 + \sinrrx}
\end{align}
whereas the capacities of the two links are $\captx = \logtwo{1 + \snrtxbar}$ and $\caprx = \logtwo{1 + \snrrxbar}$.
%\begin{align}
%\captx &= \logtwo{1 + \snrtxbar}, \qquad
%\caprx = \logtwo{1 + \snrrxbar}. % \\ \capsum &= \capul + \capdl
%\end{align}

We assume no forms of self-interference cancellation are employed at the \bs.
Instead, we will rely solely on beamforming to mitigate self-interference and enable full-duplex operation. 
The degree of self-interference coupled at the full-duplex \bs depends on the transmit beam $\vf$ and receive beam $\vw$, each of which also dictates its respective link's \gsnr.
As such, it is important to design $\vf$ and $\vw$ such that low self-interference is coupled while still delivering high $\snrtx$ and $\snrrx$, in an effort to achieve high sum spectral efficiency $\setx + \serx$.
% This will be done by strategically designing $\vf$ and $\vw$ such that they couple low self-interference, as we will outline in the next section.

% The research community currently lacks a practically sound channel model for self-interference in \mmwave systems.
% As such, we do not assume a particular model for $\mH$ but rather will consider two models in our numerical results in \secref{sec:simulation-results}.
In our design, we rely on estimation of the self-interference \mimo channel $\mH$ at the full-duplex \bs.
We do not assume perfect estimation of $\mH$ but rather model its imperfections as
\begin{align}
% \mH = \mHbar + \mDelta \label{eq:channel}
\mH = \mHbar + \mDelta, \qquad \entry{\mDelta}{i,j} \sim \distcgauss{0}{\epsilon^2} \ \forall \ i,j.  \label{eq:channel}
\end{align}
where $\mHbar$ is the estimate of $\mH$ and $\mDelta$ captures \iid Gaussian estimation error with mean $0$ and variance $\epsilon^2$. 
% We assume elements of $\mDelta$ are \iid Gaussian with mean $0$ and variance $\epsilon^2$ as
% \begin{align}
% \entry{\mDelta}{i,j} \sim \distcgauss{0}{\epsilon^2} \ \forall \ i,j. \label{eq:channel-error}
% \end{align}
% Notice that the estimation of $\mH$ does not introduce any feedback over-the-air, since it takes place between the arrays at the full-duplex \bs.
% Efficient and accurate 
Self-interference channel estimation in \mmwave systems is an open research problem \cite{roberts_wcm}.
As such, the choice of a particular estimation error model is currently difficult to practically justify, but we remark that other error models (e.g., norm-based models) may be encompassed by our Gaussian model with arbitrarily high probability for appropriately chosen $\eps^2$.
It is our hope that $\mH$ can be estimated with high fidelity for two reasons.
First, the self-interference channel is likely much stronger than traditional downlink/uplink \mimo channels, meaning it may be estimated with higher accuracy.
Second, the estimation of $\mH$ takes place across the arrays of the \bs, meaning it does not consume resources for feedback and does not suffer from feedback quantization.
This suggests that the estimation of $\mH$ may be more thorough and precise than that of traditional downlink/uplink \mimo channels.
% Second, the estimation of $\mH$ does not introduce any feedback over-the-air, since it takes place between the arrays at the full-duplex \bs, suggesting that the estimation may be more thorough than traditional estimation of downlink/uplink channels; moreover, this estimation does not suffer from feedback quantization.
Nonetheless, our design in the next section incorporates channel estimation error.

In our recent measurement campaign \cite{roberts_att_angular}, we observed that the 28 GHz self-interference channel in an anechoic chamber was nearly static on the order of minutes at least.
Dynamics of the environment (e.g., moving vehicles) may lead to a reduced coherence time of $\mH$, but many unknowns remain about the degree of self-interference contributed by environmental reflections relative to the direct coupling between the transmit and receive arrays.
In this work, we assume that the self-interference channel $\mH$ is sufficiently static over many downlink/uplink time slots. % , as illustrated in \figref{fig:timeline} and described further shortly.
% It may be possible to capture slight drift of the self-interference channel over the coherence time of $\mH$ in the error matrix $\mDelta$ by appropriately choice of $\eps^2$.
% significance of the environment on self-interference.
% This will likely be reduced with dynamic environmental factors but it is unclear the significance of the.
% NMSE?
%  which is bounded as $\normfro{\mDelta}^2 \leq \eps^2 \cdot \Nt \cdot \Nr$.
% As such, the 
% \begin{align}
% \frac{\normfro{\mH - \mHbar}^2}{\ev{\normfro{\mH}^2}}
% \frac{\normfro{\mDelta}^2}{\normfro{\mH}^2} \leq \frac{\eps^2 \cdot \Nt \cdot \Nr}{\Nt \cdot \Nr} = \eps^2
% \end{align}
% Need to fix, not exactly true since not mean error, channel is not guaranteed to be norm Nt Nr.
% The normalized mean squared error of the estimation of $\mH$ is $\eps^2$.
% On average, each entry of $\mHbar$ will have an error power of $\eps^2$.
% Note that other norm-bounded errors can be translated via norm equivalence.
% In the next section, we proceed with \lonestar, our design of transmit and receive beamforming codebooks for full-duplex \mmwave systems.
% We proceed with our design in the following section.

% ---

% a service region (some portion of space based on an assumed user distribution) and then discretizing it based on the desired number of beams in the codebook or their beamwidth.

% sweeping candidate beams, measuring the reference signal received power
% (RSRP) for each candidate, and delivering feedback before determining the beam(s) for the
% mmWave link [21], [22]. 
% Candidate beams often come from a codebook, which is constructed by first defining a service region (some portion of space based on an assumed user distribution) and then discretizing it based on the desired number of beams in the codebook or their beamwidth.

% Practical systems do not have knowledge of over-the-air channels (i.e., $\vhtx$ and $\vhrx$) but rather employs beam alignment to identify beams from some beam codebook that delivers maximum gain to a user.
% This is done by explicitly measuring beams.

% Rather than design particular beams $\vf$ and $\vw$ to mitigate self-interference, we instead design beam codebooks $\precb$ and $\comcb$ such that all possible transmit-receive beam pairs couple low self-interference.
% This allows a full-duplex \mmwave system to conduct beam alignment using 

% In this paper, we seek a means to strategically select beams $\vf$ and $\vw$ such that the spectral efficiency can be improved over conventional/\naive approaches.
% Taking a full-duplex perspective, we desire a sum spectral efficiency $\setx + \serx$ that approaches the full-duplex capacity $\captx + \caprx$.
% In this pursuit, we account for a number of practical considerations in this work, most notably limited channel knowledge and practical codebook-based beam alignment.

% Introduce beam alignment. The need for beams to be highly directional.

% Why conventional beams are not good for full-duplex.

% General roadmap of our design.

% Self-interference channel variability and knowledge.
% \begin{align}
% \mH = \mHbar + \mDelta
% \end{align}
% where $\normfro{\mDelta}^2 \leq \eps$.

% With our design, cite work that will benefit (plug-and-play). Will enable analog-only BF systems. No further cancellation required. Can support codebook-based beam alignment.


\comment{
%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{fig/alignment/alignment_type_03.pdf}
%	\caption{An illustration of the coverage regions that the transmitter and receiver aim to serve.}
%	\label{fig:aod-aoa}
%\end{figure}


%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=0.3\textheight,keepaspectratio]{plots/nf_patterns_v3.eps}
%	\caption{While extremely narrow beams produced by dense antenna arrays are ``extremely narrow'' in the far-field, they are not necessarily so in the near-field.}
%	\label{fig:nf-patterns}
%\end{figure}

% Analog beamforming codebooks are used for beam alignment in \fg cellular systems and IEEE 802.11ad/ay.

Rather than obtaining over-the-air channel knowledge between two devices in order to configure $\prerf$ and $\comrf$, practical systems like \fg cellular and IEEE 802.11ad/ay have turned to codebook-based beam alignment.
By taking this approach, promising analog beams (e.g., those that offer high \gls{snr}) are identified by searching through the codebook and measuring the power delivered to a device being served.
This results in a significant complexity reduction in designing $\prerf$ and $\comrf$ and simplifies channel estimation and initial access.
Clearly, searching through $\prerfcb$ or $\comrfcb$ exhaustively during beam alignment is highly impractical.
Therefore, it is much more practical to build significantly reduced codebooks $\prerfcbbar$ and $\comrfcbbar$ from which analog precoders and combiners are drawn.
With this being said, one can see that a codebook-based analog beamforming leaves very little room for optimization: the only flexibility the system has in configuring its analog beamformers is choosing from the entries in the codebook. \edit{Improve.}

Consider our full-duplex setting where the analog precoder couples with the analog combiner via the self-interference channel.
Some transmit-receive beam pairs will inherently afford more isolation than others.
To reduce the amount of self-interference reaching the receiver, it would be ideal if all beam pairs afforded high isolation.
It is unlikely, however, for this to be the case when using ``off-the-shelf'' codebooks---after all, they were not designed with full-duplex in mind.
One may be inclined to believe that the extremely narrow beams that have become ubiquitous in \mmwave would offer robustness to coupling because of their pencil-like shape.
This is, however, not necessarily the case because these extremely narrow beams are only ``extremely narrow'' in the far-field and not necessarily so in near-field.
This is evidenced by \figref{fig:nf-patterns}, where BLANK.
This motivates us to design an analog precoding codebook $\prerfcbbar$ and combining codebook $\comrfcbbar$ that together offer high isolation across all transmit-receive beam pairs to ensure that no matter which directions a device transmits and receives from, it sees a relatively low degree of coupled self-interference.

En route to reducing the amount of self-interference coupled by the analog precoding and combining codebooks, we must ensure that the beams within the codebooks remain useful in their ability to serve users.
Since \mmwave communication relies on high analog beamforming gains for sufficient link margin, beams are only useful if they offer high gain.
Additionally, since users may exist anywhere within a service region, a codebook of beams must collectively maintain coverage to the service region.
Conventional codebooks certainly satisfy this definition of ``usefulness'' by design as exhibited by \figref{fig:conventional-codebooks}, but do not offer much robustness to self-interference as exhibited by 

With $\bitsamp$ bits of amplitude control per attenuator and $\bitsphase$ bits of phase control per phase shifter, there are a total of $2^{\bitsamp + \bitsphase}$ different ways to configure a \textit{single} analog beamforming weight.
With $\Na$ antennas, there are $2^{\Na\cdot\parens{\bitsamp+\bitsphase}}$ different ways to configure an analog beamforming vector.
With $L$ \rf chains, there are $2^{L\cdot\Na\cdot\parens{\bitsamp+\bitsphase}}$ different ways to configure an analog beamforming matrix.
To design our codebook, clearly searching exhaustively through $\prerfcb$ or $\comrfcb$ for beams that supply good coverage with reduced self-interference coupling is impractical.
This motivates us to develop a systematic methodology to efficiently build our codebook, which we present in \secref{sec:contribution-i}.

\subsection{3-D Geometry}
Let $\dirset$ be the set of all azimuth-elevation pairs $(\theta,\phi)$ where $\theta \in [0,2\pi]$ and $\phi \in [0,\pi]$.
\begin{align}
\dirset = \braces{(\theta,\phi) : \theta \in [0,2\pi], \phi \in [0,\pi]}
\end{align}
A vector in the direction $(\theta,\phi)$ is described by $\theta$ being angle between the positive $y$ axis and the vector's orthogonal projection onto the $x$-$y$ plane and $\phi$ being the angle from the $x$-$y$ plane to the vector itself.

\begin{definition}[Transmit and receive beam mappings]
	Let $f : \dirset \to \precb$ be a mapping from transmit direction to analog precoding weights $\vf$ as
	\begin{align}
	\vf = f(\thetatx,\phitx)
	\end{align}
	where $(\thetatx,\phitx) \in \dirset$ is a transmit direction.
	Similarly, let $w : \set{A} \to \comcb$ be a mapping from receive direction to analog combining weights $\vw$ as
	\begin{align}
	\vw = w(\thetarx,\phirx)
	\end{align}
	where $(\thetarx,\phirx) \in \dirset$ is a receive direction.
	The mappings $f$ and $w$ capture arbitrary beamforming design methodologies, which are implemented by system engineers or supplied by the array manufacturer.
\end{definition}
}

==> sec-problem-formulation.tex <==
\section{Problem Formulation and Motivation} \label{sec:problem-formulation}

Using the established system model, we now further formulate and motivate this work.
For some transmit and receive beams $\vf$ and $\vw$, the \glspl{snr} of downlink and uplink are respectively
\begin{align}
\snrtx &= \frac{\powertxbs \cdot \Gtx^2 \cdot \bars{\vhtx\ctrans \vf}^2}{\powernoiseue}, \quad \\
\snrrx &= \frac{\powertxue \cdot \Grx^2 \cdot \bars{\vw\ctrans \vhrx}^2}{\powernoisebs}.
\end{align}
By virtue of the fact that
\begin{align}
% \Na &= \max_{\vf} \ \bars{\vh\ctrans \vf}^2 \ \st \normtwo{\vf}^2 = 1, \normtwo{\vh}^2 = \Na \\
% \Na &= \max_{\vw} \ \bars{\vw\ctrans \vh}^2 \ \st \normtwo{\vw}^2 = 1, \normtwo{\vh}^2 = \Na
\Na &= \max_{\vx} \ \bars{\vh\ctrans \vx}^2 \ \st \normtwo{\vx}^2 = 1, \normtwo{\vh}^2 = \Na
\end{align}
the maximum \gpsnr, which we denote with an overline, are 
%\begin{align}
%\snrbhdlbar &= \frac{\powertxdonor \cdot \Gbh^2 \cdot \Na}{\powernoiseiab} \geq \snrbhdl \\
%\snracdlbar &= \frac{\powertxiab \cdot \Gac^2 \cdot \Na}{\powernoiseue} \geq \snracdl \\
%\snrbhulbar &= \frac{\powertxiab \cdot \Gbh^2 \cdot \Na}{\powernoisedonor} \geq \snrbhul \\
%\snraculbar &= \frac{\powertxue \cdot \Gac^2 \cdot \Na}{\powernoiseiab} \geq \snracul.
%\end{align}
\begin{align}
\snrtxbar &= \frac{\powertxbs \cdot \Gtx^2 \cdot \Nt}{\powernoiseue} \geq \snrtx, \quad \\
\snrrxbar &= \frac{\powertxue \cdot \Grx^2 \cdot \Nr}{\powernoisebs} \geq \snrrx
\end{align}

The full-duplex \bs couples self-interference, leading to a receive link \ginr of
\begin{align}
\inrrx = \frac{\powertxbs \cdot G^2 \cdot \bars{\vw\ctrans \mH \vf}^2}{\powernoisebs}
\end{align}
where $\bars{\vw\ctrans \mH \vf}^2$ captures the transmit and receive beam coupling over the self-interference channel.
Since the downlink and uplink users operate simultaneously and in-band in this full-duplex setting, let $\inrtx$ be the \ginr due to cross-link interference.
\begin{align}
\inrtx = \frac{\powertxue \cdot \Gcl^2 \cdot \bars{\hcl}^2}{\powernoisebs}
\end{align}
Note that cross-link interference only depends on its inherent channel and path loss, not on $\vf$ nor $\vw$.
With these, the \gsinr of the two links becomes
\begin{align}
\sinrtx &= \frac{\snrtx}{1+\inrtx}, \quad 
\sinrrx = \frac{\snrrx}{1+\inrrx}.
\end{align}
Treating interference as noise, the maximum achievable spectral efficiencies on each link are
\begin{align}
\setx &= \logtwo{1 + \sinrtx}, \quad
\serx = \logtwo{1 + \sinrrx}
\end{align}
whereas the individual Shannon capacities of each of these links are
\begin{align}
\captx &= \logtwo{1 + \snrtxbar}, \quad
\caprx = \logtwo{1 + \snrrxbar}. % \\ \capsum &= \capul + \capdl
\end{align}

The degree of self-interference coupled at the full-duplex \bs depends on the choice of transmit beam $\vf$ and receive beam $\vw$, each of which also dictates its respective link \gsnr.
As such, it is important to design $\vf$ and $\vw$ such that low self-interference is coupled while still delivering high \gsnr, in an effort to achieve high sum spectral efficiency $\setx + \serx$.

Practical \mmwave systems---which have operated in a half-duplex fashion thus far---rely on beam alignment to identify transmit and receive beams that deliver high beamforming gain when serving a particular user.
This is typically done by sweeping a set of candidate beams (called a \textit{codebook}) and measuring the \gls{rsrp} for each candidate to select which beam to use for a given \mmwave link.
This allows the \mmwave system to reliably deliver high beamforming gain without the need for over-the-air channel knowledge (i.e., $\vhtx$ and $\vhrx$).
A beam codebook is often constructed by discretizing a service region based on the number of beams in the codebook or their beamwidth.

In this work, rather than design particular transmit and receive beams $\vf$ and $\vw$ to use at the full-duplex \bs, we instead design transmit and receive beam codebooks $\precbbar$ and $\comcbbar$ from which it will draw from for $\vf$ and $\vw$.
% If successful, our beam codebooks will have effects twofold.
A full-duplex \mmwave \bs with our codebooks will be able to deliver high beamforming gain to users via beam alignment and simultaneously mitigate self-interference.
With our design, transmit and receive beams will couple low self-interference, regardless of which $\vf \in \precbbar$ and $\vw \in \comcbbar$ are selected following beam alignment.
In contrast, off-the-shelf codebooks have delivered high beamforming gain but are not robust to self-interference, since they have been designed with half-duplex in mind.

If our design sufficiently mitigates self-interference between all beam pairs, a \mmwave \bs employing our codebooks can seamlessly operate in a full-duplex fashion without any additional self-interference cancellation---any transmit and receive beams selected via beam alignment will inherently offer high isolation.
In addition, our design could enhance existing \mmwave full-duplex work that accounts for codebook-based analog beamforming.
Hybrid beamforming full-duplex systems could leverage our codebooks to weaken the effective self-interference channel post beam alignment.

The research community currently lacks a practically sound channel model for self-interference in \mmwave systems.
As such, we do not assume a particular model for $\mH$ but rather will consider two models in our numerical results in \secref{sec:simulation-results}.
In our design, we rely on estimation of the \mimo self-interference channel $\mH$, which does not introduce any over-the-air feedback since it takes place between the arrays at the full-duplex \bs.
We assume that the self-interference channel $\mH$ is sufficiently static over many uplink and downlink time slots.\footnote{In our recent measurement campaign, which was conducted in an anechoic chamber, we observed that the 28 GHz self-interference channel was static on the order of minutes, at least. This will likely be reduced with dynamic environmental factors.}
We do not assume perfect estimation of $\mH$ but rather capture its estimation error as
\begin{align}
\mH = \mHbar + \mDelta
\end{align}
where $\mHbar$ is the estimate of $\mH$ and $\mDelta$ is the error, which is bounded as $\normfro{\mDelta}^2 \leq \eps^2 \cdot \Nt \cdot \Nr$.
\begin{align}
\frac{\normfro{\mDelta}^2}{\normfro{\mH}^2} \leq \frac{\eps^2 \cdot \Nt \cdot \Nr}{\Nt \cdot \Nr} = \eps^2
\end{align}
Need to fix, not exactly true since not mean error, channel is not guaranteed to be norm Nt Nr.
The normalized mean squared error of the estimation of $\mH$ is $\eps^2$.
On average, each entry of $\mHbar$ will have an error power of $\eps^2$.
Note that other norm-bounded errors can be translated via norm equivalence.
Practically, we envision conducting thorough estimation of $\mH$ and execution of our design during initial setup of the \bs and performing updates to the estimate of $\mH$ and to our design.

In pursuit of transmit and receive beam codebooks that can offer high sum spectral efficiency $\setx + \serx$, we desire transmit-receive beam pairs that deliver high $\snrtx$ and $\snrrx$ while coupling low self-interference $\inrrx$.
As mentioned, $\inrtx$ is fixed for a given downlink-uplink user pair since it does not depend on the choice of $\vf$ nor $\vw$.
We proceed with our design in the follow section.

% ---

% a service region (some portion of space based on an assumed user distribution) and then discretizing it based on the desired number of beams in the codebook or their beamwidth.

% sweeping candidate beams, measuring the reference signal received power
% (RSRP) for each candidate, and delivering feedback before determining the beam(s) for the
% mmWave link [21], [22]. 
% Candidate beams often come from a codebook, which is constructed by first defining a service region (some portion of space based on an assumed user distribution) and then discretizing it based on the desired number of beams in the codebook or their beamwidth.

% Practical systems do not have knowledge of over-the-air channels (i.e., $\vhtx$ and $\vhrx$) but rather employs beam alignment to identify beams from some beam codebook that delivers maximum gain to a user.
% This is done by explicitly measuring beams.

% Rather than design particular beams $\vf$ and $\vw$ to mitigate self-interference, we instead design beam codebooks $\precb$ and $\comcb$ such that all possible transmit-receive beam pairs couple low self-interference.
% This allows a full-duplex \mmwave system to conduct beam alignment using 

% In this paper, we seek a means to strategically select beams $\vf$ and $\vw$ such that the spectral efficiency can be improved over conventional/\naive approaches.
% Taking a full-duplex perspective, we desire a sum spectral efficiency $\setx + \serx$ that approaches the full-duplex capacity $\captx + \caprx$.
% In this pursuit, we account for a number of practical considerations in this work, most notably limited channel knowledge and practical codebook-based beam alignment.

% Introduce beam alignment. The need for beams to be highly directional.

% Why conventional beams are not good for full-duplex.

% General roadmap of our design.

% Self-interference channel variability and knowledge.
% \begin{align}
% \mH = \mHbar + \mDelta
% \end{align}
% where $\normfro{\mDelta}^2 \leq \eps$.

% With our design, cite work that will benefit (plug-and-play). Will enable analog-only BF systems. No further cancellation required. Can support codebook-based beam alignment.


\comment{
%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{fig/alignment/alignment_type_03.pdf}
%	\caption{An illustration of the coverage regions that the transmitter and receiver aim to serve.}
%	\label{fig:aod-aoa}
%\end{figure}


%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=0.3\textheight,keepaspectratio]{plots/nf_patterns_v3.eps}
%	\caption{While extremely narrow beams produced by dense antenna arrays are ``extremely narrow'' in the far-field, they are not necessarily so in the near-field.}
%	\label{fig:nf-patterns}
%\end{figure}

% Analog beamforming codebooks are used for beam alignment in \fg cellular systems and IEEE 802.11ad/ay.

Rather than obtaining over-the-air channel knowledge between two devices in order to configure $\prerf$ and $\comrf$, practical systems like \fg cellular and IEEE 802.11ad/ay have turned to codebook-based beam alignment.
By taking this approach, promising analog beams (e.g., those that offer high \gls{snr}) are identified by searching through the codebook and measuring the power delivered to a device being served.
This results in a significant complexity reduction in designing $\prerf$ and $\comrf$ and simplifies channel estimation and initial access.
Clearly, searching through $\prerfcb$ or $\comrfcb$ exhaustively during beam alignment is highly impractical.
Therefore, it is much more practical to build significantly reduced codebooks $\prerfcbbar$ and $\comrfcbbar$ from which analog precoders and combiners are drawn.
With this being said, one can see that a codebook-based analog beamforming leaves very little room for optimization: the only flexibility the system has in configuring its analog beamformers is choosing from the entries in the codebook. \edit{Improve.}

Consider our full-duplex setting where the analog precoder couples with the analog combiner via the self-interference channel.
Some transmit-receive beam pairs will inherently afford more isolation than others.
To reduce the amount of self-interference reaching the receiver, it would be ideal if all beam pairs afforded high isolation.
It is unlikely, however, for this to be the case when using ``off-the-shelf'' codebooks---after all, they were not designed with full-duplex in mind.
One may be inclined to believe that the extremely narrow beams that have become ubiquitous in \mmwave would offer robustness to coupling because of their pencil-like shape.
This is, however, not necessarily the case because these extremely narrow beams are only ``extremely narrow'' in the far-field and not necessarily so in near-field.
This is evidenced by \figref{fig:nf-patterns}, where BLANK.
This motivates us to design an analog precoding codebook $\prerfcbbar$ and combining codebook $\comrfcbbar$ that together offer high isolation across all transmit-receive beam pairs to ensure that no matter which directions a device transmits and receives from, it sees a relatively low degree of coupled self-interference.

En route to reducing the amount of self-interference coupled by the analog precoding and combining codebooks, we must ensure that the beams within the codebooks remain useful in their ability to serve users.
Since \mmwave communication relies on high analog beamforming gains for sufficient link margin, beams are only useful if they offer high gain.
Additionally, since users may exist anywhere within a service region, a codebook of beams must collectively maintain coverage to the service region.
Conventional codebooks certainly satisfy this definition of ``usefulness'' by design as exhibited by \figref{fig:conventional-codebooks}, but do not offer much robustness to self-interference as exhibited by 

With $\bitsamp$ bits of amplitude control per attenuator and $\bitsphase$ bits of phase control per phase shifter, there are a total of $2^{\bitsamp + \bitsphase}$ different ways to configure a \textit{single} analog beamforming weight.
With $\Na$ antennas, there are $2^{\Na\cdot\parens{\bitsamp+\bitsphase}}$ different ways to configure an analog beamforming vector.
With $L$ \rf chains, there are $2^{L\cdot\Na\cdot\parens{\bitsamp+\bitsphase}}$ different ways to configure an analog beamforming matrix.
To design our codebook, clearly searching exhaustively through $\prerfcb$ or $\comrfcb$ for beams that supply good coverage with reduced self-interference coupling is impractical.
This motivates us to develop a systematic methodology to efficiently build our codebook, which we present in \secref{sec:contribution-i}.

\subsection{3-D Geometry}
Let $\dirset$ be the set of all azimuth-elevation pairs $(\theta,\phi)$ where $\theta \in [0,2\pi]$ and $\phi \in [0,\pi]$.
\begin{align}
\dirset = \braces{(\theta,\phi) : \theta \in [0,2\pi], \phi \in [0,\pi]}
\end{align}
A vector in the direction $(\theta,\phi)$ is described by $\theta$ being angle between the positive $y$ axis and the vector's orthogonal projection onto the $x$-$y$ plane and $\phi$ being the angle from the $x$-$y$ plane to the vector itself.

\begin{definition}[Transmit and receive beam mappings]
	Let $f : \dirset \to \precb$ be a mapping from transmit direction to analog precoding weights $\vf$ as
	\begin{align}
	\vf = f(\thetatx,\phitx)
	\end{align}
	where $(\thetatx,\phitx) \in \dirset$ is a transmit direction.
	Similarly, let $w : \set{A} \to \comcb$ be a mapping from receive direction to analog combining weights $\vw$ as
	\begin{align}
	\vw = w(\thetarx,\phirx)
	\end{align}
	where $(\thetarx,\phirx) \in \dirset$ is a receive direction.
	The mappings $f$ and $w$ capture arbitrary beamforming design methodologies, which are implemented by system engineers or supplied by the array manufacturer.
\end{definition}
}

==> sec-simulation-results.tex <==
\section{Simulation Results} \label{sec:simulation-results}

% Operating at higher $\inrrxbar$ means we can transmit with higher power, less constrained on our system setup since we can tolerate higher $\inrrxbar$.

% -------------------------------------------------------------------------------------------------
% Setup.
% -------------------------------------------------------------------------------------------------
We simulated the full-duplex system illustrated in \figref{fig:system} at 30 GHz in a Monte Carlo fashion to extensively evaluate \lonestar against conventional, off-the-shelf codebooks \cite{mfm_arxiv}.
% The two users are equipped with a single antenna while 
The full-duplex \bs is equipped with two $8 \times 8$ half-wavelength \acrlongpl{upa} for transmission and reception; users have a single antenna for simplicity.
Analog beamforming networks at the \bs use log-stepped attenuators with $0.5$ dB of attenuation per \gls{lsb}.
To serve downlink and uplink users, the full-duplex \bs uses $\Mtx = \Mrx = 45$ beams distributed from $-60^\circ$ to $60^\circ$ in azimuth and from $-30^\circ$ to $30^\circ$ in elevation, each in $15^\circ$ steps.
Users are distributed uniformly from $-67.5^\circ$ to $67.5^\circ$ in azimuth and from $-37.5^\circ$ to $37.5^\circ$ in elevation.
The downlink and uplink channels are simulated as \gls{los} channels for simplicity; similar conclusions would be expected when modeling them otherwise due to the directional nature of \mmwave channels.
To select which transmit and receive beams serve a given downlink and uplink user pair, we use exhaustive beam sweeping on each link independently and choose the beams that maximize $\snrtx$ and $\snrrx$.
% We use exhaustive beam search to select which beam serves each user.
The choice of a particular self-interference channel model is a difficult one to justify practically, given there lacks a well-accepted, measurement-backed model.
We have chosen to simulate the self-interference channel $\mH$ using the spherical-wave channel model \cite{spherical_2005}, which captures idealized near-field propagation between the transmit and receive arrays of the full-duplex device and has been used widely thus far in related literature.
This channel model is a function of the relative geometry between the transmit and receive arrays and is described as
\begin{align}
\entry{\mH}{m,n} = \frac{\rho}{r_{n,m}}\exp \parens{-\j 2 \pi \frac{r_{n,m}}{\lambda}} \label{eq:spherical-wave}
\end{align}
where $r_{n,m}$ is the distance between the $n$-th transmit antenna and the $m$-th receive antenna, $\lambda$ is the carrier wavelength, and $\rho$ is a normalizing factor to satisfy $\normfro{\mH}^2 = \Nt \cdot \Nr$.
To realize such a channel, we have vertically stacked our transmit and receive arrays with $10 \lambda$ of separation.
While this channel model may not hold perfectly in practice, it provides a sensible starting point to evaluate \lonestar, particularly when self-interference is dominated by idealized near-field propagation. % \footnote{Shortly, for more extensive evaluation, we consider a self-interference channel model that mixes this spherical-wave model with a Rayleigh faded channel.}
Shortly, for more extensive evaluation, we consider a self-interference channel model that mixes this spherical-wave model with a Rayleigh faded channel.
% In addition, it motivates the possibility that our design be executed on some deterministic or well estimated near-field model while treating imperfections (e.g., stemming from far-field reflections) as channel estimation error.
We do not model cross-link interference explicitly but instead evaluate it over various $\inrtx$.


% As such, we consider two channel models: (i) a Rayleigh-faded channel and (2) an idealized near-field model.
% To ensure the channels are compared fairly, they each satisfy $\ev{\normfro{\mH}^2} = \Nt \Nr$, meaning only their spatial characteristics dictate our design's ability to reduce the coupling of self-interference, rather than the energy contained therein.

% Our transmit and receive coverage regions are comprised of uniformly spaced points in azimuth from $-60^\circ$ to $60^\circ$ with $15^\circ$ spacing and in elevation from $-30^\circ$ to $30^\circ$ with $15^\circ$ spacing.
% This amounts to $\Mtx = \Mrx = 45$ total directions in $\dirtxset$ and $\dirrxset$.



% -------------------------------------------------------------------------------------------------
% Baselines.
% -------------------------------------------------------------------------------------------------
\subsection{Baselines and Performance Metrics}
Considering \lonestar is the first known codebook design specifically for \mmwave full-duplex, we evaluate it against two off-the-shelf codebooks, both of which are used in practice by half-duplex systems to form sets of beams that provide broad coverage with high gain:
\begin{itemize}
    \item A \textit{CBF codebook} that uses conjugate beamforming \cite{heath_lozano}, where
    \begin{align}
    % \vf_i = \atx{\dirtx\idx{i}}, \qquad \vw_j = \arx{\dirrx\idx{j}}.
    \vf_i = \project{\atx{\dirtx\idx{i}}}{\precb}, \qquad \vw_j = \project{\arx{\dirrx\idx{j}}}{\comcb}.
    \end{align}
    \cbf codebooks can deliver (approximately) maximum gain to all directions in $\txdirsetcb$ and $\rxdirsetcb$.
    The projections here are simply to ensure the beams are physically realizable and do not have significant impacts on the beam shapes with modest resolutions $\bitsphase$ and $\bitsamp$.
    \item A \textit{Taylor codebook} that uses conjugate beamforming with side lobe suppression as
    \begin{align}
    % \vf_i = \atx{\dirtx\idx{i}} \odot \vv, \qquad \vw_j = \arx{\dirrx\idx{j}} \odot \vv \\
    \vf_i = \project{\atx{\dirtx\idx{i}} \odot \vv_{\labeltx}}{\precb}, \qquad \vw_j = \project{\arx{\dirrx\idx{j}} \odot \vv_{\labelrx}}{\comcb}
    \label{eq:cbf-tay}
    \end{align}
    where $\vv_{\labeltx}$ and $\vv_{\labelrx}$ are Taylor windows applied element-wise, providing $25$ dB of side lobe suppression; we found this level of side lobe suppression competes best with \lonestar.
    Taylor windowing is an established means to reduce interference inflicted by side lobe levels at the cost of lessened beamforming gain and a wider main lobe \cite{taylor_1955,taylor_SAR_1995}.
\end{itemize}
% The projections here are simply to ensure the beams are physically realizable and do not have significant impacts on the beam shapes with modest resolutions $\bitsphase$ and $\bitsamp$.
% \cbf and Taylor codebooks are both used in practice to form sets of beams that provide broad coverage with high gain.
% The beam pattern of each conventional codebook is shown in \figref{fig:beams-a}.
% \cbf offers maximum beamforming gain with a narrow main lobe but exhibits high side lobe levels.
% Taylor windowing reduces the side lobe levels at the cost of lessened beamforming gain and a wider main lobe: with $25$ dB of side lobe suppression, beams sacrifice about $X$ dB in maximum gain.

% -------------------------------------------------------------------------------------------------
% Metrics.
% -------------------------------------------------------------------------------------------------
% \subsection{Performance Metrics}
% Given this full-duplex setting, 
We assess \lonestar against our baseline codebooks in terms of sum spectral efficiency of the transmit and receive links.
Specifically, we use the normalized sum spectral efficiency
\begin{align}
\sesumnorm = \frac{\setx + \serx}{\captxcb  + \caprxcb}
\end{align}
where $\captxcb$ and $\caprxcb$ we term the \textit{codebook capacities}, which are the individual capacities
\begin{align}
\captxcb = \logtwo{1 + \snrtxcbf}, \qquad \caprxcb = \logtwo{1 + \snrrxcbf}.
\end{align}
Here, $\snrtxcbf$ and $\snrrxcbf$ are the maximum \gpsnr delivered to a given downlink-uplink user pair by a CBF codebook.
In other words, $\captxcb + \caprxcb$ is the maximum sum spectral efficiency when using a \cbf codebook and interference is inherently not present (i.e., when $\inrrxbar = \inrtx = -\infty$ dB).
With this normalization, $\sesumnorm$ will gauge how well a given codebook delivers transmission and reception in the face of self-interference and cross-link interference, relative to the interference-free capacity when beamforming with a CBF codebook.
Note that $\sesumnorm = 0.5$ can be achieved with a \cbf codebook by half-duplexing transmission and reception with equal \gls{tdd}.
As such, \lonestar generally aims to exceed $\sesumnorm = 0.5$ and outperform that achieved by CBF and Taylor codebooks.
Note that $\sesumnorm$ is not truly upper-bounded by $1$ since $\captxcb + \caprxcb$ is not the true sum Shannon capacity; nonetheless, achieving $\sesumnorm \approx 1$ indicates near best-case full-duplex performance one can expect when using beamforming codebooks.
Having simulated our system in a Monte Carlo fashion, in our results we will present $\sesumnorm$ averaged over downlink-uplink user realizations. %  (i.e., ergodic sum spectral efficiency).

%We now provide a brief reminder to the reader of key parameters that we will evaluate our design against.
%\begin{itemize}
%    \item $\snrtxbar$: inherent strength of the transmit channel
%    \item $\snrrxbar$: inherent strength of the receive channel
%    \item $\inrrxbar$: inherent strength of the self-interference channel
%    \item $\inrtx$: the strength of cross-link interference, which $\lonestar$ has no impact on.
%    \item $\bitsphase$, $\bitsamp$: resolutions of the phase shifters and attenuators in the analog beamforming networks
%    \item $\sigmatx^2$, $\sigmarx^2$: tolerated transmit and receive coverage variances, a design parameter of \lonestar
%\end{itemize}

% The $\inr$ of a \mmwave full-duplex system depends on a variety of factors including transmit power, noise power, and system setup.
% The uplink and downlink spectral efficiencies are bounded by their Shannon capacities (neglecting self-interference on the uplink) with unconstrained beams $\vf$ and $\vw$.
% The sum spectral efficiency $\setx + \serx$ is bounded by the full-duplex capacity $\capfd$, the sum of the two Shannon capacities.
% Under equal \gls{tdd}, the half-duplex capacity is simply $\caphd = 0.5 \cdot \capfd$.
% Note that the use of beamforming codebooks will naturally fall short of these capacities.

%\begin{align}
%	\sinrrx = \frac{\snrrx}{1 + \inr}
%\end{align}

%\begin{align}
%R = \setx + \serx
%\end{align}

% -------------------------------------------------------------------------------------------------
% 0. Our beam patterns.
% -------------------------------------------------------------------------------------------------
\begin{figure*}
    \centering
    \subfloat[Conventional beams.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{plots/main_lonestar_v03_10}
        \label{fig:beams-a}}
    \quad
    \subfloat[\lonestar beams.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{plots/main_lonestar_v03_09}
        \label{fig:beams-b}}
    \caption{(a) The azimuth cut of a broadside beam from conventional \cbf and \taylor codebooks. (b) The azimuth cuts of transmit beams produced by \lonestar that serve various azimuth directions at an elevation of $0^\circ$.} % Here, $\sigmatxrxsq = X$ dB.}
    \label{fig:beams}
\end{figure*}

\subsection{Beam Patterns}
In \figref{fig:beams}, we compare conventional beams to those produced by \lonestar.
\figref{fig:beams-a} depicts the shape of beams from our two baseline codebooks.
CBF beams can each deliver maximum gain in their steered direction and exhibit a narrow main lobe and high side lobes.
With the \taylor codebook, these side lobes are reduced to $25$ dB below the main lobe, which itself sacrificed about $6$ dB in maximum gain for this side lobe suppression.
% Taylor windowing is commonly used to reduce interference inflicted by side lobes.
In \figref{fig:beams-b}, we plot transmit beams from a codebook produced by \lonestar; receive beams are similar.
Clearly, unlike the Taylor codebook, \lonestar does not attempt to merely shrink side lobes to reduce self-interference.
Instead, \lonestar makes use of side lobes, shaping them to cancel self-interference spatially, and while doing so, \lonestar maintains near maximum gain across its beams.

% ------------------------------------------------------------------------
% Plan.
% ------------------------------------------------------------------------

%A. Assume no estimation error to start.
%B. Assume spherical wave model to start.
%C. Assume INRtx = 0 dB or -Infty to start.
%
%0. Beam patterns.
%(a) CBF and Taylor steered broadside.
%(b) Our codebook azimuth cut.
%
%1. Choosing sigma; do not compare against conventional.
%(a) For fixed INRrx, bits: sum SE vs sigma sq for various SNR.
%(b) For fixed SNR, bits: sum SE vs INRrx for various sigma.
%
%2. Compare against conventional codebooks.
%(a) For fixed INRrx: sum SE as function of SNRtx = SNRrx for various bits.
%(b) For fixed SNRtx = SNRrx: sum SE as a function of INRrx for various bits.
%
%3. CDFs; compare against conventional.
%(a) INR reduction.
%(b) SINR gain.
%
%4. How does INRtx impact things; compare against conventional.
%(a) For fixed INRrx and bits, sum SE as function of INRtx for various SNRtx = SNRrx
%(b) For various SNRtx = SNRrx, contours as a function of (INRrx,INRtx).
%
%5. SNRtx not equal to SNRrx
%(a) Conventional: For fixed INRrx, INRtx, bits, sum SE as function of (SNRtx,SNRrx).
%(b) LoneSTAR: For fixed INRrx, INRtx, bits, sum SE as function of (SNRtx,SNRrx).
%
%6.
%(a) Show the impacts of estimation error.
%(b). Show the impacts of mixture model.

% -------------------------------------------------------------------------------------------------
% 1. Choosing sigma.
% -------------------------------------------------------------------------------------------------
\subsection{Choosing Coverage Variances, $\sigmatx^2$ and $\sigmarx^2$}


% Recall that the design parameters of \lonestar are the transmit and receive coverage variances $\sigmatx^2$ and $\sigmarx^2$.
In general, it is not possible to analytically state optimal choices for the design parameters $\sigmatx^2$ and $\sigmarx^2$ that maximize normalized sum spectral efficiency $\sesumnorm$.
This motivates us to first examine heuristically how to choose $\sigmatx^2$ and $\sigmarx^2$.
In \figref{fig:choosing-sigma-a}, we plot the normalized sum spectral efficiency $\sesumnorm$ as a function of $\sigmatx^2 = \sigmarx^2$ for various levels of self-interference $\inrrxbar$.
Here, we let $\snrtxbar = \snrrxbar = 10$ dB and have assumed no channel estimation error nor cross-link interference (i.e., $\eps^2 = -\infty$ dB, $\inrtx = -\infty$ dB).
At low self-interference $\inrrxbar$ (in black), there is inherently low coupling between the transmit and receive beams, meaning it is best to maintain high beamforming gain rather than reduce self-interference further.
This makes a low coverage variance optimal on average, shown as the $\star$ at $\sigmatx^2 = \sigmarx^2 = -40$ dB.
As $\inrrxbar$ increases, \lonestar benefits from having greater transmit and receive coverage variance since it affords more flexibility to reduce self-interference and increase the sum spectral efficiency.
The non-smooth nature to the sum spectral efficiency in \figref{fig:choosing-sigma-a} is largely due to the non-convexity posed by limited phase and amplitude control.

\begin{figure*}
    \centering
    \subfloat[As a function of coverage variance, $\sigmatx^2 = \sigmarx^2$.]{\includegraphics[width=\linewidth,height=0.265\textheight,keepaspectratio]{plots/main_lonestar_v03_01_02}
        \label{fig:choosing-sigma-a}}
    \quad
    \subfloat[As a function of self-interference strength, $\inrrxbar$.]{\includegraphics[width=\linewidth,height=0.265\textheight,keepaspectratio]{plots/main_lonestar_v03_01_03}
        \label{fig:choosing-sigma-b}}
    \caption{Normalized sum spectral efficiency $\sesumnorm$ (a) as a function of the coverage variance $\sigmatx^2 = \sigmarx^2$ for various $\inrrxbar$; and (b) as a function of self-interference strength $\inrrxbar$ for various $\sigmatxrxsq$. In both, $\snrtxbar = \snrrxbar = 10$ dB, $\bitsphase = \bitsamp = 8$ bits, $\inrtx = -\infty$ dB, and $\epsilon^2 = -\infty$ dB. Performance with the optimal $\sigmatxrxsq$ is denoted with $\star$.}
    % \caption{1. Choosing $\sigmatx^2 = \sigmarx^2$. (a) $\snrtxbar = \snrrxbar = 10$ dB, $\bitsphase = \bitsamp = 8$ bits, $\inrtx = -\infty$ dB, $\epsilon^2 = -\infty$ dB. (b) $\snrtxbar = \snrrxbar = 10$ dB, $\bitsphase = \bitsamp = 8$ bits, $\inrtx = -\infty$ dB, $\epsilon^2 = -\infty$ dB.}
    \label{fig:choosing-sigma}
\end{figure*}

In \figref{fig:choosing-sigma-b}, we highlight this further by plotting the normalized sum spectral efficiency as a function of $\inrrxbar$ for various $\sigmatx^2 = \sigmarx^2$.
Naturally, one may independently choose $\sigmatx^2$ and $\sigmarx^2$, rather than assume them equal as we have done here for simplicity; this can therefore be considered a conservative evaluation of \lonestar.
The starred curve represents tuning $\sigmatx^2 = \sigmarx^2$ at each $\inrrxbar$ to maximize sum spectral efficiency.
At very low $\inrrxbar$, full-duplex operation ``is free'', as transmit and receive beams couple sufficiently low self-interference on their own.
In this region, minimizing the coverage variance $\sigmatx^2 = \sigmarx^2$ is ideal since it preserves near-maximum $\snrtx$ and $\snrrx$.
As $\inrrxbar$ increases, increasing $\sigmatx^2 = \sigmarx^2$ supplies the system with greater robustness to self-interference, evidenced by the rightward shift of the curves.
When $\inrrxbar$ is overwhelmingly high, \lonestar cannot mitigate self-interference enough, succumbing to self-interference and offering at most around $\sesumnorm = 0.5$ (essentially half-duplexing).
% Notice that under very high self-interference $\inrrxbar$, 
Notice that in this region, it is optimal to return to using very low  $\sigmatx^2 = \sigmarx^2$ in order to preserve half-duplex performance at worst by maximizing \gsnr.
Clearly, choosing $\sigmatx^2 = \sigmarx^2$ is an important design decision and depends heavily on system factors (chiefly $\inrrxbar$).
In practice, we imagine a system relying on a lookup table to retrieve the optimal $\sigmatx^2$ and $\sigmarx^2$ based on its measured $\inrrxbar$ (along with other system factors), which would likely depend on simulation and experimentation. % field trials.
Henceforth, we assume that the optimal $\sigmatxrxsq$ is used which maximizes $\sesumnorm$.
% Naturally, one may independently choose $\sigmatx^2$ and $\sigmarx^2$ rather than assume them equal as we have done here for simplicity; this can therefore be considered a conservative evaluation of \lonestar.
% Comment on SNR.



% -------------------------------------------------------------------------------------------------
% 2. Comparing against conventional.
% -------------------------------------------------------------------------------------------------
\subsection{Comparing \lonestar Against Off-The-Shelf Codebooks}


Now, in \figref{fig:compare}, we compare \lonestar codebooks against two off-the-shelf codebooks: the \cbf and \taylor codebooks defined before as baselines. 
% Henceforth, unless specified otherwise, we assume $\snrtxbar = \snrrxbar = 10$ dB, $\inrrxbar = 90$ dB\footnote{We commonly use $\inrrxbar = 90$ dB since this produces a median $\inrrx$ with the \cbf codebook that aligns with our \ginr measurements using an actual $28$ GHz phased array platform in \cite{roberts_att_angular}.}, no cross-link interference ($\inrtx = -\infty$ dB), and no channel estimation error ($\eps^2 = -\infty$ dB); we will evaluate \lonestar against all of these shortly.
We assume no cross-link interference ($\inrtx = -\infty$ dB) and no channel estimation error ($\eps^2 = -\infty$ dB); we will evaluate \lonestar against both of these shortly.
In \figref{fig:compare-a}, we plot the normalized sum spectral efficiency $\sesumnorm$ achieved by \lonestar as a function of $\snrtxbar = \snrrxbar$ for various resolutions $\bitsphase = \bitsamp$, where $\inrrxbar = 90$ dB\footnote{We commonly use $\inrrxbar = 90$ dB since this produces a median $\inrrx$ with the \cbf codebook that aligns with our \ginr measurements using an actual $28$ GHz phased array platform in \cite{roberts_att_angular}.}. % ; here, \lonestar uses the tuned (optimal) $\sigmatxrxsq$.
% In \figref{fig:compare-a}, we plot the normalized sum spectral efficiency $\sesumnorm$ achieved by \lonestar as a function of $\snrtxbar = \snrrxbar$ for various resolutions $\bitsphase = \bitsamp$; here, \lonestar uses the tuned (optimal) $\sigmatxrxsq$, $\inrrxbar = 90$ dB, and $\inrtx = -\infty$ dB.
The dashed black curve denotes the \cbf codebook and the dashed red curve denotes the \taylor codebook, both of which are configured with $\bitsphaseamp = 8$ bits.
At low $\snrtxrxbar$, the \cbf codebook can deliver $\sesumnorm \approx 0.5$, since the receive link is overwhelmed by self-interference while the transmit link sees nearly full beamforming gain.
The \taylor codebook sacrifices beamforming gain to reduce its side lobes and therefore achieves only $\sesumnorm \approx 0.46$ at low $\snrtxrxbar$, suggesting that it is also plagued by self-interference at this particular $\inrrxbar$, even with reduced side lobes.
As $\snrtxrxbar$ increases, \cbf and \taylor codebooks naturally both improve their performance as the impacts of self-interference diminish with increased \gsnr.
Shown as solid lines, \lonestar improves significantly as $\bitsphaseamp$ increases from $4$ bits to $8$ bits. % , though with diminishing gains.
At low $\snrtxrxbar$, \lonestar can deliver sum spectral efficiencies well above that of off-the-shelf codebooks by better rejecting self-interference while maintaining high beamforming gain.
This is especially true when $\bitsphaseamp \geq 6$ bits, which allows \lonestar to deliver upwards of $90$\% of the full-duplex codebook capacity.
At high $\snrtxrxbar$, \lonestar naturally improves, saturating due to diminishing gains in $\logtwo{1+x}$.
For $\snrtxrxbar \geq 5$ dB, the \taylor codebook can significantly outperform the \cbf codebook and can marginally outperform \lonestar having only $\bitsphaseamp = 4$ bits, especially at high \gsnr.
Here, it is clear that limited resolution bottlenecks \lonestar. % , though it should be noted that the \taylor codebook has been allotted $\bitsphaseamp = 8$ bits for illustration.

\begin{figure*}
    \centering
    \subfloat[As a function of link quality, $\snrtxbar = \snrrxbar$.]{\includegraphics[width=\linewidth,height=0.265\textheight,keepaspectratio]{plots/main_lonestar_v03_02_12}
        \label{fig:compare-a}}
    \quad
    \subfloat[As a function of self-interference strength, $\inrrxbar$.]{\includegraphics[width=\linewidth,height=0.261\textheight,keepaspectratio]{plots/main_lonestar_v03_01_07}
        \label{fig:compare-b}}
    \caption{Normalized sum spectral efficiency $\sesumnorm$ (a) as a function of $\snrtxbar = \snrrxbar$ where $\inrrxbar = 90$ dB; (b) as a function of $\inrrxbar$ where $\snrtxbar = \snrrxbar = 10$ dB. In both, $\inrtx = -\infty$ dB, $\epsilon^2 = -\infty$ dB, and $\sigmatx^2 = \sigmarx^2$ are tuned to maximize sum spectral efficiency. \cbf and \taylor codebooks are each with $\bitsphaseamp = 8$ bits.}
    % \caption{2. Compare against conventional. (a) $\inrrxbar = 90$ dB, $\inrtx = -\infty$ dB, $\epsilon^2 = -\infty$ dB, tuned $\sigmatx^2 = \sigmarx^2$, conventional are $8$ bits in both. (b) $\snrtxbar = \snrrxbar = 10$ dB, $\inrtx = -\infty$ dB, $\epsilon^2 = -\infty$ dB, tuned $\sigmatx^2 = \sigmarx^2$.}
    \label{fig:compare}
\end{figure*}

In \figref{fig:compare-b}, we now fix $\snrtxrxbar = 10$ dB and vary $\inrrxbar$, keeping all other factors the same as in \figref{fig:compare-a}.
\cbf and \lonestar both can nearly reach the full-duplex codebook capacity at low $\inrrxbar$, where self-interference is negligible and near maximal beamforming gain can be delivered.
The \taylor codebook sacrifices beamforming gain for reduced side lobes and therefore falls well short of $\sesumnorm = 1$ even in the presence of extremely weak self-interference. % at extremely low $\inrrxbar$.
As $\inrrxbar$ is increased, \cbf quickly succumbs to self-interference, whereas \lonestar proves to be notably more robust to such.
In fact, with each unit increase in resolution $\bitsphaseamp$, \lonestar supplies around $10$ dB of added robustness to self-interference.
The \taylor codebook can outperform the \cbf codebook but only for $\inrrxbar \in \brackets{72,100}$ dB before also being overwhelmed by self-interference.
At higher \gsnr, when $\snrtxrxbar \geq 10$ dB, this $\inrrxbar$ range would widen, as evidenced by \figref{fig:compare-a}.
As $\inrrxbar$ increases to extremely high levels, \lonestar converges to offer nearly the same sum spectral efficiency as \cbf of $\sesumnorm = 0.5$, essentially only serving the downlink user due to uplink being overwhelmed by self-interference.
% It is important to note that $\inrrxbar$ depends on the particular \mmwave platform, and as such, each full-duplex \mmwave \bs will see a unique $\inrrxbar$, making \lonestar an attractive codebook design since it is more robust than off-the-shelf codebooks over a wide range of $\inrrxbar$.
Each full-duplex \mmwave \bs will see a unique $\inrrxbar$ depending on a variety of parameters including transmit power, noise power, and, most importantly, the isolation between its transmit and receive arrays.
This makes \lonestar an attractive codebook design since it is more robust than off-the-shelf codebooks over a wide range of $\inrrxbar$ and provides greater flexibility when designing full-duplex \mmwave platforms.
Systems employing \lonestar can operate at higher $\inrrxbar$, meaning they can potentially increase transmit power without being severely penalized by increased self-interference, for instance.

% -------------------------------------------------------------------------------------------------
% 3. 
% -------------------------------------------------------------------------------------------------
%\begin{figure*}
%    \centering
%    \subfloat[Caption a.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{plots/main_lonestar_v03_14}
%        \label{fig:inr-tx-a}}
%    \quad
%    \subfloat[Caption b.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{plots/main_lonestar_v03_14}
%        \label{fig:compare-b}}
%    \caption{X. Compare against conventional. (a) $\snrtxbar = \snrrxbar = 10$ dB, $\inrrxbar = 90$ dB, $\epsilon^2 = -\infty$ dB, tuned $\sigmatx^2 = \sigmarx^2$, conventional are $8$ bits in both, \lonestar hits a floor because it's better to just give up on transmitting at high $\inrtx$ and since $\sigmatx^2 = \sigmarx^2$ are tied together, we also shut of receiver, perhaps tuning $\sigmatx^2$ and $\sigmarx^2$ separately would be best in cases like this. The bend at like 11 dB is due to choosing optimal sigma over discrete set. (b) }
%    \label{fig:subfigs}
%\end{figure*}

% -------------------------------------------------------------------------------------------------
% 3. SNR heatmap.
% -------------------------------------------------------------------------------------------------
\subsection{For Various Link Qualities, $\parens{\snrtxbar,\snrrxbar}$}

\begin{figure*}
    \centering
    \subfloat[Taylor codebook.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{plots/main_lonestar_v03_03_02}
        \label{fig:heatmap-snr-a}}
    \quad
    \subfloat[\lonestar codebooks.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{plots/main_lonestar_v03_03_01}
        \label{fig:heatmap-snr-b}}
    \caption{Normalized sum spectral efficiency $\sesumnorm$ as a function of $\parens{\snrtxbar,\snrrxbar}$ for the (a) Taylor codebook ($\bitsphaseamp = 8$ bits) and (b) \lonestar codebooks, where $\inrrxbar = 90$ dB, $\inrtx = -\infty$ dB, $\bitsphaseamp = 6$ bits, and $\eps^2 = -\infty$ dB. \lonestar delivers higher $\sesumnorm$ broadly across \gpsnr and demands lower \gpsnr to net $\sesumnorm \geq 0.5$.}
    \label{fig:heatmap-snr}
\end{figure*}

Rather than assume symmetric downlink/uplink quality $\snrtxrxbar$, we now consider $\snrtxbar \neq \snrrxbar$.
In \figref{fig:heatmap-snr-a}, we show the normalized sum spectral efficiency achieved by the \taylor codebook as a function of $\parens{\snrtxbar,\snrrxbar}$, where $\inrrxbar = 90$ dB and $\bitsphaseamp = 8$ bits.
In \figref{fig:heatmap-snr-b}, we show that of \lonestar with $\bitsphaseamp = 6$ bits. 
We chose to compare against the \taylor codebook rather than the \cbf codebook because it better competes with \lonestar at $\inrrxbar = 90$ dB (see \figref{fig:compare-a}).
Clearly, \lonestar can deliver higher spectral efficiencies than the \taylor codebook broadly over $\parens{\snrtxbar,\snrrxbar}$.
It is important to notice that the region where $\sesumnorm \geq 0.5$---where full-duplexing is superior to half-duplexing with equal \tdd---grows significantly with \lonestar versus the \taylor codebook.
This means that full-duplex operation is justified over a much broader range of $\parens{\snrtxbar,\snrrxbar}$ with \lonestar compared to with off-the-shelf codebooks.
It is also important to notice that \lonestar introduces a significant \gsnr gain versus off-the-shelf codebooks since it demands a much lower $\parens{\snrtxbar,\snrrxbar}$ to achieve a desired sum spectral efficiency $\sesumnorm$.
% In general, to achieve a desired sum spectral efficiency, \lonestar can be thought of as introducing a significant \gsnr gain over conventional codebooks.
Note that we have tuned $\sigmatxrxsq$, meaning the performance of \lonestar may improve if $\sigmatxsq$ and $\sigmarxsq$ were tuned separately, especially with highly asymmetric \gpsnr.

% -------------------------------------------------------------------------------------------------
% 4. INR heatmap.
% -------------------------------------------------------------------------------------------------
\subsection{For Various Levels of Interference, $\parens{\inrtx,\inrrxbar}$}

\begin{figure*}
    \centering
    \subfloat[Taylor codebook.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{plots/main_lonestar_v03_04_02}
        \label{fig:heatmap-inr-a}}
    \quad
    \subfloat[\lonestar codebook.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{plots/main_lonestar_v03_04_01}
        \label{fig:heatmap-inr-b}}
    \caption{Normalized sum spectral efficiency $\sesumnorm$ as a function of $\parens{\inrtx,\inrrxbar}$ for the (a) Taylor codebook, where $\bitsphaseamp = 8$ bits; and (b) \lonestar codebooks, where $\bitsphaseamp = 6$ bits. In both, $\snrtxrxbar = 10$ dB and $\eps^2 = -\infty$ dB. \lonestar is more robust to self-interference and cross-link interference than off-the-shelf codebooks.}
    \label{fig:heatmap-inr}
\end{figure*}

Similar to \figref{fig:heatmap-snr}, we now compare the \taylor codebook against \lonestar for various $\parens{\inrtx,\inrrxbar}$ in \figref{fig:heatmap-inr}, where we have fixed $\snrtxrxbar = 10$ dB.
Again, \lonestar can clearly deliver much higher spectral efficiencies than the \taylor codebook, achieving nearly the full-duplex codebook capacity when cross-link interference and self-interference are both low.
Even at very low \gpinr, the \taylor codebook cannot approach $\sesumnorm = 1$ since it sacrificed beamforming gain for side lobe suppression.
At high \gpinr, both \lonestar and the \taylor codebook struggle to deliver high $\sesumnorm$, largely due to the fact that neither can reduce cross-link interference.
In between, at moderate \gpinr, \lonestar can sustain spectral efficiencies notably higher than the \taylor codebook.
\lonestar's added robustness to cross-link interference and self-interference is on display here, as it can tolerate higher $\parens{\inrtx,\inrrxbar}$ than the \taylor codebook while delivering the same $\sesumnorm$.
% This is thanks to its ability to net higher receive link spectral efficiency, leading to a higher sum spectral efficiency.
This is thanks to \lonestar's ability to net a higher receive link spectral efficiency, which it can then sacrifice in the presence of high cross-link interference $\inrtx$.
At an $\inrrxbar = 50$ dB, for example, \lonestar provides around $10$ dB of robustness to $\inrtx$ for $\sesumnorm = 0.7$, compared to the \taylor codebook.
At an $\inrtx = -10$ dB, \lonestar provides around $30$ dB of robustness to self-interference $\inrrxbar$ for $\sesumnorm = 0.7$.
% As both cross-link interference and self-interference are driven extremely high, \lonestar struggles to deliver $\sesumnorm \geq 0.5$, highlighting conditions where half-duplexing is superior to full-duplexing with \lonestar.

% -------------------------------------------------------------------------------------------------
% 5. Channel estimation error and mixture.
% -------------------------------------------------------------------------------------------------
\subsection{Impacts of Channel Estimation Error}

\begin{figure*}
    \centering
    \subfloat[Channel estimation error.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{plots/main_lonestar_v03_process_06_01}
        \label{fig:mixture-error-a}}
    \quad
    \subfloat[Gaussian mixing.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{plots/main_lonestar_v03_process_05_01}
        \label{fig:mixture-error-b}}
    \caption{Normalized sum spectral efficiency as a function of (a) self-interference channel estimation error variance $\eps^2$ and (b) mixing variance $\zeta^2$. In both, $\snrtxbar = \snrrxbar = 10$ dB, $\inrrxbar = 90$ dB, and $\inrtx = -\infty$ dB. The true channel $\mH$ is distributed the same in both, but in (b), we assume perfect channel knowledge, $\eps^2 = -\infty$ dB.}
    \label{fig:mixture-error}
\end{figure*}

Now, in \figref{fig:mixture-error-a}, we examine the impacts of imperfect self-interference channel knowledge, $\eps^2 > -\infty$ dB.
To do so, we model $\mHbar$ as in \eqref{eq:spherical-wave}, meaning the true channel $\mH$ is Gaussian distributed about $\mHbar$ according to \eqref{eq:channel}.
We chose to model it in this fashion, rather than use $\mH$ as the spherical-wave model in \eqref{eq:spherical-wave}, for two reasons.
First, it is more challenging for \lonestar to face a channel under this mixed model (as we will see shortly in \figref{fig:mixture-error-b}).
Second, it represents the potential case where the estimate $\mHbar$ is computed directly based on the relative geometry of the transmit and receive arrays using the spherical-wave model (which can be done \textit{a priori}) and the estimation error captures deviations from this assumed spherical-wave behavior.
In \figref{fig:mixture-error-a}, we plot the normalized sum spectral efficiency as a function of self-interference channel estimation error variance $\epsilon^2$.
With accurate estimation of $\mH$, \lonestar performs quite well as it has proven thus far.
As the quality of estimation degrades, \lonestar has difficulty reliably avoiding self-interference.
Its performance suffers but remains well above $\sesumnorm = 0.5$ before converging to performance offered by the \cbf codebook around $\eps^2 = -30$ dB.
The \cbf codebook sees mild degradation with increased estimation error.
Clearly, the \taylor codebook, like \lonestar, suffers as $\eps^2$ increases. % from a channel that is increasingly Gaussian.
It may seem strange that the \cbf and \taylor codebooks both vary as a function of estimation error $\eps^2$ since neither codebook depends on self-interference channel knowledge \textit{a priori}.
This can be explained by the fact that the estimation error $\mDelta$ is distributed differently than the estimate $\mHbar$.
In other words, the \taylor codebook is inherently more robust to a spherical-wave self-interference channel than a Gaussian one.
Gaussian-distributed error proves to be especially difficult for \lonestar and \taylor to endure,  compared to the more structured spherical-wave channel.
As such, it is evident that the lack of channel knowledge \textit{and} the fact that estimation error is Gaussian contributes to \lonestar's degradation as $\eps^2$ increases.

% To further dissect the impacts of estimation error versus that of mixing the spherical-wave model with a Gaussian matrix, we introduce a new self-interference channel model and examine its performance in \figref{fig:mixture-error-b}.
% We consider the following mixed self-interference channel model
We dissect the impacts of estimation error versus that of mixing the spherical-wave model with a Gaussian matrix in \figref{fig:mixture-error-b} by considering the mixed self-interference channel model
\begin{align}
% \mH = \frac{\mH_{\mathrm{SW}} + \zeta \cdot \mH_{\mathrm{Ray}}}{\normfro{\mH_{\mathrm{SW}} + \zeta \cdot \mH_{\mathrm{Ray}}}} \cdot \sqrt{\Nt\cdot\Nr} \label{eq:mixture}
\mH = \frac{\mH_{\mathrm{SW}} + \mH_{\mathrm{Ray}}}{\normfro{\mH_{\mathrm{SW}} + \mH_{\mathrm{Ray}}}} \cdot \sqrt{\Nt\cdot\Nr}, \qquad \entry{\mH_{\mathrm{Ray}}}{m,n} \sim \distcgauss{0}{\zeta^2} \ \forall \ m,n \label{eq:mixture}
\end{align}
where $\mH_{\mathrm{SW}}$ is the spherical-wave model defined in \eqref{eq:spherical-wave} and $\mH_{\mathrm{Ray}}$ is Rayleigh faded with variance $\zeta^2$.
%\begin{align}
%% \mH = \frac{\mH_{\mathrm{SW}} + \zeta \cdot \mH_{\mathrm{Ray}}}{\normfro{\mH_{\mathrm{SW}} + \zeta \cdot \mH_{\mathrm{Ray}}}} \cdot \sqrt{\Nt\cdot\Nr} \label{eq:mixture}
%\mH = \frac{\mH_{\mathrm{SW}} + \mH_{\mathrm{Ray}}}{\normfro{\mH_{\mathrm{SW}} + \mH_{\mathrm{Ray}}}} \cdot \sqrt{\Nt\cdot\Nr} \label{eq:mixture}
%\end{align}
%where $\mH_{\mathrm{SW}}$ is the spherical-wave model defined in \eqref{eq:spherical-wave} and $\mH_{\mathrm{Ray}}$ is Rayleigh faded as 
%% $\entry{\mH_{\mathrm{Ray}}}{m,n} \sim \distcgauss{0}{1} \ \forall \ m,n$.
%\begin{align}
%\entry{\mH_{\mathrm{Ray}}}{m,n} \sim \distcgauss{0}{\zeta^2} \ \forall \ m,n.
%\end{align}
The scaling in \eqref{eq:mixture} simply ensures $\normfro{\mH}^2 = \Nt\cdot\Nr$.
We evaluate \lonestar using this channel model for various $\zeta^2$, which we term the \textit{mixing variance}.
In doing so, we assume perfect knowledge of the realized channel $\mH$ (i.e., $\eps^2 = -\infty$ dB) to solely investigate the effects of this mixing.
The spherical-wave channel $\mH_{\mathrm{SW}}$ is a highly structured channel based on the relative geometry between the transmit and receive arrays at the \bs.
The Rayleigh faded channel $\mH_{\mathrm{Ray}}$ (a Gaussian matrix) lay at the other extreme, lacking any inherent structure.
At $\zeta^2 = 0$ dB, the channel is virtually equal parts spherical-wave and Rayleigh faded.
It is important to notice that the distribution of true channel $\mH$ here is identical to that examined in \figref{fig:mixture-error-a}.
% In this case, however, we examine $\eps^2 = -\infty$ dB to investigate the impacts of imperfect channel knowledge versus that of $\mH$ becoming increasingly Gaussian.
In this case, however, we examine $\eps^2 = -\infty$ dB to investigate the impacts of $\mH$ becoming increasingly Gaussian, rather than those stemming from imperfect channel knowledge.

In \figref{fig:mixture-error-b}, we plot the normalized sum spectral efficiency as a function of the mixing variance $\zeta^2$. 
Having considered perfect channel knowledge $\eps^2 = -\infty$ dB here, \figref{fig:mixture-error-b} is an upper bound on \figref{fig:mixture-error-a} since they follow the same channel model.
At very low $\zeta^2$, $\mH \approx \mH_{\mathrm{SW}}$, allowing \lonestar to achieve appreciable spectral efficiencies above off-the-shelf codebooks, as we have seen thus far. % , nearing the codebook capacity with high $\bitsphaseamp$.
As $\zeta^2$ increases, the sum spectral efficiency offered by \lonestar tends to decrease, though so does the \taylor codebook and the \cbf codebook slightly so.
At high $\zeta^2$, \lonestar suffers since it cannot find ways to pack the transmit and receive beams such that they do not couple across the self-interference channel.
This is intimately related to the fact that Gaussian matrices (almost surely) tend to inflict self-interference across all dimensions of $\mH$, making it a statistically more difficult channel for \lonestar to build codebooks that minimize transmit-receive beam coupling.
Thus, we can conclude that, even with perfect channel estimation, \lonestar struggles with self-interference channels that are heavily Gaussian.
From the results in \figref{fig:mixture-error}, we observe that there is the need for accurate and perhaps frequent self-interference channel estimation.
% Clearly, there is the need for accurate and perhaps frequent self-interference channel estimation, and
Our hope is that this can be accomplished by taking advantage of the strength of the self-interference channel, along with a potentially known channel structure and occasional, but thorough, measurements at the \bs.
\figref{fig:mixture-error} also motivates further investigation of the statistical limitations of \lonestar---along with beamforming-based full-duplex solutions in general---based on the distribution of the self-interference channel and its estimation error.
% Investigating the statistics and limitations of \lonestar further---along with beamforming-based full-duplex solutions in general---for a variety of self-interference channel models would be excellent future work.
% Clearly, 

% ---

% These results highlight a few important takeaways.
% First, \lonestar can perform quite well on structured channels with low self-interference channel estimation error.
% It struggles, however, when with significant estimation errors that are Gaussian distributed.
% This is due in part to the fact that the errors are Gaussian distributed and that there is uncertainty in the self-interference channel.


% As mentioned, there does not currently exist a measurement-backed self-interference channel model, and we have used the spherical-wave channel model in \eqref{eq:spherical-wave} as a sensible starting point to evaluate \lonestar.
% Now, to further evaluate \lonestar against a more general channel model, we consider the following mixed self-interference channel model
% \begin{align}
% % \mH = \frac{\mH_{\mathrm{SW}} + \zeta \cdot \mH_{\mathrm{Ray}}}{\normfro{\mH_{\mathrm{SW}} + \zeta \cdot \mH_{\mathrm{Ray}}}} \cdot \sqrt{\Nt\cdot\Nr} \label{eq:mixture}
% \mH = \frac{\mH_{\mathrm{SW}} + \mH_{\mathrm{Ray}}}{\normfro{\mH_{\mathrm{SW}} + \mH_{\mathrm{Ray}}}} \cdot \sqrt{\Nt\cdot\Nr} \label{eq:mixture}
% \end{align}
% where $\mH_{\mathrm{SW}}$ is the spherical-wave model defined in \eqref{eq:spherical-wave} and  $\mH_{\mathrm{Ray}}$ is a Rayleigh faded channel distributed as 
% % $\entry{\mH_{\mathrm{Ray}}}{m,n} \sim \distcgauss{0}{1} \ \forall \ m,n$.
% \begin{align}
% \entry{\mH_{\mathrm{Ray}}}{m,n} \sim \distcgauss{0}{\zeta^2} \ \forall \ m,n.
% \end{align}
%The scaling in \eqref{eq:mixture} simply ensures $\normfro{\mH}^2 = \Nt\cdot\Nr$.
%We reevaluate \lonestar using this channel model for various $\zeta^2$, the variance of each element in $\mH_{\mathrm{Ray}}$, which we term the \textit{mixing variance}.
%The spherical-wave channel $\mH_{\mathrm{SW}}$ is a highly structured channel based on the relative geometry between the transmit and receive arrays at the \bs, whereas the Rayleigh faded channel $\mH_{\mathrm{Ray}}$ is at the other extreme, lacking any inherent structure.
%% This mixing effectively inflicts self-interference across all dimensions of $\mH$ (almost surely), making it a potentially more difficult channel for \lonestar to operate on.



%The insights are twofold.
%1. To evaluate \lonestar against a more general channel model.
%2. To investigate the impacts of the channel structure on the degraded performance of \lonestar with increased $\epsilon^2$. In (b), we use a mixture model that is similar to our estimation error distribution but assume we have perfect knowledge of the mixed self-interference channel.
%Some other distributions may be less troublesome for \lonestar. Gaussian is particularly difficult to avoid even with channel knowledge because it tends (almost surely) to inflict self-interference across all spatial dimensions of $\mH$, making it a potentially more difficult channel for \lonestar to operate on.
%The effects we see in \figref{fig:mixture-error-a} are due to (i) errors in self-interference channel knowledge and (ii) the fact that the errors are distributed as Gaussian.


==> sec-solving.tex <==
\section{Solving our Codebook Design Problem} % \label{sec:contribution-ii}

Having arrived at our design problem \eqref{eq:problem-i}, we now set out to solve for our design.
The non-convexity posed by digitally controlled phase shifters and attenuators, captured by \eqref{eq:problem-quantize-tx-1} and \eqref{eq:problem-quantize-rx-1}, presents difficulty in solving this problem.
%  problem \eqref{eq:problem-full-3} is non-convex due to the limited resolution of our digitally-controlled phase shifters and attenuators used for analog beamforming, captured by \eqref{eq:problem-quantize-tx-3} and \eqref{eq:problem-quantize-rx-3}.
% \edit{Is the objective jointly convex?}
In general, we found that we cannot handle this non-convexity well by merely ignoring it, solving, and then projecting the solutions $\precbmat\opt$ and $\comcbmat\opt$ onto $\precb$ and $\comcb$, respectively, though this may offer reasonable results when $\bitsphase$ and $\bitsamp$ are sufficiently high.
To present a general approach to handling this non-convexity, we present the following alternating minimization with the understanding that more sophisticated algorithms may enhance the results we observe in \secref{sec:simulation-results}.

We define $\project{\vf}{\precb}$ as the projection of a beamforming vector $\vf$ onto the set $\precb$ and extend this to matrices as $\project{\mF}{\precb}$, which acts column-wise on $\mF$.
Our algorithm begins by initializing $\precbmat$ and $\comcbmat$ as the projections of scaled $\Atx$ and $\Arx$ onto $\precb$ and $\comcb$, respectively, quantizing their entries to have phase and amplitude resolutions $\bitsphase$ and $\bitsamp$.
% That is, $\precbmat \leftarrow \project{\Atx \cdot \Deltatx}{\precb}$ and $\comcbmat \leftarrow \project{\Arx \cdot \Deltarx}{\comcb}$, which initializes our beams to achieve gains $\Gtxtgt^2$ and $\Grxtgt^2$ across $\dirtxset$ and $\dirrxset$, respectively.
That is, 
\begin{gather}
\precbmat \leftarrow \project{\Atx}{\precb} \\
\comcbmat \leftarrow \project{\Arx}{\comcb} 
\end{gather}
which initializes our beams as matched filters to achieve gains $\Nt^2$ and $\Nr^2$ across $\dirtxset$ and $\dirrxset$, respectively.
% This 

In this approach, we approximately solve problem \eqref{eq:problem-i} by solving for the codebooks beam-by-beam. 
We separate problem \eqref{eq:problem-i} into problems \eqref{eq:problem-full-4a} and \eqref{eq:problem-full-4b} below, which solve for the $i$-th transmit beam and $j$-th receive beam, respectively.
Problems \eqref{eq:problem-full-4a} and \eqref{eq:problem-full-4b} are convex since they remove the hardware constraints and can be readily solved using a convex solver (we used \cite{cvx}).
We solve for the $i$-th transmit beam $\vf_i$ in problem \eqref{eq:problem-full-4a}, starting with $i=1$ and the initialized $\comcbmat$.
Note that we have introduced the constraint \eqref{eq:problem-entry-tx-4a} to ensure our beamforming weights can be implemented using attenuators.
\begin{subequations} \label{eq:problem-full-4a}
	\begin{align}
	\vf_i\opt = \arg \min_{\vf_i} &\ \normtwo{\comcbmat\ctrans \mH \vf_i} \label{eq:problem-objective-4a} \\
	\st 
	&\ \bars{\Nt - \atx{\dirtx\idx{i}}\ctrans \vf_i}^2 \leq \sigmatx^2 \cdot \Nt^2 \label{eq:problem-coverage-tx-4a} \\
	&\ \bars{\entry{\vf_i}{n}} \leq 1 \ \forall \ n = 1, \dots, \Nt \label{eq:problem-entry-tx-4a}
	\end{align}
\end{subequations}
Then, the solution $\vf_i\opt$ is projected onto the set $\precb$ before updating it in the matrix $\precbmat$ to ensure it is physically realizable.
\begin{align}
\entry{\precbmat}{:,i} \leftarrow \project{\vf_i\opt}{\precb}
\end{align}
The updated $\precbmat$ is then used when solving for the $j$-th receive beam (beginning with $j=1$) in problem \eqref{eq:problem-full-4b}.
\begin{subequations} \label{eq:problem-full-4b}
	\begin{align}
	\vw_j\opt = \arg \min_{\vw_j} &\ \normtwo{\vw_j\ctrans \mH \precbmat}  \label{eq:problem-objective-4b} \\
	\st 
	&\ \bars{\Nr - \arx{\dirrx\idx{j}}\ctrans \vw_j}^2 \leq \sigmarx^2 \cdot \Nr^2 \label{eq:problem-coverage-rx-4b} \\
	&\ \bars{\entry{\vw_j}{n}} \leq 1 \ \forall \  = 1, \dots, \Nr \label{eq:problem-entry-rx-4b} 
	\end{align}
\end{subequations}
The solution $\vw_j\opt$ is then projected onto $\comcb$ before updating $\comcbmat$.
\begin{align}
\entry{\comcbmat}{:,j} \leftarrow \project{\vw_j\opt}{\comcb}
\end{align}
We iteratively solve for the $(i+1)$-th transmit beam and then the $(j+1)$-th receive beam until all $\Mtx$ and $\Mrx$ beams are solved for.
% When $\Mtx = \Mrx$, the transmit and receive beams can be solved one after another.
When $\Mtx \neq \Mrx$, the remaining transmit/receive beams can be solved for after $\minop{\Mtx,\Mrx}$ iterations.
We have found that this iterative approach handles the quantization of $\precbmat$ and $\comcbmat$ quite well by \textit{progressively} incorporating quantization beam-by-beam, allowing later beams to account for the quantization imposed on earlier beams.
% Additionally, by alternating between transmit and receive beams $\vf_i$ and $\vw_j$ rather than between the \textit{entire} codebooks $\precbmat$ and $\comcbmat$, this approach ensures the burden of reducing self-interference is not biased to one codebook or the other but rather distributed more evenly across all beams.
% One of the artifacts of this design it does not jointly utilize the total codebook variance but rather satisfies a per-beam variance, meaning it has access to less flexibility in its codebook design but maintains the total variance nonetheless.

\input{alg/algorithm-ii.tex}

\begin{remark}[Design decisions]
We now present a few remarks on this approach and communicate our motivations and design decisions.
First, one benefit of this design is that it iteratively solves each transmit beam and receive beam one after another, rather than all transmit beams followed by all receive beams.
Empirically, we found that a full-fledged projected alternating minimization approach (i.e., solve for $\precbmat$, quantize, solve for $\comcbmat$, quantize, solve for $\precbmat$, quantize, ...), while seemingly superior, resulted in a bias since the first minimization (e.g., over the entire transmit codebook) would carry most of the weight in minimizing our objective.
This was worsened by projection-based quantization, which would trap our solutions in a solution that it could not escape even with more alternating minimization iterations.
Secondly, as mentioned, other designs that quantize the entire codebook at once can suffer more severely from quantization versus our solution which gradually incorporates quantization beam-by-beam, allowing later beams to account for the quantization imposed on earlier beams.
\end{remark}

\begin{remark}[Complexity]
Test
\end{remark}


% One of the artifacts of this design it does not jointly utilize the total codebook variance but rather satisfies a per-beam variance, meaning it has access to less flexibility in its codebook design but maintains the total variance nonetheless.

% Furthermore, the nature of our design allows for two convenient features that may be useful in practice.
% First, since our design has the ability to solve for individual beams while preserving the rest, it can be used to periodically update select beams.
% This may be useful to account for service updates (e.g., increasing or decreasing gain/variance) or to incorporate updated channel information.
% Secondly, an ordering of the codebook may be useful for engineers since it allows them to prioritize certain beams.
% For example, transmit beams toward the end of the codebook enjoy the fact that many receive beams have already undergone their design to reduce interference, lessening its load and optimizing it for a receive codebook $\comcbmat$ that is close to the final one.
 
% \input{alg/algorithm-v2.tex}



==> sec-statistics.tex <==
\section{Bounds on the Design Under Various Channels}

$\inrrxbar$ is the maximum $\inrrx$ across all possible $\mH = \mHbar + \mDelta$ and $\vf$ and $\vw$.

For a given $\mHbar$, what is the maximum $\inrrx$ possible when $\normfro{\mDelta}^2 \leq \eps$, $\normtwo{\vf} = 1$, and $\normtwo{\vw} = 1$?
\begin{align}
\max_{\vf,\vw} \ \normtwo{\vw\ctrans \mH \vf}^2 
&= \max_{\vf,\vw,\mDelta} \ \normtwo{\vw\ctrans \parens{\mHbar + \mDelta} \vf}^2 \\
&= \max_{\vf,\vw,\mDelta} \ \normtwo{\vw\ctrans \mHbar \vf}^2 + \normtwo{\vw\ctrans \mDelta \vf}^2 \\
&= \svmaxsq{\mHbar} + \eps
\end{align}

What is the minimum $\inrrx$ possible? Suppose $\mDelta = \zeromat$ and $\svminsq{\mHbar} = 0$.
\begin{align}
\min_{\vf,\vw} \ \normtwo{\vw\ctrans \mH \vf}^2 
&= \min_{\vf,\vw,\mDelta} \ \normtwo{\vw\ctrans \parens{\mHbar + \mDelta} \vf}^2 \\
&= \min_{\vf,\vw,\mDelta} \ \normtwo{\vw\ctrans \mHbar \vf}^2 \\
&= \svminsq{\mHbar} \\
&= 0
\end{align}

Suppose $\entry{\mHbar}{i,j} \sim \distcgauss{0}{1}$ for all $i,j$. Suppose $\mDelta = \zeromat$. What is the probability that $\inrrx$ falls below some threshold?
Without estimation error, minimum $\inrrx$ is $\svminsq{\mHbar}$. 
Its CDF is blank.

---

Suppose $\entry{\mHbar}{i,j} \sim \distcgauss{0}{1}$ for all $i,j$, where $\mHbar$ is $N \times N$.
\begin{align}
\prob{\svminsq{\mHbar} \leq t/N} 
&= \int_{0}^{t} \exp\parens{-x} \ \ddx \\
&= 1 - \exp\parens{-t}
\end{align}

--- 

Suppose $\entry{\mHbar}{i,j} \sim \distcgauss{0}{1}$ for all $i,j$. 
Suppose $\entry{\mDelta}{i,j} \sim \distcgauss{0}{\sigma^2}$ for all $i,j$. 
What is the probability that $\inrrxmin$ falls below some threshold?

---

The distribution of its worst case error depends on its 
\begin{align}
\max_{\vf,\vw,\mDelta} \ \normtwo{\vw\ctrans \mDelta \vf}^2 = \svmaxsq{\mDelta}
\end{align}

---

An upper bound on worst case error due to estimation error is $\eps$.




==> sec-system-model.tex <==
\section{Measurement Setup and Methodology} \label{sec:system-model}


==> tab/tab-fitting-results-v2.tex <==
\begin{table*}[!t]
    \small
    \centering
    \caption{System parameters and fitted model parameters.}
    \label{tab:fitting-results}
    \begin{tabular}{ccc}
        \hline
        \textbf{Parameter(s)} & \textbf{Symbol(s)} & \textbf{Value(s)} \\
        \hline
        EIRP & \textbf{$\eirp$} & $60$ dBm \\
        Noise Power (over 100 MHz) & \textbf{$\powernoise$} & $-68$ dBm \\
        \hline
        {Cluster Centers} of $\mHbar$ & $\braces{\parens{\varthetatx\idx{k},\varphitx\idx{k}}, \parens{\varthetarx\idx{k},\varphirx\idx{k}}}$ & See \tabref{tab:fitting-results-clusters} \\
        Angular Spread of $\mHbar$ & \textbf{$(\Delta\vartheta,\Delta\varphi)$} & $(4,3)$ \\
        Location Parameter of $\mu$ & \textbf{$\Gsqest$} & $-130.19$ dB \\
        Scale Parameter of $\mu$ & \textbf{$\xi$} & $0.503$ \\
        \hline
        Estimator Parameters of $\sigma^2$ & \textbf{$(\alpha,\beta)$} & $(-0.733,42.53)$ \\
        Variance Parameter of $\sigma^2$ & $\nu^2$ & $126.091$ \\
        \hline
        INR Bounds & \textbf{$\parens{\inrmin,\inrmax}$} & $(-44.57,46.99)$ dB  \\
        % \textbf{$(p_2,p_1,p_0)$} & $(1,2,3)$ & $(1,2,3)$ \\
        % \textbf{$(q_2,q_1,q_0)$} & $(1,2,3)$ & $(1,2,3)$ \\
        \hline
    \end{tabular}
\end{table*}

%\begin{table*}[!t]
%    \small
%    \centering
%    \caption{Fitting results for each measurement set.}
%    \label{tab:fitting-results}
%    \begin{tabular}{cccccc}
%        \hline
%        & \multicolumn{5}{c}{\textbf{(transmit beam, receive beam, polarization)}}  \\
%        \textbf{Parameter(s)} & \textbf{(0,0,H)} & \textbf{(1,0,H)} & \textbf{(1,1,H)} & \textbf{(0,0,V)} & \textbf{(1,0,V)} \\
%        \hline
%        \textbf{$(\Delta\vartheta,\Delta\varphi)$} & $(4,3)$ & $(4,3)$ & $(4,3)$ & $(4,3)$ & $(4,3)$ \\
%        \textbf{$\todB{\Gsqest}$} & $54.82$ & $59.63$ & $65.00$ & $61.72$ & $72.45$ \\
%        \textbf{$\xi$} & $0.4983$ & $0.4793$ & $0.4353$ & $0.4607$ & $0.5342$ \\
%        \textbf{$(\alpha,\beta)$} & $(4.22,6.54)$ & $(3.38,7.37)$ & $(2.85,7.62)$ & $(5.06,4.88)$ & $(3.93,5.75)$ \\
%        \textbf{$\parens{\todB{\inrmin},\todB{\inrmax}}$} & $(6.01,97.57)$ & $(7.04,93.74)$ & $(11.95,97.57)$ & $(6.02,95.57)$ & $(6.01,96.60)$ \\
%        % \textbf{$(p_2,p_1,p_0)$} & $(1,2,3)$ & $(1,2,3)$ \\
%        % \textbf{$(q_2,q_1,q_0)$} & $(1,2,3)$ & $(1,2,3)$ \\
%        \hline
%    \end{tabular}
%\end{table*}


==> tab/tab-fitting-results-v3.tex <==
\begin{table*}[!t]
    \small
    \centering
    \caption{System parameters and fitted model parameters from measurements.}
    \label{tab:fitting-results}
    \begin{tabular}{ccccc}
        \hline
        % \textbf{Parameter(s)} & \textbf{Symbol(s)}  & \multicolumn{3}{c}{\textbf{Value(s)}}\\
        \textbf{Parameter(s)} & \textbf{Symbol(s)} & \textbf{Default} & \textbf{Vertical} & \textbf{Tapered} \\
        \hline
        EIRP & \textbf{$\eirp$} & $60$ dBm & $60$ dBm & $54$ dBm \\
        Noise Power & \textbf{$\powernoise$} & $-68$ dBm & $-68$ dBm & $-68$ dBm \\
        \hline
        {Cluster Centers} of $\mHbar$ & ${\parens{\varthetatx\idx{k},\varphitx\idx{k}}, \parens{\varthetarx\idx{k},\varphirx\idx{k}}}$ & See \tabref{tab:fitting-results-clusters} & See \tabref{tab:fitting-results-clusters} & See \tabref{tab:fitting-results-clusters} \\
        Angular Spread of $\mHbar$ & \textbf{$(\Delta\vartheta,\Delta\varphi)$} & $(4,3)$ & $(4,3)$ & $(4,3)$ \\
        Location Parameter of $\muest$ & \textbf{$\Gsqest$} & $-130.19$ dB & $-142.83$ dB  & $-130.50$ dB \\
        Scale Parameter of $\muest$ & \textbf{$\xi$} & $0.503$ & $0.528$ & $0.392$ \\
        \hline
        Estimator Parameters of $\varest$ & \textbf{$(\alpha,\beta)$} & $(-0.733,42.53)$ & $(-0.588,29.71)$ & $(-0.822,25.42)$ \\
        Variance Parameter of $\varest$ & $\nu^2$ & $126.091$ & $75.794$ & $110.391$ \\
        \hline
        % INR Bounds & \textbf{$\parens{\inrmin,\inrmax}$} & $(-44.57,46.99)$ dB & $(-44.57,46.99)$ dB & $(-44.57,46.99)$ dB \\
        Minimum INR & $\inrmin$ & $-44.57$ dB & $-42.57$ dB & $-44.57$ dB \\
        Maximum INR & $\inrmax$ & $46.99$ dB & $46.98$ dB & $41.05$ dB \\
        % \textbf{$(p_2,p_1,p_0)$} & $(1,2,3)$ & $(1,2,3)$ \\
        % \textbf{$(q_2,q_1,q_0)$} & $(1,2,3)$ & $(1,2,3)$ \\
        \hline
    \end{tabular}
% \vspace{-0.25cm}
\end{table*}

%\begin{table*}[!t]
%    \small
%    \centering
%    \caption{Fitting results for each measurement set.}
%    \label{tab:fitting-results}
%    \begin{tabular}{cccccc}
%        \hline
%        & \multicolumn{5}{c}{\textbf{(transmit beam, receive beam, polarization)}}  \\
%        \textbf{Parameter(s)} & \textbf{(0,0,H)} & \textbf{(1,0,H)} & \textbf{(1,1,H)} & \textbf{(0,0,V)} & \textbf{(1,0,V)} \\
%        \hline
%        \textbf{$(\Delta\vartheta,\Delta\varphi)$} & $(4,3)$ & $(4,3)$ & $(4,3)$ & $(4,3)$ & $(4,3)$ \\
%        \textbf{$\todB{\Gsqest}$} & $54.82$ & $59.63$ & $65.00$ & $61.72$ & $72.45$ \\
%        \textbf{$\xi$} & $0.4983$ & $0.4793$ & $0.4353$ & $0.4607$ & $0.5342$ \\
%        \textbf{$(\alpha,\beta)$} & $(4.22,6.54)$ & $(3.38,7.37)$ & $(2.85,7.62)$ & $(5.06,4.88)$ & $(3.93,5.75)$ \\
%        \textbf{$\parens{\todB{\inrmin},\todB{\inrmax}}$} & $(6.01,97.57)$ & $(7.04,93.74)$ & $(11.95,97.57)$ & $(6.02,95.57)$ & $(6.01,96.60)$ \\
%        % \textbf{$(p_2,p_1,p_0)$} & $(1,2,3)$ & $(1,2,3)$ \\
%        % \textbf{$(q_2,q_1,q_0)$} & $(1,2,3)$ & $(1,2,3)$ \\
%        \hline
%    \end{tabular}
%\end{table*}


==> tab/tab-fitting-results.tex <==
\begin{table*}[!t]
    \small
    \centering
    \caption{Fitting results for each measurement set.}
    \label{tab:fitting-results}
    \begin{tabular}{cccccc}
        \hline
        & \multicolumn{5}{c}{\textbf{(transmit beam, receive beam, polarization)}}  \\
        \textbf{Parameter(s)} & \textbf{(0,0,H)} & \textbf{(1,0,H)} & \textbf{(1,1,H)} & \textbf{(0,0,V)} & \textbf{(1,0,V)} \\
        \hline
        \textbf{$(\Delta\vartheta,\Delta\varphi)$} & $(4,3)$ & $(4,3)$ & $(4,3)$ & $(4,3)$ & $(4,3)$ \\
        \textbf{$\todB{G^{-2}}$} & $54.82$ & $59.63$ & $65.00$ & $61.72$ & $72.45$ \\
        \textbf{$\xi$} & $0.4983$ & $0.4793$ & $0.4353$ & $0.4607$ & $0.5342$ \\
        \textbf{$(\alpha,\beta)$} & $(4.22,6.54)$ & $(3.38,7.37)$ & $(2.85,7.62)$ & $(5.06,4.88)$ & $(3.93,5.75)$ \\
        \textbf{$\parens{\todB{\inrmin},\todB{\inrmax}}$} & $(6.01,97.57)$ & $(7.04,93.74)$ & $(11.95,97.57)$ & $(6.02,95.57)$ & $(6.01,96.60)$ \\
        % \textbf{$(p_2,p_1,p_0)$} & $(1,2,3)$ & $(1,2,3)$ \\
        % \textbf{$(q_2,q_1,q_0)$} & $(1,2,3)$ & $(1,2,3)$ \\
        \hline
    \end{tabular}
\end{table*}


